Near and Mid-IR Photometry of the Pleiades, and a New List of Substellar Candidate Members

We make use of new near and mid-IR photometry of the Pleiades cluster in order to help identify proposed cluster members. We also use the new photometry with previously published photometry to define the single-star main sequence locus at the age of the Pleiades in a variety of color-magnitude planes. The new near and mid-IR photometry extend effectively two magnitudes deeper than the 2MASS All-Sky Point Source catalog, and hence allow us to select a new set of candidate very low mass and sub-stellar mass members of the Pleiades in the central square degree of the cluster. We identify 42 new candidate members fainter than Ks =14 (corresponding to 0.1 Mo). These candidate members should eventually allow a better estimate of the cluster mass function to be made down to of order 0.04 solar masses. We also use new IRAC data, in particular the images obtained at 8 um, in order to comment briefly on interstellar dust in and near the Pleiades. We confirm, as expected, that -- with one exception -- a sample of low mass stars recently identified as having 24 um excesses due to debris disks do not have significant excesses at IRAC wavelengths. However, evidence is also presented that several of the Pleiades high mass stars are found to be impacting with local condensations of the molecular cloud that is passing through the Pleiades at the current epoch.

==> table2_electronic.tex <==
\begin{deluxetable}{lllllllllllll}
\tablecaption{Pleiades Members: Literature Photometry}
\tablewidth{0pt}
\rotate
\tabletypesize{\scriptsize}
\tablehead{
\colhead{RA (deg)} &  \colhead{Dec (deg)} &
\colhead{$J$} & \colhead{$H$} & 
\colhead{\ks} & \colhead{`ph-qual'\tablenotemark{a}}& 
\colhead{$B$}&  \colhead{$V$} &
\colhead{\ic} & \colhead{Ref} & 
\colhead{names} 
}
\startdata
51.898273&24.528660&10.781$\pm$0.025&10.066$\pm$0.030&9.892$\pm$0.017&AAA1&
\nodata&\nodata&11.85&22&
DH001
\\
51.925262&23.803688&9.066$\pm$0.013&8.754$\pm$0.009&8.679$\pm$0.014&AAA1&10.96&
10.30&\nodata&4&
PELS121
\\
51.976067&24.936478&12.880$\pm$0.019&12.219$\pm$0.030&11.981$\pm$0.016&AAA1&
\nodata&\nodata&14.34&22&
DH003
\\
52.006481&23.078499&13.525$\pm$0.022&12.919$\pm$0.022&12.619$\pm$0.021&AAA1&
\nodata&\nodata&15.05&22&
DH004
\\
52.168613&25.607782&10.198$\pm$0.019&9.883$\pm$0.029&9.723$\pm$0.016&AAA1&12.59&
11.75&\nodata&9&
AKIII59
\\
52.200249&25.575842&13.072$\pm$0.019&12.442$\pm$0.029&12.153$\pm$0.015&AAA1&
\nodata&\nodata&14.75&22&
DH006
\\
52.203186&26.499350&10.429$\pm$0.019&10.006$\pm$0.029&9.924$\pm$0.016&AAA1&
\nodata&\nodata&11.16&22&
DH007
\\
52.355843&25.652304&8.459$\pm$0.015&8.314$\pm$0.059&8.270$\pm$0.031&AAA1&9.90&
9.43&\nodata&9&
AKIII79
\\
52.409874&24.510546&10.318$\pm$0.023&9.856$\pm$0.028&9.698$\pm$0.016&AAA1&
\nodata&\nodata&11.19&22&
DH008
\\
52.494766&23.371859&12.799$\pm$0.018&12.206$\pm$0.019&11.946$\pm$0.018&AAA1&
\nodata&\nodata&14.39&22&
DH009
\\
52.534420&22.644163&13.680$\pm$0.022&12.968$\pm$0.024&12.770$\pm$0.023&AAA1&
\nodata&\nodata&15.16&22&
DH010
\\
52.639614&26.215767&11.007$\pm$0.018&10.400$\pm$0.027&10.279$\pm$0.016&AAA1&
\nodata&\nodata&11.86&22&
DH011
\\
52.647411&23.052334&15.319$\pm$0.051&14.565$\pm$0.060&14.260$\pm$0.073&AAA1&
\nodata&\nodata&16.68&22&
DH012
\\
52.656086&26.346100&14.239$\pm$0.026&13.524$\pm$0.037&13.299$\pm$0.032&AAA1&
\nodata&\nodata&15.73&22&
DH013
\\
52.799591&25.165100&11.489$\pm$0.016&10.784$\pm$0.020&10.602$\pm$0.014&AAA1&
\nodata&\nodata&12.65&22&
DH014
\\
52.810955&25.981148&11.991$\pm$0.018&11.291$\pm$0.022&11.091$\pm$0.018&AAA1&
\nodata&\nodata&13.30&22&
DH015
\\
52.873249&26.503525&13.613$\pm$0.022&13.018$\pm$0.026&12.758$\pm$0.022&AAA1&
\nodata&\nodata&15.28&22&
DH016
\\
52.890076&26.265507&9.514$\pm$0.016&9.222$\pm$0.021&9.068$\pm$0.015&AAA1&11.45&
10.77&\nodata&4&
PELS008 AKIII170
\\
53.001957&23.774900&11.329$\pm$0.017&10.686$\pm$0.019&10.520$\pm$0.016&AAA1&
15.27&13.95&\nodata&4&
PELS109
\\
53.032749&23.232655&13.135$\pm$0.019&12.486$\pm$0.019&12.254$\pm$0.018&AAA1&
\nodata&\nodata&14.71&22&
DH017
\\
53.063702&26.698545&12.628$\pm$0.021&11.971$\pm$0.024&11.725$\pm$0.020&AAA1&
\nodata&\nodata&14.10&22&
DH018
\\
53.117847&22.468489&16.377$\pm$0.105&15.668$\pm$0.120&15.543$\pm$0.181&ABC1&
\nodata&\nodata&18.07&22&
DH019
\\
53.137291&22.303474&13.900$\pm$0.022&13.293$\pm$0.024&13.026$\pm$0.027&AAA1&
\nodata&\nodata&15.42&22&
DH020
\\
53.140408&24.493067&13.067$\pm$0.019&12.452$\pm$0.022&12.194$\pm$0.021&AAA1&
\nodata&\nodata&14.56&22&
DH021
\\
53.176254&23.566795&13.456$\pm$0.021&12.825$\pm$0.022&12.540$\pm$0.021&AAA1&
\nodata&\nodata&15.00&22&
DH022
\\
53.214275&25.579544&11.150$\pm$0.015&10.484$\pm$0.018&10.323$\pm$0.016&AAA1&
\nodata&\nodata&12.14&22&
DH023
\\
53.239834&27.288858&14.458$\pm$0.028&13.768$\pm$0.033&13.496$\pm$0.034&AAA1&
\nodata&\nodata&16.19&22&
DH024
\\
53.251518&25.996056&10.862$\pm$0.018&10.249$\pm$0.021&10.128$\pm$0.016&AAA1&
\nodata&\nodata&11.40&22&
DH025
\\
53.274277&22.134232&9.897$\pm$0.013&9.522$\pm$0.014&9.425$\pm$0.018&AAA1&12.25&
11.43&\nodata&4&
PELS004 DH026 AKII131
\\
53.293736&22.522045&12.119$\pm$0.016&11.448$\pm$0.019&11.248$\pm$0.021&AAA1&
\nodata&\nodata&13.66&22&
DH027
\\
53.307938&23.006475&10.259$\pm$0.016&9.787$\pm$0.019&9.669$\pm$0.011&AAA1&12.93&
11.98&\nodata&4&
PELS123 DH028 AKII138
\\
53.412479&22.352493&14.331$\pm$0.023&13.675$\pm$0.030&13.437$\pm$0.037&AAA1&
\nodata&\nodata&15.61&22&
DH029
\\
53.444305&23.805531&13.006$\pm$0.020&12.396$\pm$0.021&12.140$\pm$0.020&AAA1&
\nodata&\nodata&14.31&22&
DH030
\\
53.457481&22.938919&14.158$\pm$0.023&13.525$\pm$0.027&13.292$\pm$0.033&AAA1&
\nodata&\nodata&15.85&22&
DH031
\\
53.507523&24.880957&9.582$\pm$0.019&9.269$\pm$0.021&9.178$\pm$0.016&AAA1&11.58&
10.88&\nodata&4&
PELS005 DH032 AKIII284
\\
53.530495&24.344501&8.553$\pm$0.029&8.312$\pm$0.015&8.274$\pm$0.016&AAA1&10.08&
9.57&\nodata&4&
PELS006 TrS4 AKIII288
\\
53.579792&22.466692&13.134$\pm$0.019&12.524$\pm$0.021&12.237$\pm$0.020&AAA1&
\nodata&\nodata&14.89&22&
DH033
\\
53.580631&22.811804&14.899$\pm$0.031&14.270$\pm$0.044&13.926$\pm$0.042&AAA1&
\nodata&\nodata&16.79&22&
DH034
\\
53.592125&27.396076&12.681$\pm$0.021&11.970$\pm$0.024&11.761$\pm$0.018&AAA1&
\nodata&\nodata&14.31&22&
DH035
\\
53.673096&26.157646&14.308$\pm$0.023&13.746$\pm$0.027&13.322$\pm$0.031&AAA1&
\nodata&\nodata&15.94&22&
DH036
\\
53.684944&26.096003&11.140$\pm$0.016&10.555$\pm$0.025&10.371$\pm$0.015&AAA1&
\nodata&\nodata&12.04&22&
DH037
\\
53.693138&27.925793&12.530$\pm$0.019&11.860$\pm$0.022&11.624$\pm$0.018&AAA1&
\nodata&\nodata&14.13&22&
DH038
\\
53.696770&26.094885&9.240$\pm$0.018&8.953$\pm$0.025&8.833$\pm$0.016&AAA1&11.14&
10.48&\nodata&4&
PELS007 AKIII327
\\
53.698025&26.370512&13.615$\pm$0.021&12.949$\pm$0.026&12.733$\pm$0.025&AAA1&
\nodata&\nodata&15.07&22&
DH039
\\
53.728901&22.079634&12.403$\pm$0.020&11.798$\pm$0.013&11.566$\pm$0.018&AAA1&
\nodata&\nodata&13.89&22&
DH040
\\
53.769581&25.846750&14.754$\pm$0.028&14.143$\pm$0.038&13.763$\pm$0.045&AAA1&
\nodata&\nodata&16.47&22&
DH041
\\
53.789181&24.238947&11.908$\pm$0.018&11.235$\pm$0.021&11.029$\pm$0.018&AAA1&
\nodata&\nodata&13.27&22&
DH042
\\
53.793442&24.531931&13.549$\pm$0.020&12.936$\pm$0.024&12.658$\pm$0.022&AAA1&
\nodata&\nodata&15.17&22&
DH043
\\
53.817753&23.799503&14.083$\pm$0.026&13.504$\pm$0.026&13.185$\pm$0.027&AAA1&
\nodata&\nodata&15.71&22&
DH044
\\
53.828117&23.439199&14.892$\pm$0.035&14.246$\pm$0.041&13.980$\pm$0.049&AAA1&
\nodata&\nodata&16.67&22&
DH045
\\
53.882030&22.823627&8.831$\pm$0.019&8.599$\pm$0.019&8.541$\pm$0.014&AAA1&10.40&
9.86&\nodata&4&
PELS124
\\
53.915810&25.645988&13.989$\pm$0.021&13.280$\pm$0.024&13.044$\pm$0.028&AAA1&
\nodata&\nodata&15.40&22&
DH046
\\
53.934399&22.452787&12.870$\pm$0.019&12.244$\pm$0.020&12.023$\pm$0.019&AAA1&
\nodata&\nodata&14.40&22&
DH047
\\
53.956963&25.080112&12.603$\pm$0.018&11.947$\pm$0.020&11.691$\pm$0.022&AAA1&
\nodata&\nodata&13.98&22&
DH048
\\
53.959488&25.705828&12.887$\pm$0.018&12.273$\pm$0.025&11.990$\pm$0.020&AAA1&
\nodata&\nodata&14.40&22&
DH049
\\
53.983532&25.366608&12.401$\pm$0.023&11.754$\pm$0.024&11.524$\pm$0.019&AAA1&
\nodata&\nodata&13.70&22&
DH050
\\
54.004112&24.266083&9.793$\pm$0.017&9.489$\pm$0.020&9.388$\pm$0.016&AAA1&12.06&
11.29&\nodata&9&
AKIII391
\\
54.022148&25.351067&13.365$\pm$0.023&12.790$\pm$0.028&12.460$\pm$0.022&AAA1&
\nodata&\nodata&14.89&22&
DH051
\\
54.044819&26.264559&9.043$\pm$0.015&8.784$\pm$0.021&8.713$\pm$0.016&AAA1&\nodata
&\nodata&9.50&22&
DH052
\\
54.046085&23.806517&14.004$\pm$0.022&13.401$\pm$0.023&13.079$\pm$0.028&AAA1&
\nodata&\nodata&15.71&22&
DH053
\\
54.067921&25.146992&12.158$\pm$0.018&11.568$\pm$0.021&11.306$\pm$0.021&AAA1&
\nodata&\nodata&13.76&22&
DH054
\\
54.073441&21.894218&9.635$\pm$0.016&9.311$\pm$0.019&9.250$\pm$0.016&AAA1&11.65&
10.96&\nodata&9&
AKII293
\\
54.093006&22.742544&12.759$\pm$0.021&12.168$\pm$0.016&11.911$\pm$0.018&AAA1&
\nodata&\nodata&14.50&22&
DH055
\\
54.101337&22.623798&11.346$\pm$0.022&10.703$\pm$0.030&10.563$\pm$0.025&EAE1&
\nodata&\nodata&12.04&22&
DH056
\\
54.108974&22.246052&13.457$\pm$0.020&12.780$\pm$0.025&12.528$\pm$0.015&AAA1&
\nodata&\nodata&14.98&22&
DH057
\\
54.113979&24.688215&12.960$\pm$0.019&12.342$\pm$0.021&12.122$\pm$0.020&AAA1&
\nodata&\nodata&14.40&22&
DH058
\\
54.126263&24.012226&10.468$\pm$0.018&10.026$\pm$0.021&9.903$\pm$0.018&AAA1&13.26
&12.29&\nodata&4&
PELS189 DH059
\\
54.159966&23.145693&14.223$\pm$0.023&13.642$\pm$0.026&13.273$\pm$0.029&AAA1&
\nodata&\nodata&16.03&22&
DH060
\\
54.169426&27.832399&11.348$\pm$0.016&10.683$\pm$0.021&10.542$\pm$0.018&AAA1&
\nodata&\nodata&12.29&22&
DH061
\\
54.177719&28.351748&14.174$\pm$0.026&13.528$\pm$0.032&13.244$\pm$0.031&AAA1&
\nodata&\nodata&15.96&22&
DH062
\\
54.183781&22.027538&13.870$\pm$0.022&13.284$\pm$0.021&12.919$\pm$0.023&AAA1&
\nodata&\nodata&15.64&22&
DH063
\\
54.193634&28.251774&14.417$\pm$0.030&13.771$\pm$0.030&13.531$\pm$0.038&AAA1&
\nodata&\nodata&16.11&22&
DH064
\\
54.218864&23.262587&11.384$\pm$0.017&10.758$\pm$0.023&10.625$\pm$0.015&AAA1&
\nodata&\nodata&12.37&22&
DH065
\\
54.264439&24.743233&12.310$\pm$0.020&11.679$\pm$0.022&11.439$\pm$0.016&AAA1&
\nodata&16.00&13.60&21&
HCG6 HHJ392 DH066
\\
54.293758&25.292999&13.875$\pm$0.020&13.283$\pm$0.026&13.022$\pm$0.029&AAA1&
\nodata&\nodata&15.59&22&
DH067
\\
54.299866&26.774736&13.123$\pm$0.020&12.543$\pm$0.021&12.281$\pm$0.019&AAA1&
\nodata&\nodata&14.80&21&
HHJ242 DH068
\\
54.301289&21.468174&10.560$\pm$0.016&10.067$\pm$0.021&9.946$\pm$0.015&AAA1&13.49
&12.45&\nodata&4&
PELS009
\\
54.318829&23.184605&13.435$\pm$0.020&12.770$\pm$0.019&12.550$\pm$0.020&AAA1&
\nodata&17.90&15.20&21&
HHJ179 DH069
\\
54.319614&25.736509&13.662$\pm$0.020&13.023$\pm$0.024&12.768$\pm$0.025&AAA1&
\nodata&18.20&15.30&21&
HHJ154 DH070
\\
54.350204&22.350985&8.141$\pm$0.013&7.946$\pm$0.009&7.902$\pm$0.023&AAA1&9.71&
9.20&\nodata&4&
PELS003 HD22444 TrS19 AKII346
\\
54.359913&24.567097&13.384$\pm$0.020&12.813$\pm$0.023&12.540$\pm$0.022&AAA1&
\nodata&\nodata&14.89&22&
DH071
\\
54.360809&26.691065&12.186$\pm$0.019&11.474$\pm$0.018&11.300$\pm$0.021&AAA1&
\nodata&\nodata&13.30&21&
HHJ422
\\
54.376141&28.540815&14.488$\pm$0.030&13.891$\pm$0.033&13.589$\pm$0.035&AAA1&
\nodata&\nodata&15.93&22&
DH072
\\
54.377811&24.848555&13.834$\pm$0.023&13.262$\pm$0.026&12.974$\pm$0.026&AAA1&
\nodata&18.90&15.70&21&
HHJ110
\\
54.392365&24.704319&14.386$\pm$0.028&13.789$\pm$0.028&13.544$\pm$0.036&AAA1&
\nodata&\nodata&15.98&22&
DH074
\\
54.395443&24.236599&9.363$\pm$0.019&9.124$\pm$0.020&9.021$\pm$0.015&AAA1&11.20&
10.59&\nodata&9&
AKII359
\\
54.399998&26.546907&11.740$\pm$0.020&11.039$\pm$0.018&10.842$\pm$0.018&AAA1&
\nodata&\nodata&13.10&22&
DH075
\\
54.407017&26.351254&13.576$\pm$0.020&13.006$\pm$0.026&12.712$\pm$0.022&AAA1&
\nodata&18.10&15.20&21&
HHJ172 DH076
\\
54.446129&28.066071&11.094$\pm$0.017&10.481$\pm$0.020&10.354$\pm$0.014&AAA1&
\nodata&\nodata&12.24&22&
DH077
\\
54.447887&24.896196&14.145$\pm$0.025&13.572$\pm$0.032&13.294$\pm$0.030&AAA1&
\nodata&19.20&15.90&21&
HHJ72 DH078
\\
54.453815&26.862658&13.408$\pm$0.020&12.868$\pm$0.026&12.592$\pm$0.025&AAA1&
\nodata&\nodata&15.40&21&
HHJ137 DH079
\\
54.485046&23.382483&12.976$\pm$0.021&12.341$\pm$0.021&12.068$\pm$0.020&AAA1&
\nodata&17.40&14.60&21&
HHJ268 DH080
\\
54.508484&24.337620&13.109$\pm$0.019&12.529$\pm$0.022&12.261$\pm$0.019&AAA1&
\nodata&17.60&14.80&21&
HHJ248 DH081
\\
54.536648&21.247047&11.802$\pm$0.016&11.137$\pm$0.019&10.926$\pm$0.015&AAA1&
\nodata&\nodata&13.05&22&
DH082
\\
54.538715&27.586023&11.245$\pm$0.019&10.629$\pm$0.022&10.466$\pm$0.016&AAA1&
\nodata&\nodata&12.31&22&
DH083
\\
54.554283&24.638088&13.678$\pm$0.023&13.084$\pm$0.022&12.794$\pm$0.019&AAA1&
\nodata&18.30&15.30&21&
HHJ149 DH084
\\
54.594090&22.499697&9.018$\pm$0.025&8.775$\pm$0.021&8.696$\pm$0.015&AAA1&10.67&
10.10&\nodata&4&
PELS015 AKII383
\\
54.597412&23.108112&11.899$\pm$0.017&11.247$\pm$0.021&11.036$\pm$0.017&AAA1&
\nodata&15.30&13.30&21&
HHJ418 DH085
\\
54.600864&25.330435&13.807$\pm$0.028&13.275$\pm$0.035&12.918$\pm$0.030&AAA1&
\nodata&\nodata&15.41&22&
DH086
\\
54.603271&26.256620&13.091$\pm$0.021&12.493$\pm$0.029&12.218$\pm$0.021&AAA1&
\nodata&17.60&14.50&21&
HHJ295 DH087
\\
54.612637&27.270704&12.401$\pm$0.021&11.770$\pm$0.029&11.534$\pm$0.019&AAA1&
\nodata&\nodata&13.73&22&
DH088
\\
54.614620&25.505075&15.356$\pm$0.057&14.810$\pm$0.065&14.494$\pm$0.067&AAA1&
\nodata&\nodata&17.30&11&
HHJ2
\\
54.615955&26.857151&13.745$\pm$0.024&13.132$\pm$0.032&12.883$\pm$0.025&AAA1&
\nodata&\nodata&15.60&21&
HHJ121 DH089
\\
54.642464&23.718723&14.015$\pm$0.022&13.422$\pm$0.026&13.083$\pm$0.030&AAA1&
\nodata&19.10&15.80&21&
HHJ98 DH090
\\
54.643658&23.672913&14.015$\pm$0.022&13.427$\pm$0.024&13.097$\pm$0.030&AAA1&
\nodata&18.90&15.80&21&
HHJ97 DH091
\\
54.680405&25.374271&12.158$\pm$0.020&11.541$\pm$0.027&11.320$\pm$0.024&AAA1&
\nodata&16.40&13.80&21&
HCG11 HHJ378 DH092
\\
54.690529&27.462290&14.727$\pm$0.034&14.108$\pm$0.044&13.848$\pm$0.044&AAA1&
\nodata&\nodata&16.35&22&
DH093
\\
54.690571&24.467789&14.026$\pm$0.025&13.406$\pm$0.036&13.104$\pm$0.029&AAA1&
\nodata&19.70&15.80&21&
HHJ91 DH094
\\
54.702824&25.188787&11.038$\pm$0.018&10.384$\pm$0.029&10.231$\pm$0.022&AAA1&
\nodata&14.10&\nodata&20&
HCG12 DH095
\\
54.720390&25.236456&11.417$\pm$0.019&10.766$\pm$0.028&10.614$\pm$0.016&AAA1&
\nodata&15.50&\nodata&20&
HCG13 DH096
\\
54.724518&24.418850&12.941$\pm$0.028&12.369$\pm$0.035&12.084$\pm$0.020&AAA1&
\nodata&15.80&13.96&23&
HCG15
\\
54.725647&24.704390&14.022$\pm$0.031&13.393$\pm$0.030&13.086$\pm$0.026&AAA1&
\nodata&20.40&16.00&21&
HHJ63
\\
54.736942&24.569799&9.358$\pm$0.026&9.053$\pm$0.030&9.041$\pm$0.018&AAA1&11.19&
10.54&\nodata&4&
PELS020 DH097 AKIa006
\\
54.763737&26.491993&13.168$\pm$0.021&12.574$\pm$0.030&12.354$\pm$0.027&AAA1&
\nodata&16.90&14.30&21&
HHJ317
\\
54.766895&27.001368&13.085$\pm$0.021&12.481$\pm$0.030&12.240$\pm$0.024&AAA1&
\nodata&\nodata&14.25&22&
DH098
\\
54.783817&24.770718&12.088$\pm$0.023&11.519$\pm$0.032&11.239$\pm$0.019&AAA1&
\nodata&16.20&13.60&21&
HCG16 HHJ398 DH099
\\
54.805485&25.730488&12.630$\pm$0.019&12.019$\pm$0.030&11.759$\pm$0.020&AAA1&
\nodata&17.10&14.10&21&
HHJ349 DH100
\\
54.806122&24.466509&9.232$\pm$0.015&8.999$\pm$0.032&8.905$\pm$0.020&AAA1&11.02&
10.40&\nodata&4&
PELS018 DH101 AKIb008
\\
54.814789&26.801069&14.269$\pm$0.025&13.715$\pm$0.044&13.388$\pm$0.038&AAA1&
\nodata&\nodata&15.90&21&
HHJ66 DH102
\\
54.819721&24.960720&14.071$\pm$0.025&13.479$\pm$0.038&13.139$\pm$0.026&AAA1&
\nodata&\nodata&15.77&22&
DH103
\\
54.841930&24.044233&14.268$\pm$0.026&13.617$\pm$0.036&13.383$\pm$0.034&AAA1&
\nodata&\nodata&15.79&19&
BPL1
\\
54.843376&26.193405&13.597$\pm$0.025&12.965$\pm$0.030&12.725$\pm$0.027&AAA1&
\nodata&18.20&14.90&21&
HHJ224 DH104
\\
54.865852&23.895006&9.957$\pm$0.023&9.556$\pm$0.030&9.475$\pm$0.018&AAA1&12.42&
11.56&\nodata&4&
PELS011 AKIb010
\\
54.870735&25.582235&12.603$\pm$0.025&11.988$\pm$0.033&11.735$\pm$0.018&AAA1&
\nodata&16.70&14.00&21&
HHJ359
\\
54.871662&23.499392&11.506$\pm$0.017&10.844$\pm$0.014&10.688$\pm$0.013&AAA1&
15.60&14.23&12.50&1&
HCG20 T1B DH105
\\
54.881130&20.077984&12.567$\pm$0.019&11.913$\pm$0.017&11.705$\pm$0.016&AAA1&
\nodata&\nodata&13.75&22&
DH106
\\
54.884640&24.267057&13.072$\pm$0.019&12.471$\pm$0.033&12.201$\pm$0.024&AAA1&
\nodata&\nodata&14.57&19&
BPL2 DH107
\\
54.897739&24.118422&12.070$\pm$0.019&11.411$\pm$0.029&11.181$\pm$0.018&AAA1&
99.99&15.60&13.50&21&
HHJ407 DH108
\\
54.921291&23.473207&14.012$\pm$0.024&13.443$\pm$0.024&13.115$\pm$0.027&AAA1&
\nodata&18.80&15.80&21&
HHJ83
\\
54.921543&23.290886&8.920$\pm$0.016&8.686$\pm$0.013&8.634$\pm$0.017&AAA1&10.48&
9.94&\nodata&4&
PELS017 HD22680 AKII437
\\
54.927963&23.907763&13.276$\pm$0.020&12.655$\pm$0.019&12.406$\pm$0.017&AAA1&
18.73&17.85&14.86&1&
HCG22 T2B BPL3 HHJ230 DH109
\\
54.930431&23.207113&14.154$\pm$0.025&13.598$\pm$0.025&13.208$\pm$0.032&AAA1&
\nodata&\nodata&15.66&22&
DH110
\\
54.934086&22.129412&12.767$\pm$0.015&12.122$\pm$0.017&11.893$\pm$0.017&AAA1&
\nodata&\nodata&14.03&22&
DH111
\\
54.936604&22.654327&13.624$\pm$0.021&12.982$\pm$0.023&12.730$\pm$0.022&AAA1&
\nodata&18.20&15.40&21&
HHJ141 DH112
\\
54.943066&23.981441&12.643$\pm$0.023&12.004$\pm$0.029&11.830$\pm$0.020&AAA1&
\nodata&\nodata&14.01&19&
HHJ324 BPL4 DH113
\\
54.945892&26.354061&13.573$\pm$0.026&12.990$\pm$0.034&12.730$\pm$0.024&AAA1&
\nodata&18.20&15.20&21&
HHJ178 DH114
\\
54.949902&23.849167&12.675$\pm$0.019&12.073$\pm$0.019&11.834$\pm$0.017&AAA1&
\nodata&17.24&14.24&7&
HHJ291 BPL5 DH115
\\
54.950558&27.189531&12.877$\pm$0.023&12.273$\pm$0.029&12.019$\pm$0.020&AAA1&
\nodata&\nodata&14.02&22&
DH116
\\
54.952084&23.767841&14.038$\pm$0.025&13.435$\pm$0.028&13.131$\pm$0.029&AAA1&
\nodata&18.92&15.72&7&
HHJ74 BPL6
\\
54.957100&23.057367&13.667$\pm$0.018&13.068$\pm$0.024&12.805$\pm$0.025&AAA1&
\nodata&18.50&15.40&21&
HHJ138 DH117
\\
54.961128&23.764631&14.475$\pm$0.028&13.827$\pm$0.028&13.502$\pm$0.038&AAA1&
\nodata&\nodata&16.08&19&
BPL7 DH118
\\
54.973812&26.716982&9.003$\pm$0.019&8.778$\pm$0.028&8.660$\pm$0.020&AAA1&10.92&
10.27&\nodata&4&
PELS128 AKIII652
\\
54.980007&24.215099&14.362$\pm$0.026&13.700$\pm$0.037&13.452$\pm$0.040&AAA1&
\nodata&\nodata&15.96&19&
BPL8
\\
54.991032&25.924984&14.324$\pm$0.033&13.631$\pm$0.042&13.352$\pm$0.031&AAA1&
\nodata&\nodata&15.72&22&
DH120
\\
55.000751&23.435015&11.945$\pm$0.015&11.309$\pm$0.019&11.098$\pm$0.015&AAA1&
\nodata&15.63&13.24&20&
HCG26 SK802 HHJ403 DH121
\\
55.007530&22.989111&11.773$\pm$0.015&11.140$\pm$0.019&10.917$\pm$0.016&AAA1&
99.99&15.10&13.20&21&
HHJ426
\\
55.007618&25.072172&13.847$\pm$0.026&13.266$\pm$0.032&12.895$\pm$0.035&AAA1&
\nodata&19.40&15.80&21&
HHJ102
\\
55.007771&24.773937&13.310$\pm$0.022&12.708$\pm$0.028&12.485$\pm$0.024&AAA1&
18.90&17.69&14.84&1&
HCG24 T35B HHJ226 DH122
\\
55.012829&27.740541&8.638$\pm$0.019&8.479$\pm$0.053&8.373$\pm$0.023&AAA1&10.11&
9.62&\nodata&4&
PELS025
\\
55.020943&25.526901&12.939$\pm$0.021&12.241$\pm$0.030&12.040$\pm$0.021&AAA1&
99.99&15.90&14.00&21&
HHJ356
\\
55.023949&26.196384&9.758$\pm$0.019&9.383$\pm$0.030&9.264$\pm$0.017&AAA1&12.02&
11.22&\nodata&4&
PELS138 DH123 AKIII664
\\
55.024868&25.672556&13.801$\pm$0.023&13.186$\pm$0.037&12.923$\pm$0.028&AAA1&
\nodata&\nodata&15.34&22&
DH124
\\
55.025810&28.142338&14.321$\pm$0.034&13.720$\pm$0.044&13.403$\pm$0.035&AAA1&
\nodata&\nodata&16.10&22&
DH125
\\
55.029179&22.646589&13.921$\pm$0.021&13.290$\pm$0.024&13.052$\pm$0.028&AAA1&
\nodata&19.20&15.60&21&
HHJ114
\\
55.029575&24.217674&14.371$\pm$0.035&13.812$\pm$0.050&13.541$\pm$0.035&AAA1&
\nodata&19.57&16.16&7&
HHJ38 BPL10 DH126
\\
55.040314&23.175781&13.460$\pm$0.019&12.882$\pm$0.024&12.655$\pm$0.020&AAA1&
\nodata&\nodata&14.92&22&
HCG31 DH127
\\
55.045483&26.111404&13.629$\pm$0.023&13.016$\pm$0.034&12.749$\pm$0.023&AAA1&
99.99&18.20&15.20&21&
HCG28 HHJ177 DH128
\\
55.045963&25.390810&13.778$\pm$0.025&13.211$\pm$0.032&12.890$\pm$0.030&AAA1&
\nodata&18.30&15.30&21&
HHJ147 DH129
\\
55.050087&25.642265&10.208$\pm$0.017&9.757$\pm$0.028&9.579$\pm$0.017&AAA1&13.06&
12.12&\nodata&4&
PELS022
\\
55.053047&23.159986&12.926$\pm$0.017&12.286$\pm$0.019&12.085$\pm$0.021&AAA1&
\nodata&16.30&\nodata&21&
HCG32 SK794 HHJ280 DH130
\\
55.061630&25.834896&12.959$\pm$0.023&12.415$\pm$0.032&12.137$\pm$0.021&AAA1&
\nodata&17.54&14.86&20&
SK781
\\
55.062073&25.321938&12.343$\pm$0.019&11.690$\pm$0.035&11.507$\pm$0.016&AAA1&
\nodata&16.00&13.60&21&
SK785 HHJ397 DH131
\\
55.066326&24.375460&14.749$\pm$0.038&14.049$\pm$0.046&13.807$\pm$0.049&AAA1&
\nodata&\nodata&16.33&19&
BPL11
\\
55.069336&27.922834&12.637$\pm$0.021&11.977$\pm$0.029&11.754$\pm$0.021&AAA1&
\nodata&\nodata&13.64&22&
DH132
\\
55.082924&28.815956&11.086$\pm$0.017&10.596$\pm$0.030&10.490$\pm$0.016&AAA1&
\nodata&\nodata&12.12&22&
DH133
\\
55.091206&26.072004&10.194$\pm$0.021&9.666$\pm$0.030&9.516$\pm$0.019&AAA1&13.20&
12.20&\nodata&9&
AKIII679
\\
55.096031&25.496622&12.529$\pm$0.017&11.951$\pm$0.028&11.664$\pm$0.019&AAA1&
\nodata&16.84&14.24&20&
HCG33 HHJ343 DH134
\\
55.099293&23.069250&13.556$\pm$0.019&12.963$\pm$0.024&12.686$\pm$0.026&AAA1&
\nodata&18.20&15.20&21&
HHJ162 DH135
\\
55.100780&24.584513&12.496$\pm$0.025&11.830$\pm$0.029&11.607$\pm$0.017&AAA1&
\nodata&16.16&13.75&20&
HCG34 SK777 BPL12 DH136
\\
55.102680&22.816730&11.434$\pm$0.015&10.775$\pm$0.023&10.558$\pm$0.015&AAA1&
\nodata&14.90&12.66&20&
SK787 DH137
\\
55.106705&24.100086&13.760$\pm$0.026&13.139$\pm$0.033&12.831$\pm$0.028&AAA1&
\nodata&18.45&15.35&7&
HHJ135 BPL13 DH138
\\
55.109444&23.358168&13.506$\pm$0.020&12.931$\pm$0.029&12.670$\pm$0.021&AAA1&
\nodata&18.20&15.20&21&
HHJ167
\\
55.109978&24.089958&12.618$\pm$0.019&11.943$\pm$0.033&11.685$\pm$0.022&AAA1&
\nodata&\nodata&13.93&18&
SK778 HHJ338 BPL14 DH139
\\
55.112305&24.237360&13.441$\pm$0.025&12.828$\pm$0.029&12.517$\pm$0.025&AAA1&
\nodata&17.99&14.96&7&
HHJ169 BPL15 DH140
\\
55.123280&23.551123&11.665$\pm$0.015&10.994$\pm$0.019&10.816$\pm$0.015&AAA1&
\nodata&14.31&12.59&20&
SK775
\\
55.128021&24.487307&10.082$\pm$0.015&9.659$\pm$0.027&9.556$\pm$0.019&AAA1&12.66&
11.77&\nodata&4&
PELS019 DH141 AKIb031
\\
55.129833&25.148058&12.585$\pm$0.020&11.965$\pm$0.028&11.709$\pm$0.020&AAA1&
18.72&17.17&14.22&1&
HCG36 T102 HHJ329 DH142
\\
55.131195&23.550671&11.949$\pm$0.015&11.268$\pm$0.019&11.057$\pm$0.015&AAA1&
\nodata&15.17&13.09&20&
SK773 DH143
\\
55.135735&25.478029&14.004$\pm$0.026&13.443$\pm$0.037&13.176$\pm$0.034&AAA1&
\nodata&19.50&15.80&21&
HHJ101 DH144
\\
55.143185&23.682613&9.585$\pm$0.015&9.241$\pm$0.019&9.148$\pm$0.015&AAA1&11.62&
10.89&\nodata&4&
PELS012 DH145 AKIb030
\\
55.147179&20.965818&12.185$\pm$0.018&11.519$\pm$0.021&11.295$\pm$0.020&AAA1&
\nodata&\nodata&13.44&22&
DH146
\\
55.149448&26.151411&9.801$\pm$0.019&9.469$\pm$0.027&9.395$\pm$0.020&AAA1&11.85&
11.14&\nodata&9&
AKIII700
\\
55.164364&23.443092&15.037$\pm$0.037&14.401$\pm$0.041&14.038$\pm$0.046&AAA1&
\nodata&\nodata&16.54&22&
DH147
\\
55.166805&24.735874&12.810$\pm$0.031&12.204$\pm$0.041&11.934$\pm$0.036&AAA1&
\nodata&16.20&13.73&20&
HCG40 SK760 HHJ412
\\
55.167969&25.846764&13.086$\pm$0.019&12.448$\pm$0.030&12.208$\pm$0.022&AAA1&
\nodata&\nodata&14.34&22&
DH148
\\
55.176861&22.431391&16.622$\pm$0.121&15.754$\pm$0.121&16.020$\pm$0.268&BBD1&
\nodata&\nodata&18.41&22&
DH149
\\
55.177364&25.705488&10.799$\pm$0.021&10.240$\pm$0.030&10.134$\pm$0.020&AAA1&
\nodata&13.09&11.35&20&
HCG39 DH150
\\
55.179966&22.831705&13.809$\pm$0.022&13.166$\pm$0.028&12.927$\pm$0.022&AAA1&
\nodata&\nodata&15.34&22&
DH151
\\
55.180183&25.198736&12.202$\pm$0.020&11.474$\pm$0.027&11.283$\pm$0.024&AAA1&
\nodata&15.37&13.33&20&
SK754
\\
55.196980&23.876715&15.220$\pm$0.036&14.617$\pm$0.053&14.241$\pm$0.053&AAA1&
\nodata&\nodata&16.79&19&
BPL16
\\
55.205772&21.215467&13.450$\pm$0.021&12.791$\pm$0.023&12.487$\pm$0.024&AAA1&
\nodata&\nodata&15.07&22&
DH152
\\
55.207882&26.059305&11.356$\pm$0.019&10.702$\pm$0.028&10.482$\pm$0.022&AAA1&
\nodata&\nodata&12.04&22&
DH153
\\
55.210121&23.418465&9.531$\pm$0.017&9.192$\pm$0.021&9.123$\pm$0.015&AAA1&11.54&
10.84&\nodata&9&
AK1B038 DH154
\\
55.212769&20.688232&14.616$\pm$0.027&13.996$\pm$0.036&13.706$\pm$0.046&AAA1&
\nodata&\nodata&16.52&22&
DH155
\\
55.213596&23.598438&10.735$\pm$0.015&10.209$\pm$0.021&10.083$\pm$0.017&AAA1&
\nodata&\nodata&11.38&22&
DH156
\\
55.214352&19.546183&13.262$\pm$0.019&12.596$\pm$0.021&12.365$\pm$0.021&AAA1&
\nodata&\nodata&14.54&22&
DH157
\\
55.215866&23.230789&13.211$\pm$0.017&12.601$\pm$0.021&12.339$\pm$0.021&AAA1&
99.99&17.80&14.90&21&
HCG43 HHJ234 DH158
\\
55.226952&22.907171&13.888$\pm$0.022&13.312$\pm$0.028&12.999$\pm$0.026&AAA1&
\nodata&18.70&15.60&21&
HHJ123 DH159
\\
55.229332&22.349735&12.358$\pm$0.015&11.692$\pm$0.019&11.441$\pm$0.019&AAA1&
\nodata&16.15&13.65&20&
HCG44 SK758 HHJ355 DH160
\\
55.233509&28.727594&12.001$\pm$0.019&11.333$\pm$0.028&11.127$\pm$0.019&AAA1&
\nodata&\nodata&13.18&22&
DH161
\\
55.246910&25.198713&14.574$\pm$0.032&13.974$\pm$0.039&13.660$\pm$0.036&AAA1&
\nodata&\nodata&16.30&21&
HHJ41 DH162
\\
55.251610&24.226461&13.839$\pm$0.029&13.224$\pm$0.033&12.944$\pm$0.028&AAA1&
\nodata&\nodata&15.38&19&
BPL17
\\
55.262409&23.722698&12.915$\pm$0.017&12.277$\pm$0.021&12.003$\pm$0.020&AAA1&
\nodata&17.15&14.29&20&
HCG45 HHJ290 BPL18 DH163
\\
55.271732&23.837591&14.635$\pm$0.027&14.019$\pm$0.029&13.757$\pm$0.040&AAA1&
\nodata&\nodata&16.19&19&
BPL19
\\
55.292770&25.765617&13.034$\pm$0.018&12.408$\pm$0.027&12.166$\pm$0.022&AAA1&
\nodata&17.57&14.49&20&
SK733 DH164
\\
55.295620&28.011417&11.416$\pm$0.020&10.745$\pm$0.025&10.530$\pm$0.018&AAA1&
\nodata&\nodata&12.28&22&
DH165
\\
55.307491&23.384953&11.451$\pm$0.015&10.787$\pm$0.019&10.631$\pm$0.015&AAA1&
\nodata&\nodata&12.35&22&
DH166
\\
55.330593&23.861725&13.691$\pm$0.019&13.043$\pm$0.026&12.781$\pm$0.025&AAA1&
\nodata&\nodata&15.53&22&
HCG48 DH167
\\
55.332741&25.113682&13.659$\pm$0.024&13.082$\pm$0.031&12.828$\pm$0.025&AAA1&
\nodata&18.20&15.10&21&
HHJ191
\\
55.333279&22.631664&12.854$\pm$0.017&12.216$\pm$0.019&11.994$\pm$0.021&AAA1&
\nodata&16.95&14.21&20&
SK739 DH168
\\
55.343479&24.397757&14.280$\pm$0.029&13.570$\pm$0.031&13.347$\pm$0.028&AAA1&
\nodata&\nodata&16.00&22&
DH169
\\
55.345337&23.930075&13.262$\pm$0.018&12.629$\pm$0.028&12.342$\pm$0.022&AAA1&
\nodata&\nodata&14.76&19&
HCG49 HHJ233 BPL20 DH170
\\
55.348396&27.404812&14.259$\pm$0.025&13.643$\pm$0.032&13.291$\pm$0.036&AAA1&
\nodata&\nodata&15.57&22&
DH171
\\
55.352634&24.253899&15.157$\pm$0.042&14.488$\pm$0.058&14.199$\pm$0.045&AAA1&
\nodata&\nodata&16.96&22&
DH172
\\
55.352810&25.385002&14.050$\pm$0.021&13.415$\pm$0.032&13.099$\pm$0.025&AAA1&
\nodata&18.80&15.60&21&
HHJ117
\\
55.355484&22.548937&12.590$\pm$0.017&11.946$\pm$0.019&11.703$\pm$0.020&AAA1&
\nodata&15.90&13.89&23&
HCG51 SK732 HHJ345 DH173
\\
55.359795&23.134157&13.586$\pm$0.017&12.926$\pm$0.024&12.622$\pm$0.020&AAA1&
\nodata&\nodata&15.50&22&
DH174
\\
55.362019&24.017363&12.402$\pm$0.017&11.738$\pm$0.028&11.466$\pm$0.021&AAA1&
\nodata&17.01&13.88&20&
SK729 HHJ340 BPL21 DH175
\\
55.365917&23.708357&9.761$\pm$0.015&9.407$\pm$0.021&9.313$\pm$0.016&AAA1&11.98&
11.20&\nodata&9&
AK1B055 DH176
\\
55.379993&24.056950&13.953$\pm$0.020&13.340$\pm$0.028&13.073$\pm$0.021&AAA2&
\nodata&19.00&15.80&21&
HHJ90 BPL23 DH177
\\
55.389881&27.164007&13.966$\pm$0.027&13.354$\pm$0.034&13.002$\pm$0.030&AAA1&
\nodata&\nodata&15.45&22&
DH178
\\
55.390476&25.113523&12.977$\pm$0.021&12.336$\pm$0.028&12.093$\pm$0.022&AAA1&
99.99&17.30&14.50&21&
HCG50 HHJ285 DH179
\\
55.390682&24.188528&15.561$\pm$0.026&14.900$\pm$0.034&14.629$\pm$0.029&AAA2&
\nodata&\nodata&17.15&19&
BPL24
\\
55.391205&23.195833&15.114$\pm$0.023&14.485$\pm$0.034&14.201$\pm$0.026&AAA2&
\nodata&20.41&16.77&7&
HHJ12
\\
55.394962&23.637722&14.140$\pm$0.020&13.542$\pm$0.029&13.210$\pm$0.021&AAA2&
\nodata&\nodata&15.91&22&
DH180
\\
55.400673&25.619331&8.959$\pm$0.023&8.657$\pm$0.028&8.593$\pm$0.021&AAA1&10.69&
10.10&\nodata&4&
PELS023 DH181 AKIII756
\\
55.405205&25.142485&13.629$\pm$0.024&13.044$\pm$0.032&12.788$\pm$0.023&AAA1&
\nodata&18.30&15.30&21&
HHJ148 DH182
\\
55.411682&24.385941&14.347$\pm$0.021&13.764$\pm$0.030&13.457$\pm$0.022&AAA2&
\nodata&\nodata&15.93&19&
BPL25
\\
55.411892&22.277939&13.481$\pm$0.017&12.878$\pm$0.021&12.603$\pm$0.021&AAA1&
\nodata&\nodata&15.00&22&
HHJ176 DH183
\\
55.414906&23.763084&11.691$\pm$0.019&11.044$\pm$0.026&10.870$\pm$0.020&AAA2&
\nodata&14.51&12.69&20&
SK724 DH184
\\
55.415966&24.875067&14.243$\pm$0.016&13.650$\pm$0.028&13.364$\pm$0.022&AAA2&
\nodata&19.70&15.90&21&
HHJ69
\\
55.426693&23.915899&14.749$\pm$0.021&14.051$\pm$0.030&13.726$\pm$0.022&AAA2&
\nodata&\nodata&17.00&21&
HHJ6 BPL26
\\
55.437744&22.467276&14.346$\pm$0.025&13.729$\pm$0.030&13.470$\pm$0.036&AAA1&
\nodata&\nodata&16.10&22&
DH185
\\
55.443485&24.925913&14.937$\pm$0.018&14.395$\pm$0.031&14.060$\pm$0.023&AAA2&
\nodata&\nodata&16.61&22&
DH186
\\
55.446171&22.857038&11.728$\pm$0.017&11.062$\pm$0.019&10.852$\pm$0.017&AAA1&
\nodata&14.81&12.76&20&
HCG57 DH187
\\
55.450180&26.789177&12.797$\pm$0.021&12.134$\pm$0.028&11.901$\pm$0.017&AAA1&
\nodata&\nodata&14.00&21&
HHJ357 DH188
\\
55.453979&23.056513&14.094$\pm$0.020&13.499$\pm$0.029&13.155$\pm$0.021&AAA2&
\nodata&19.37&15.84&7&
HHJ58
\\
55.456657&22.493631&14.390$\pm$0.025&13.772$\pm$0.030&13.513$\pm$0.036&AAA1&
\nodata&\nodata&16.21&22&
DH189
\\
55.464550&24.324308&15.251$\pm$0.022&14.644$\pm$0.030&14.273$\pm$0.025&AAA2&
\nodata&\nodata&17.08&19&
BPL27
\\
55.467960&24.699417&13.928$\pm$0.016&13.347$\pm$0.029&13.052$\pm$0.020&AAA2&
\nodata&18.90&15.60&21&
HHJ120 BPL28 DH190
\\
55.470573&24.123610&14.092$\pm$0.020&13.555$\pm$0.029&13.217$\pm$0.021&AAA2&
\nodata&18.80&15.70&21&
HHJ108 BPL29 DH191
\\
55.471031&27.078693&13.750$\pm$0.026&13.192$\pm$0.031&12.874$\pm$0.029&AAA1&
\nodata&\nodata&15.22&22&
DH192
\\
55.473595&23.457975&11.155$\pm$0.019&10.386$\pm$0.033&10.249$\pm$0.033&AAA2&
\nodata&\nodata&12.14&22&
DH193
\\
55.475868&25.729809&12.798$\pm$0.017&12.127$\pm$0.030&11.911$\pm$0.021&AAA1&
18.36&16.79&14.19&1&
HCG55 B346 HHJ342 DH194
\\
55.485363&27.049528&13.779$\pm$0.023&13.191$\pm$0.035&12.903$\pm$0.030&AAA1&
\nodata&\nodata&15.25&22&
DH195
\\
55.486328&23.978710&14.173$\pm$0.020&13.536$\pm$0.028&13.230$\pm$0.021&AAA2&
\nodata&\nodata&15.79&19&
BPL30
\\
55.494366&22.950556&12.747$\pm$0.017&12.168$\pm$0.023&11.902$\pm$0.018&AAA1&
99.99&16.80&14.40&21&
HCG66 HHJ312 DH196
\\
55.494484&23.707314&11.742$\pm$0.019&11.032$\pm$0.027&10.843$\pm$0.019&AAA2&
\nodata&14.61&12.74&5&
SK709
\\
55.495197&26.205971&12.854$\pm$0.021&12.174$\pm$0.031&11.955$\pm$0.022&AAA1&
18.54&17.02&14.32&1&
HCG56 B117 HHJ351 DH197
\\
55.495556&25.329012&10.976$\pm$0.019&10.296$\pm$0.028&10.091$\pm$0.019&AAA1&
15.70&14.24&12.20&1&
HCG58 T35 DH198
\\
55.496101&25.920921&10.752$\pm$0.019&10.167$\pm$0.028&10.074$\pm$0.017&AAA1&
\nodata&\nodata&11.29&22&
DH199
\\
55.498581&24.705162&14.976$\pm$0.019&14.393$\pm$0.031&14.087$\pm$0.025&AAA2&
\nodata&\nodata&16.62&19&
BPL31
\\
55.498886&26.461098&13.519$\pm$0.022&12.960$\pm$0.031&12.635$\pm$0.024&AAA1&
\nodata&18.20&15.00&21&
HHJ213 DH200
\\
55.500050&25.029800&13.041$\pm$0.021&12.443$\pm$0.030&12.165$\pm$0.020&AAA1&
\nodata&17.19&14.66&20&
SK702 HHJ277 DH201
\\
55.501530&24.170252&15.045$\pm$0.022&14.463$\pm$0.032&14.068$\pm$0.023&AAA2&
\nodata&\nodata&16.70&19&
BPL32
\\
55.506943&22.390800&13.332$\pm$0.018&12.712$\pm$0.021&12.427$\pm$0.019&AAA1&
99.99&17.80&15.00&21&
HCG67 HHJ201 DH202
\\
55.511932&24.210073&12.514$\pm$0.019&11.835$\pm$0.028&11.606$\pm$0.019&AAA2&
\nodata&16.41&13.80&20&
HCG63 HHJ350 BPL33 DH203
\\
55.512192&23.931648&12.017$\pm$0.019&11.362$\pm$0.028&11.128$\pm$0.020&AAA2&
\nodata&\nodata&13.51&19&
HCG64 HHJ406 BPL34 DH204
\\
55.513741&24.537067&12.523$\pm$0.019&11.860$\pm$0.030&11.632$\pm$0.019&AAA2&
\nodata&16.36&13.79&20&
SK701 HHJ354 BPL35 DH205
\\
55.514214&25.377609&13.346$\pm$0.021&12.729$\pm$0.028&12.444$\pm$0.026&AAA1&
\nodata&18.10&15.00&21&
HHJ212 DH206
\\
55.515965&24.712622&10.740$\pm$0.021&10.100$\pm$0.033&9.916$\pm$0.022&AAA1&14.82
&13.46&11.73&1&
HCG65 A100 DH207
\\
55.516399&22.426901&9.797$\pm$0.018&9.338$\pm$0.019&9.159$\pm$0.015&AAA1&12.72&
11.74&\nodata&4&
PELS028 DH208 AKIa029
\\
55.517284&22.280857&13.541$\pm$0.018&12.859$\pm$0.023&12.611$\pm$0.024&AAA1&
\nodata&17.22&15.04&20&
SK708
\\
55.519608&25.885885&10.784$\pm$0.019&10.183$\pm$0.025&10.093$\pm$0.019&AAA1&
\nodata&13.01&11.70&5&
HCG61 DH209
\\
55.520260&25.663296&11.798$\pm$0.021&11.110$\pm$0.028&10.896$\pm$0.021&AAA1&
\nodata&15.58&13.13&5&
SK698 DH210
\\
55.534512&25.616734&13.036$\pm$0.023&12.408$\pm$0.027&12.156$\pm$0.023&AAA1&
\nodata&17.80&14.60&21&
HHJ270 DH211
\\
55.536823&23.588072&12.208$\pm$0.019&11.511$\pm$0.027&11.313$\pm$0.020&AAA2&
\nodata&15.81&13.44&5&
SK699 HHJ384 DH212
\\
55.541031&27.957092&12.893$\pm$0.023&12.189$\pm$0.030&11.974$\pm$0.022&AAA1&
\nodata&\nodata&13.60&22&
DH213
\\
55.544144&22.301603&14.190$\pm$0.024&13.610$\pm$0.028&13.260$\pm$0.027&AAA1&
\nodata&19.20&16.00&21&
HHJ55
\\
55.545494&24.085728&12.027$\pm$0.019&11.366$\pm$0.028&11.152$\pm$0.019&AAA2&
17.45&15.95&13.44&1&
HCG68 T36 HHJ396 DH214
\\
55.552551&26.829239&13.283$\pm$0.022&12.642$\pm$0.030&12.371$\pm$0.025&AAA1&
\nodata&\nodata&14.90&21&
HHJ236 DH215
\\
55.556168&24.313845&14.493$\pm$0.020&13.907$\pm$0.027&13.587$\pm$0.022&AAA2&
\nodata&\nodata&16.40&21&
HHJ34 BPL36
\\
55.557869&20.362230&13.649$\pm$0.021&13.064$\pm$0.023&12.794$\pm$0.021&AAA1&
\nodata&\nodata&15.58&22&
DH216
\\
55.564034&23.191994&13.859$\pm$0.020&13.286$\pm$0.027&12.997$\pm$0.020&AAA2&
\nodata&19.10&15.70&21&
HHJ109
\\
55.570366&23.390644&13.489$\pm$0.020&12.823$\pm$0.028&12.566$\pm$0.020&AAA2&
\nodata&17.83&15.22&20&
SK694
\\
55.574543&24.116062&13.847$\pm$0.020&13.237$\pm$0.029&12.926$\pm$0.020&AAA2&
\nodata&18.90&15.50&21&
HHJ129 BPL37 DH217
\\
55.578609&23.989525&12.048$\pm$0.021&11.346$\pm$0.030&11.174$\pm$0.019&AAA1&
99.99&14.67&13.07&20&
SK687 HHJ437
\\
55.589748&24.664650&11.578$\pm$0.015&10.933$\pm$0.027&10.718$\pm$0.019&AAA2&
15.89&14.48&12.66&1&
HCG71 B256 DH218
\\
55.592190&25.065676&14.685$\pm$0.036&13.989$\pm$0.041&13.755$\pm$0.046&AAA1&
\nodata&\nodata&16.01&22&
DH219
\\
55.599987&21.473492&8.797$\pm$0.013&8.604$\pm$0.025&8.526$\pm$0.017&AAA1&10.40&
9.85&\nodata&4&
PELS035 TrS42
\\
55.600094&22.421131&9.117$\pm$0.018&8.868$\pm$0.025&8.758$\pm$0.015&AAA1&11.03&
10.39&\nodata&4&
PELS029 DH220 AKIa036
\\
55.609455&23.860777&14.325$\pm$0.017&13.722$\pm$0.029&13.388$\pm$0.022&AAA2&
\nodata&19.49&16.12&7&
HHJ49 BPL38 DH221
\\
55.609512&24.235518&13.215$\pm$0.019&12.621$\pm$0.028&12.343$\pm$0.020&AAA2&
\nodata&17.83&15.03&20&
HCG73 SK680 HHJ262 BPL39
\\
55.609531&22.894669&11.550$\pm$0.016&10.880$\pm$0.023&10.715$\pm$0.019&AAA1&
15.86&14.45&12.64&1&
HCG75 B289 DH222
\\
55.613766&22.573578&12.699$\pm$0.017&12.126$\pm$0.023&11.856$\pm$0.019&AAA1&
\nodata&17.04&14.45&20&
HCG76 HHJ294 DH224
\\
55.614990&25.047003&10.736$\pm$0.019&10.200$\pm$0.025&10.065$\pm$0.020&AAA1&
13.73&12.66&\nodata&9&
AK1B078 DH225
\\
55.618435&27.216274&15.655$\pm$0.057&15.055$\pm$0.082&14.667$\pm$0.093&AAA1&
\nodata&\nodata&16.95&22&
DH226
\\
55.619373&25.016804&12.573$\pm$0.019&11.934$\pm$0.028&11.672$\pm$0.022&AAA1&
\nodata&16.48&14.13&20&
SK676 HHJ362 DH227
\\
55.622574&22.790607&11.797$\pm$0.016&11.085$\pm$0.021&10.920$\pm$0.017&AAA1&
16.66&15.16&13.07&1&
HCG77 A80 DH228
\\
55.622902&22.396116&12.315$\pm$0.018&11.797$\pm$0.025&11.548$\pm$0.019&AAA1&
\nodata&15.88&13.54&5&
SK682
\\
55.623756&20.811134&13.336$\pm$0.019&12.686$\pm$0.023&12.426$\pm$0.025&AAA1&
\nodata&\nodata&14.90&22&
DH229
\\
55.630009&24.822643&14.019$\pm$0.016&13.447$\pm$0.028&13.129$\pm$0.021&AAA2&
99.99&19.10&15.80&21&
HCG74 HHJ82 DH230
\\
55.641521&24.183582&14.371$\pm$0.021&13.790$\pm$0.029&13.457$\pm$0.020&AAA2&
\nodata&\nodata&15.94&19&
BPL40 DH231
\\
55.651115&23.368010&13.181$\pm$0.019&12.578$\pm$0.028&12.316$\pm$0.019&AAA2&
19.21&17.60&14.68&1&
HCG79 HHJ241 HHJ241 DH232
\\
55.653927&25.232704&14.214$\pm$0.028&13.580$\pm$0.041&13.291$\pm$0.032&AAA1&
\nodata&\nodata&15.76&22&
DH233
\\
55.667610&23.989374&12.021$\pm$0.015&11.385$\pm$0.026&11.137$\pm$0.019&AAA2&
17.07&15.72&13.29&1&
HCG80 T3 HHJ409 DH234
\\
55.671555&24.028597&13.978$\pm$0.020&13.360$\pm$0.028&13.087$\pm$0.021&AAA2&
\nodata&\nodata&15.56&19&
HCG82 HHJ115 BPL41 DH235
\\
55.674370&24.004383&13.562$\pm$0.020&12.927$\pm$0.027&12.714$\pm$0.020&AAA2&
\nodata&\nodata&15.04&19&
BPL42 DH236
\\
55.674564&24.199537&11.403$\pm$0.020&10.729$\pm$0.030&10.532$\pm$0.021&AAA2&
\nodata&14.37&12.52&5&
SK671
\\
55.675457&25.196920&14.304$\pm$0.031&13.764$\pm$0.040&13.390$\pm$0.038&AAA1&
\nodata&19.61&16.05&7&
HHJ45 DH237
\\
55.676598&23.502871&10.344$\pm$0.018&9.821$\pm$0.019&9.675$\pm$0.020&AAA1&
\nodata&12.75&11.07&20&
HCG85
\\
55.676662&23.339376&12.249$\pm$0.019&11.667$\pm$0.029&11.388$\pm$0.020&AAA2&
\nodata&17.04&13.92&5&
HCG86 DH238
\\
55.682472&25.535126&12.701$\pm$0.017&12.080$\pm$0.028&11.818$\pm$0.019&AAA1&
99.99&16.53&14.05&20&
SK665 HHJ341 DH239
\\
55.684860&23.104542&13.822$\pm$0.020&13.237$\pm$0.029&12.954$\pm$0.020&AAA2&
\nodata&19.00&15.60&21&
HHJ119 DH240
\\
55.685242&23.970976&14.092$\pm$0.016&13.540$\pm$0.029&13.217$\pm$0.021&AAA2&
\nodata&\nodata&15.71&19&
BPL43 DH241
\\
55.690193&23.823021&14.300$\pm$0.020&13.694$\pm$0.027&13.405$\pm$0.021&AAA2&
\nodata&19.50&16.11&7&
HHJ52 BPL44
\\
55.700706&24.067062&16.099$\pm$0.031&15.465$\pm$0.046&15.022$\pm$0.038&AAA2&
\nodata&\nodata&18.37&19&
BPL45
\\
55.703770&23.580189&13.626$\pm$0.020&13.058$\pm$0.028&12.774$\pm$0.020&AAA2&
\nodata&18.60&15.30&21&
HHJ153 DH242
\\
55.704578&24.171015&12.637$\pm$0.019&12.062$\pm$0.028&11.740$\pm$0.020&AAA2&
\nodata&17.08&13.97&20&
SK663 BPL46 DH243
\\
55.724968&26.137877&13.718$\pm$0.024&13.153$\pm$0.035&12.825$\pm$0.026&AAA1&
\nodata&18.70&15.30&21&
HHJ146 DH244
\\
55.729626&24.493065&8.514$\pm$0.009&8.325$\pm$0.027&8.263$\pm$0.013&AAA1&9.95&
9.47&8.90&3&
HII25 HD23061 TrR11
\\
55.735577&24.082775&12.076$\pm$0.019&11.495$\pm$0.027&11.228$\pm$0.020&AAA2&
\nodata&16.46&13.57&5&
HCG93 SK658 HHJ401 BPL48
\\
55.735668&24.229362&13.895$\pm$0.021&13.301$\pm$0.029&12.971$\pm$0.021&AAA2&
\nodata&\nodata&15.46&19&
HCG92 BPL47
\\
55.736076&25.980692&12.818$\pm$0.022&12.298$\pm$0.034&11.964$\pm$0.028&AAA1&
\nodata&18.00&\nodata&21&
HCG88 HHJ320 DH246
\\
55.744125&20.212561&13.876$\pm$0.022&13.184$\pm$0.023&12.946$\pm$0.023&AAA1&
\nodata&\nodata&15.87&22&
DH247
\\
55.746746&22.900925&10.280$\pm$0.016&9.850$\pm$0.023&9.713$\pm$0.017&AAA1&12.99&
12.05&\nodata&4&
PELS030 DH248 AKIa046
\\
55.748962&22.424271&11.453$\pm$0.018&10.744$\pm$0.021&10.587$\pm$0.017&AAA1&
\nodata&\nodata&12.15&22&
DH249
\\
55.750690&24.731268&16.058$\pm$0.031&15.459$\pm$0.043&15.013$\pm$0.037&AAA2&
\nodata&\nodata&18.32&19&
BPL49
\\
55.755241&24.247917&14.226$\pm$0.020&13.605$\pm$0.029&13.306$\pm$0.021&AAA2&
\nodata&\nodata&15.86&19&
BPL50
\\
55.762230&24.669737&10.275$\pm$0.019&9.808$\pm$0.028&9.727$\pm$0.017&AAA1&12.88&
11.96&10.98&1&
HII34 DH250
\\
55.767460&22.800989&11.676$\pm$0.015&10.997$\pm$0.014&10.785$\pm$0.013&AAA1&
16.72&15.16&12.96&1&
HCG101 B173 HHJ428 DH251
\\
55.768131&25.436737&13.822$\pm$0.023&13.174$\pm$0.031&12.880$\pm$0.023&AAA1&
\nodata&19.00&15.70&21&
HHJ107
\\
55.773048&24.824587&11.670$\pm$0.015&11.005$\pm$0.028&10.789$\pm$0.019&AAA2&
\nodata&15.21&12.98&20&
HCG97 HHJ432 DH252
\\
55.777054&22.297075&14.739$\pm$0.030&14.147$\pm$0.035&13.789$\pm$0.041&AAA1&
\nodata&19.99&16.57&7&
HHJ18
\\
55.781536&25.574789&13.070$\pm$0.018&12.459$\pm$0.030&12.190$\pm$0.022&AAA1&
\nodata&\nodata&14.72&22&
HCG96 DH253
\\
55.790607&24.692490&12.288$\pm$0.015&11.648$\pm$0.027&11.420$\pm$0.020&AAA2&
17.97&16.37&13.73&1&
HCG100 SK654 T40 BPL51 DH254
\\
55.798210&25.423109&12.911$\pm$0.021&12.299$\pm$0.031&12.046$\pm$0.023&AAA1&
\nodata&17.51&14.65&20&
SK650
\\
55.798500&24.114626&14.075$\pm$0.020&13.457$\pm$0.027&13.165$\pm$0.020&AAA2&
\nodata&19.50&15.90&21&
HHJ71 BPL52
\\
55.800495&24.745934&12.586$\pm$0.015&11.932$\pm$0.027&11.687$\pm$0.020&AAA2&
\nodata&17.16&14.23&20&
HCG102 SK653 HHJ328 BPL53
\\
55.804447&24.655403&12.231$\pm$0.015&11.514$\pm$0.026&11.293$\pm$0.019&AAA2&
\nodata&16.05&13.51&20&
HCG103 SK652 HHJ395 BPL54
\\
55.806698&25.270140&10.254$\pm$0.020&9.851$\pm$0.031&9.665$\pm$0.020&AAA1&
\nodata&\nodata&11.10&22&
DH257
\\
55.807945&24.138950&13.868$\pm$0.020&13.255$\pm$0.029&12.975$\pm$0.020&AAA2&
\nodata&\nodata&15.42&19&
BPL55
\\
55.815552&25.341557&12.339$\pm$0.020&11.701$\pm$0.028&11.504$\pm$0.020&AAA1&
\nodata&15.57&13.48&5&
SK646
\\
55.819164&23.833788&13.281$\pm$0.015&12.644$\pm$0.027&12.400$\pm$0.020&AAA2&
\nodata&18.48&15.32&20&
HHJ206 BPL56 DH258
\\
55.826839&26.673519&12.158$\pm$0.020&11.536$\pm$0.027&11.270$\pm$0.025&AAA1&
\nodata&\nodata&13.40&21&
HHJ413
\\
55.829182&22.786299&13.633$\pm$0.018&13.045$\pm$0.023&12.762$\pm$0.022&AAA1&
99.99&18.30&15.40&21&
HCG110 HHJ143 DH259
\\
55.829269&22.449223&9.639$\pm$0.016&9.160$\pm$0.017&9.026$\pm$0.018&AAA1&12.56&
11.58&\nodata&4&
PELS031 AKIa052
\\
55.829376&26.078924&13.224$\pm$0.023&12.615$\pm$0.027&12.310$\pm$0.021&AAA1&
99.99&18.00&14.60&20&
SK642 HHJ279 DH260
\\
55.835712&24.443079&14.088$\pm$0.019&13.466$\pm$0.027&13.155$\pm$0.020&AAA2&
\nodata&\nodata&15.67&19&
HCG106 HHJ88 BPL57 DH261
\\
55.837959&24.185894&14.254$\pm$0.020&13.646$\pm$0.029&13.345$\pm$0.022&AAE2&
\nodata&19.80&15.90&21&
HHJ65
\\
55.852238&23.225933&9.101$\pm$0.015&8.722$\pm$0.014&8.655$\pm$0.015&AAA1&11.23&
10.52&9.68&13&
HII102 Tr34 DH262
\\
55.854088&23.867096&15.433$\pm$0.021&14.801$\pm$0.032&14.452$\pm$0.029&AAA2&
\nodata&\nodata&17.38&19&
BPL58
\\
55.854794&22.895720&13.805$\pm$0.018&13.188$\pm$0.024&12.914$\pm$0.025&AAA1&
\nodata&18.70&15.50&21&
HHJ134 DH263
\\
55.859150&26.041912&12.773$\pm$0.021&12.131$\pm$0.030&11.890$\pm$0.022&AAA1&
\nodata&16.56&14.34&20&
HCG105 SK633 HHJ327 DH264
\\
55.860146&22.711876&13.160$\pm$0.015&12.516$\pm$0.021&12.269$\pm$0.019&AAA1&
\nodata&17.30&14.60&21&
HCG114 SK644 HHJ261 DH265
\\
55.860924&24.994333&10.477$\pm$0.015&9.956$\pm$0.028&9.795$\pm$0.019&AAA1&13.73&
12.65&11.40&1&
HII97 HCG108 DH266
\\
55.862373&24.452726&12.315$\pm$0.018&11.682$\pm$0.026&11.419$\pm$0.019&AAA2&
\nodata&16.89&13.71&20&
SK638 HHJ368 BPL59 DH267
\\
55.863014&25.387577&9.752$\pm$0.018&9.311$\pm$0.027&9.218$\pm$0.022&AAA1&12.25&
11.44&\nodata&4&
PELS056 AKIb121
\\
55.864304&22.628160&14.157$\pm$0.022&13.563$\pm$0.027&13.251$\pm$0.031&AAA1&
\nodata&19.30&15.90&21&
HHJ70
\\
55.867493&24.891973&13.036$\pm$0.019&12.394$\pm$0.027&12.168$\pm$0.020&AAA2&
\nodata&17.53&15.04&20&
HCG109 SK635 DH268
\\
55.869724&24.151775&14.147$\pm$0.020&13.563$\pm$0.029&13.240$\pm$0.020&AAA2&
\nodata&20.00&15.90&21&
HHJ76
\\
55.874538&24.656565&14.351$\pm$0.016&13.707$\pm$0.028&13.425$\pm$0.021&AAA2&
\nodata&20.00&16.10&21&
HHJ50 DH269
\\
55.879665&22.158371&9.086$\pm$0.016&8.819$\pm$0.019&8.777$\pm$0.019&AAA1&11.08&
10.41&\nodata&4&
PELS037 AKIa056
\\
55.883141&23.674074&9.527$\pm$0.015&9.192$\pm$0.012&9.103$\pm$0.018&AAA1&11.54&
10.84&10.06&1&
HII120 Tr37
\\
55.892231&25.590605&12.838$\pm$0.018&12.225$\pm$0.028&11.998$\pm$0.022&AAA1&
18.53&16.99&14.32&2&
HCG112 DH270
\\
55.893372&23.761917&9.865$\pm$0.013&9.476$\pm$0.017&9.370$\pm$0.018&AAA1&12.35&
11.47&99.99&3&
HII129 Tr041 DH271
\\
55.896713&25.408670&12.786$\pm$0.024&12.156$\pm$0.030&11.952$\pm$0.025&AAA1&
\nodata&16.88&14.23&5&
SK622 HHJ337 DH272
\\
55.902348&23.209543&13.259$\pm$0.019&12.660$\pm$0.029&12.374$\pm$0.020&AAA2&
19.60&18.00&14.93&12&
HCG122 T6 HHJ205 DH274
\\
55.902496&23.453930&11.575$\pm$0.019&10.873$\pm$0.027&10.726$\pm$0.020&AAA2&
15.93&14.52&12.71&1&
HII146 HCG121 SK631 DH275
\\
55.902607&24.232300&10.980$\pm$0.013&10.477$\pm$0.037&10.126$\pm$0.025&AAA1&
15.84&14.37&12.27&1&
HII134 HCG119 SK629
\\
55.902779&25.783554&12.885$\pm$0.018&12.282$\pm$0.028&12.049$\pm$0.022&AAA1&
\nodata&16.83&14.23&5&
SK619 DH276
\\
55.903843&24.393944&11.476$\pm$0.018&10.801$\pm$0.027&10.636$\pm$0.019&AAA2&
15.61&14.26&12.53&1&
HII133 HCG118 SK625 DH277
\\
55.904587&23.642277&12.767$\pm$0.019&12.141$\pm$0.026&11.869$\pm$0.020&AAA2&
\nodata&16.97&14.25&20&
SK630 DH278
\\
55.905468&25.408987&12.559$\pm$0.020&11.909$\pm$0.027&11.659$\pm$0.022&AAA1&
\nodata&16.37&13.87&5&
HCG115 SK620 HHJ377 DH279
\\
55.907204&23.536011&9.529$\pm$0.015&9.191$\pm$0.014&9.124$\pm$0.018&AAA1&11.42&
10.73&10.00&1&
HII152 Tr46
\\
55.908592&26.612484&11.397$\pm$0.020&10.784$\pm$0.027&10.614$\pm$0.024&AAA1&
\nodata&\nodata&12.39&22&
DH280
\\
55.912655&23.734838&13.187$\pm$0.015&12.533$\pm$0.027&12.266$\pm$0.019&AAA2&
\nodata&18.05&14.95&5&
HCG124 SK624 BPL61 DH281
\\
55.915485&23.692404&14.475$\pm$0.017&13.898$\pm$0.029&13.573$\pm$0.022&AAA2&
\nodata&\nodata&16.30&21&
HHJ40
\\
55.917908&24.503187&16.538$\pm$0.043&15.848$\pm$0.056&15.352$\pm$0.054&AAA2&
\nodata&\nodata&19.19&19&
BPL62
\\
55.923031&23.649132&7.198$\pm$0.019&7.070$\pm$0.013&7.028$\pm$0.017&AAA1&8.26&
7.92&7.51&3&
HII157 HD23157 Tr050
\\
55.925556&24.573168&11.832$\pm$0.019&11.197$\pm$0.027&10.955$\pm$0.020&AAA2&
17.00&15.43&13.12&1&
HCG123 SK616 MT41 DH282
\\
55.928608&23.594801&8.535$\pm$0.013&8.316$\pm$0.009&8.233$\pm$0.021&AAA1&10.02&
9.52&8.94&3&
HII164 HD23158 Tr53
\\
55.928703&25.860346&14.136$\pm$0.030&13.536$\pm$0.036&13.217$\pm$0.025&AAA1&
\nodata&19.40&15.80&21&
HHJ77
\\
55.929760&24.548950&14.045$\pm$0.020&13.441$\pm$0.028&13.108$\pm$0.020&AAA2&
\nodata&\nodata&15.37&22&
DH283
\\
55.930000&25.080687&7.207$\pm$0.013&7.241$\pm$0.057&7.168$\pm$0.021&AAA1&7.67&
7.52&7.36&3&
HII153 HD23155 Tr47
\\
55.930210&24.374550&7.692$\pm$0.035&7.610$\pm$0.053&7.561$\pm$0.011&AAA1&8.48&
8.23&7.92&3&
HII158 HD23156 Tr51
\\
55.931335&24.213951&14.417$\pm$0.017&13.860$\pm$0.029&13.554$\pm$0.022&AAA2&
\nodata&\nodata&16.20&21&
HHJ43 DH284
\\
55.932117&24.487711&12.408$\pm$0.019&11.721$\pm$0.027&11.497$\pm$0.020&AAA2&
\nodata&16.10&13.80&21&
HHJ374 BPL63 DH285
\\
55.937355&23.055908&12.694$\pm$0.019&11.989$\pm$0.027&11.731$\pm$0.019&AAA2&
\nodata&16.83&14.17&5&
SK618 HHJ321 DH286
\\
55.946163&26.076544&12.915$\pm$0.025&12.260$\pm$0.030&12.076$\pm$0.015&AAA1&
99.99&17.15&14.46&20&
SK607 HHJ311 DH287
\\
55.947838&23.211800&9.034$\pm$0.017&8.682$\pm$0.021&8.552$\pm$0.016&AAA1&11.32&
10.52&99.99&3&
HII186 Tr58 DH288
\\
55.949848&25.053202&11.695$\pm$0.021&10.981$\pm$0.029&10.832$\pm$0.016&AAA1&
\nodata&\nodata&12.42&22&
DH290
\\
55.951378&25.004387&9.958$\pm$0.023&9.496$\pm$0.030&9.374$\pm$0.016&AAA1&12.47&
11.62&99.99&3&
HII174 Tr56
\\
55.951721&25.190042&9.326$\pm$0.017&8.962$\pm$0.029&8.827$\pm$0.016&AAA1&11.73&
10.89&9.99&1&
HII173 DH291
\\
55.951855&25.043606&12.847$\pm$0.023&12.240$\pm$0.029&11.957$\pm$0.016&AAA1&
99.99&17.30&14.40&21&
HCG125 HHJ298 DH292
\\
55.952511&23.539379&11.392$\pm$0.019&10.750$\pm$0.027&10.555$\pm$0.019&AAA2&
15.36&13.99&12.33&16&
HII189 SK611 DH293
\\
55.954216&25.729616&10.294$\pm$0.017&9.834$\pm$0.029&9.719$\pm$0.016&AAA1&13.20&
12.24&\nodata&4&
PELS043 DH294
\\
55.959850&25.053202&11.695$\pm$0.024&10.981$\pm$0.039&10.832$\pm$0.018&AAA1&
\nodata&14.49&12.68&5&
SK609
\\
55.961143&25.268934&8.511$\pm$0.017&8.284$\pm$0.047&8.214$\pm$0.009&AAA1&10.15&
9.63&\nodata&9&
AK1B146 HD23170
\\
55.961273&24.247465&9.833$\pm$0.021&9.429$\pm$0.035&9.344$\pm$0.016&AAA1&12.09&
11.30&10.44&1&
HII193 Tr060
\\
55.964043&21.150957&13.648$\pm$0.020&13.001$\pm$0.023&12.747$\pm$0.024&AAA1&
\nodata&\nodata&15.15&22&
DH295
\\
55.965637&24.237814&13.281$\pm$0.015&12.651$\pm$0.027&12.384$\pm$0.021&AAA2&
\nodata&\nodata&14.84&19&
HCG128 BPL65 DH296
\\
55.967266&24.841591&11.509$\pm$0.015&10.883$\pm$0.029&10.646$\pm$0.019&AAA2&
15.89&14.50&12.66&17&
HII191 HCG127 SK606 DH297
\\
55.969906&25.491802&13.440$\pm$0.021&12.872$\pm$0.031&12.599$\pm$0.022&AAA1&
\nodata&\nodata&15.06&22&
HHJ218 DH298
\\
55.973091&24.519915&16.671$\pm$0.048&15.941$\pm$0.056&15.303$\pm$0.045&AAA2&
\nodata&\nodata&19.53&19&
BPL66
\\
55.974449&25.475054&12.346$\pm$0.017&11.718$\pm$0.030&11.467$\pm$0.022&AAA1&
17.79&16.15&13.71&1&
HCG126 SK600 T69 HHJ391
\\
55.982037&24.426390&11.514$\pm$0.019&10.820$\pm$0.026&10.645$\pm$0.021&AAA2&
15.67&14.30&12.55&1&
HII212 HCG130 SK603
\\
55.986195&25.262264&12.223$\pm$0.019&11.518$\pm$0.029&11.320$\pm$0.017&AAA1&
\nodata&15.80&13.46&5&
SK596 DH300
\\
55.986244&24.993528&12.391$\pm$0.023&11.727$\pm$0.029&11.511$\pm$0.018&AAA1&
\nodata&16.07&13.89&20&
HCG129 SK598 HHJ382 DH301
\\
55.987480&23.951660&13.201$\pm$0.019&12.532$\pm$0.027&12.304$\pm$0.019&AAA2&
18.99&17.93&14.85&1&
HCG135 HHJ229 DH302
\\
55.988647&24.222366&13.210$\pm$0.015&12.610$\pm$0.027&12.370$\pm$0.020&AAA2&
\nodata&17.57&14.71&20&
HCG133 SK601 BPL67 DH303
\\
55.995003&23.882730&8.600$\pm$0.031&8.420$\pm$0.039&8.308$\pm$0.019&AAA1&10.18&
9.66&9.00&3&
HII233 HD23195 Tr075
\\
56.001106&24.556950&7.633$\pm$0.033&7.618$\pm$0.041&7.583$\pm$0.011&AAA1&8.26&
8.06&7.85&3&
HII232 HD23194 Tr074
\\
56.002472&23.543961&9.650$\pm$0.015&9.274$\pm$0.014&9.199$\pm$0.018&AAA1&11.79&
11.02&10.17&1&
HII248 Tr079 DH304
\\
56.002628&21.282097&10.781$\pm$0.017&10.192$\pm$0.015&10.047$\pm$0.017&AAA1&
\nodata&\nodata&11.38&22&
DH305
\\
56.006973&23.862829&12.822$\pm$0.019&12.261$\pm$0.028&11.993$\pm$0.020&AAA2&
19.17&17.22&14.38&1&
JRS26 BPL68
\\
56.009483&25.064943&12.150$\pm$0.025&11.492$\pm$0.032&11.271$\pm$0.016&AAA1&
17.13&15.62&13.38&1&
HCG134 SK591 T150 DH306
\\
56.010338&21.221170&13.749$\pm$0.022&13.098$\pm$0.026&12.857$\pm$0.023&AAA1&
\nodata&\nodata&15.58&22&
DH307
\\
56.011784&25.656338&10.742$\pm$0.019&10.094$\pm$0.028&10.014$\pm$0.018&AAA1&
\nodata&12.96&11.65&5&
HCG131 DH308
\\
56.014748&24.504206&9.405$\pm$0.019&9.118$\pm$0.028&8.953$\pm$0.018&AAA1&11.39&
10.71&9.91&3&
HII253 Tr081 DH309
\\
56.017681&24.989822&9.499$\pm$0.025&9.168$\pm$0.045&9.061$\pm$0.018&AAA1&11.37&
10.70&9.97&10&
HII250 Tr080
\\
56.018703&25.856289&10.531$\pm$0.017&9.964$\pm$0.033&9.845$\pm$0.018&AAA1&
\nodata&12.84&11.41&20&
HCG132 DH310
\\
56.020168&24.275501&9.943$\pm$0.025&9.494$\pm$0.034&9.386$\pm$0.018&AAA1&12.51&
11.63&10.67&1&
HII263 Tr089
\\
56.021221&25.483807&10.605$\pm$0.019&10.087$\pm$0.031&10.007$\pm$0.018&AAA1&
13.58&12.55&\nodata&4&
PELS059 DH311
\\
56.036678&23.079908&12.000$\pm$0.019&11.336$\pm$0.026&11.109$\pm$0.019&AAA2&
16.85&15.43&13.21&1&
HCG141 SK590 T71 DH312
\\
56.038799&23.146400&13.393$\pm$0.019&12.741$\pm$0.027&12.489$\pm$0.020&AAA2&
\nodata&18.00&15.10&21&
HHJ186 DH313
\\
56.039993&24.589565&12.959$\pm$0.019&12.343$\pm$0.031&12.056$\pm$0.020&AAA2&
\nodata&17.09&14.37&5&
SK586 DH314
\\
56.041294&24.267807&12.456$\pm$0.019&11.770$\pm$0.028&11.530$\pm$0.020&AAA2&
\nodata&\nodata&13.48&22&
HCG140 DH315
\\
56.044811&25.627342&13.344$\pm$0.022&12.711$\pm$0.027&12.473$\pm$0.025&AAA1&
\nodata&17.98&14.97&7&
HHJ235 DH316
\\
56.046692&23.379330&9.956$\pm$0.016&9.512$\pm$0.021&9.408$\pm$0.020&AAA1&12.29&
11.45&10.53&1&
HII296 DH317
\\
56.049614&19.305391&11.954$\pm$0.019&11.253$\pm$0.014&11.048$\pm$0.013&AAA1&
\nodata&\nodata&13.33&22&
DH318
\\
56.050545&23.877096&13.461$\pm$0.020&12.867$\pm$0.030&12.566$\pm$0.019&AAA2&
\nodata&17.90&15.00&21&
HHJ217 DH319
\\
56.053902&24.031099&9.309$\pm$0.031&8.871$\pm$0.042&8.728$\pm$0.023&AAA1&11.77&
10.89&9.93&3&
HII298+9 Tr103
\\
56.057980&24.779388&9.530$\pm$0.021&9.172$\pm$0.031&9.062$\pm$0.020&AAA1&11.49&
10.79&10.02&1&
HII293 Tr098
\\
56.058186&25.537651&12.414$\pm$0.021&11.818$\pm$0.029&11.542$\pm$0.025&AAA1&
\nodata&16.60&13.85&20&
HCG138 SK579 DH320
\\
56.061119&24.101816&8.697$\pm$0.011&8.449$\pm$0.035&8.314$\pm$0.028&AAA1&11.36&
10.48&9.43&1&
HII303 Tr104
\\
56.063976&26.331230&9.705$\pm$0.021&9.310$\pm$0.027&9.269$\pm$0.020&AAA1&11.81&
11.07&\nodata&4&
PELS046 DH321 AKIII876
\\
56.068531&23.617830&12.741$\pm$0.019&12.119$\pm$0.027&11.886$\pm$0.019&AAA2&
\nodata&17.69&14.60&20&
HCG144 SK580 HHJ301 DH322
\\
56.073944&24.446377&12.601$\pm$0.015&11.932$\pm$0.027&11.686$\pm$0.020&AAA2&
\nodata&16.62&14.01&7&
HCG145 SK576 HHJ352 DH323
\\
56.079422&24.588455&13.341$\pm$0.019&12.699$\pm$0.029&12.437$\pm$0.020&AAA2&
19.37&17.83&14.93&12&
HCG146 T18B HHJ228 DH324
\\
56.083687&24.796156&9.339$\pm$0.019&8.996$\pm$0.030&8.900$\pm$0.018&AAA1&11.26&
10.60&9.85&3&
HII314 Tr108 DH325
\\
56.085445&24.772854&9.455$\pm$0.025&9.027$\pm$0.030&8.869$\pm$0.020&AAA1&11.92&
11.02&10.06&3&
HII320 Tr113 DH326
\\
56.086048&24.253031&14.039$\pm$0.020&13.406$\pm$0.028&13.099$\pm$0.020&AAA2&
\nodata&\nodata&16.00&21&
HHJ57
\\
56.086910&23.561136&12.874$\pm$0.019&12.238$\pm$0.027&12.010$\pm$0.019&AAA2&
\nodata&17.42&14.59&20&
HCG155 SK575 HHJ300 DH327
\\
56.091270&24.768408&10.828$\pm$0.019&10.197$\pm$0.028&10.070$\pm$0.020&AAA1&
14.08&13.01&11.70&10&
HII324 HCG147 DH328
\\
56.092247&23.181946&14.471$\pm$0.017&13.857$\pm$0.029&13.472$\pm$0.021&AAA2&
\nodata&\nodata&16.77&22&
DH329
\\
56.096096&24.068304&10.933$\pm$0.051&10.294$\pm$0.065&10.218$\pm$0.119&AAB1&
15.02&13.74&12.13&10&
HII335 HCG153 T73 DH330
\\
56.097450&25.358377&12.501$\pm$0.019&11.896$\pm$0.028&11.613$\pm$0.018&AAA1&
18.45&16.80&14.24&1&
HCG143 SK568 T19B HHJ348
\\
56.098110&24.132639&8.083$\pm$0.021&7.811$\pm$0.027&7.769$\pm$0.027&AAA1&9.52&
9.04&8.43&3&
HII338 HD23247 Tr118
\\
56.099941&21.405857&14.311$\pm$0.026&13.718$\pm$0.032&13.367$\pm$0.030&AAA1&
\nodata&\nodata&15.72&22&
DH332
\\
56.102833&24.864859&12.808$\pm$0.019&12.232$\pm$0.027&11.943$\pm$0.019&AAA2&
\nodata&17.52&14.35&20&
HCG148 SK569 HHJ307 DH333
\\
56.103378&24.768394&11.923$\pm$0.019&11.259$\pm$0.030&11.011$\pm$0.019&AAA2&
16.97&15.42&13.23&1&
HCG149 SK570 T42B DH334
\\
56.104469&25.567804&13.912$\pm$0.026&13.303$\pm$0.035&12.955$\pm$0.032&AAA1&
\nodata&19.12&15.67&7&
HHJ100
\\
56.106243&22.463919&15.174$\pm$0.042&14.612$\pm$0.058&14.243$\pm$0.060&AAA1&
\nodata&\nodata&17.23&22&
DH335
\\
56.106625&24.681362&12.525$\pm$0.019&11.946$\pm$0.031&11.651$\pm$0.019&AAA2&
18.17&16.66&14.01&1&
HCG150 SK567 B179 HHJ364
\\
56.107113&24.394674&7.588$\pm$0.007&7.528$\pm$0.037&7.470$\pm$0.017&AAA1&8.44&
8.17&7.86&3&
HII344 HD23246 Tr121
\\
56.109486&24.589705&9.835$\pm$0.019&9.389$\pm$0.027&9.266$\pm$0.017&AAA1&12.44&
11.60&99.99&14&
HII345 Tr122
\\
56.109921&26.041821&11.587$\pm$0.021&10.930$\pm$0.029&10.775$\pm$0.026&AAA1&
16.88&15.39&12.92&1&
HCG142 SK561 T10 DH337
\\
56.110554&24.486536&13.010$\pm$0.015&12.410$\pm$0.027&12.082$\pm$0.019&AAA2&
\nodata&17.94&14.71&7&
HHJ243 DH338
\\
56.111980&24.408831&12.392$\pm$0.015&11.711$\pm$0.027&11.450$\pm$0.019&AAA2&
\nodata&16.07&13.58&20&
HCG156 HHJ400 DH339
\\
56.113724&24.843962&10.913$\pm$0.021&10.248$\pm$0.031&10.015$\pm$0.022&AAA1&
15.44&14.02&12.07&16&
HII347 HCG154 T160 DH340
\\
56.114559&24.238113&13.552$\pm$0.019&12.951$\pm$0.028&12.658$\pm$0.020&AAA2&
\nodata&18.60&15.10&21&
HHJ190 DH341
\\
56.116299&23.999977&14.471$\pm$0.033&13.822$\pm$0.044&13.493$\pm$0.042&AAA1&
\nodata&\nodata&16.02&22&
DH342
\\
56.116707&24.171558&10.836$\pm$0.019&10.146$\pm$0.025&10.025$\pm$0.019&AAA1&
14.53&13.32&11.80&1&
HII357 HCG158
\\
56.117016&19.185043&10.002$\pm$0.013&9.537$\pm$0.017&9.418$\pm$0.018&AAA1&
\nodata&\nodata&10.54&22&
DH343
\\
56.125286&25.596395&11.882$\pm$0.021&11.182$\pm$0.032&10.973$\pm$0.022&AAA1&
\nodata&15.00&\nodata&21&
HCG152
\\
56.129253&22.254219&12.643$\pm$0.018&11.975$\pm$0.021&11.758$\pm$0.020&AAA1&
\nodata&\nodata&13.79&22&
SK571 DH344
\\
56.132133&23.590618&13.095$\pm$0.019&12.450$\pm$0.028&12.200$\pm$0.020&AAA2&
99.99&17.69&14.89&20&
SK564 HHJ265 DH345
\\
56.133255&23.875212&11.284$\pm$0.020&10.729$\pm$0.031&10.452$\pm$0.021&AAA2&
15.98&14.60&12.20&21&
HII370 SK562
\\
56.133984&25.136826&14.275$\pm$0.030&13.587$\pm$0.036&13.372$\pm$0.036&AAA1&
\nodata&19.30&15.90&21&
HHJ68
\\
56.137756&25.752707&13.388$\pm$0.026&12.740$\pm$0.031&12.491$\pm$0.026&AAA1&
\nodata&\nodata&15.11&22&
HCG157 DH346
\\
56.139523&26.248184&12.677$\pm$0.021&12.076$\pm$0.030&11.794$\pm$0.020&AAA1&
\nodata&17.00&14.20&21&
HHJ334 DH347
\\
56.147549&24.001354&11.552$\pm$0.019&10.845$\pm$0.031&10.654$\pm$0.017&AAA1&
15.85&14.48&99.99&20&
HII390
\\
56.149555&23.578363&15.003$\pm$0.021&14.340$\pm$0.029&14.021$\pm$0.025&AAA2&
\nodata&20.71&17.08&7&
HHJ5
\\
56.151157&23.503090&12.563$\pm$0.019&11.911$\pm$0.028&11.662$\pm$0.019&AAA2&
18.12&16.55&13.99&1&
HCG161 SK559 A23 HHJ344
\\
56.155899&25.137793&10.995$\pm$0.021&10.391$\pm$0.031&10.239$\pm$0.021&AAA1&
14.54&13.33&11.94&1&
HII380 DH349
\\
56.157349&24.427465&14.437$\pm$0.018&13.786$\pm$0.029&13.518$\pm$0.022&AAA2&
\nodata&19.51&16.22&7&
HHJ46 DH350
\\
56.157413&22.921038&11.903$\pm$0.019&11.235$\pm$0.023&11.036$\pm$0.018&AAA1&
\nodata&14.31&12.55&20&
HCG164
\\
56.162273&23.040415&13.394$\pm$0.015&12.801$\pm$0.027&12.500$\pm$0.024&AAA2&
\nodata&18.30&15.10&21&
HHJ189 DH351
\\
56.165276&22.113310&9.639$\pm$0.016&9.249$\pm$0.017&9.127$\pm$0.015&AAA1&11.88&
11.11&\nodata&4&
PELS038 AKIa071
\\
56.169800&24.818542&8.783$\pm$0.013&8.540$\pm$0.035&8.513$\pm$0.022&AAA1&10.39&
9.84&9.21&3&
HII405 HD23269 Tr131
\\
56.174259&22.464563&9.477$\pm$0.017&9.140$\pm$0.019&9.072$\pm$0.018&AAA1&11.50&
10.78&\nodata&4&
PELS034 DH352 AKIa072
\\
56.179878&25.875553&10.031$\pm$0.024&9.669$\pm$0.029&9.520$\pm$0.018&AAA1&12.62&
11.72&\nodata&4&
PELS044 DH353 AKIb200
\\
56.183105&25.499289&10.391$\pm$0.026&9.863$\pm$0.029&9.740$\pm$0.015&AAA1&13.09&
12.15&\nodata&4&
PELS041 AKIb199
\\
56.183250&24.231215&9.913$\pm$0.023&9.566$\pm$0.033&9.469$\pm$0.020&AAA1&12.20&
11.39&10.53&1&
HII430 Tr137
\\
56.192230&24.384195&14.675$\pm$0.021&14.104$\pm$0.029&13.788$\pm$0.027&AAA2&
\nodata&\nodata&16.50&21&
HHJ24
\\
56.197044&19.928274&14.769$\pm$0.033&14.252$\pm$0.043&13.925$\pm$0.043&AAA1&
\nodata&\nodata&16.76&22&
DH354
\\
56.197186&24.010527&13.194$\pm$0.019&12.575$\pm$0.026&12.325$\pm$0.024&AAA2&
99.99&17.50&14.60&21&
HHJ276 HCG167 DH355
\\
56.198265&26.600777&11.728$\pm$0.026&10.989$\pm$0.029&10.828$\pm$0.018&AAA1&
\nodata&\nodata&12.85&22&
DH356
\\
56.199333&24.214663&13.374$\pm$0.019&12.737$\pm$0.027&12.450$\pm$0.023&AAA2&
99.99&18.00&14.80&21&
HCG166 HHJ239 DH357
\\
56.200893&24.289503&5.447$\pm$0.021&5.476$\pm$0.035&5.496$\pm$0.007&EAA1&5.42&
5.46&5.45&3&
HII447 16Tau Celaeno HD23288
\\
56.209042&24.911133&11.131$\pm$0.015&10.393$\pm$0.025&10.341$\pm$0.019&AAA2&
14.64&13.43&12.00&1&
HII451 HCG168 DH358
\\
56.213482&23.268969&8.184$\pm$0.015&8.006$\pm$0.019&7.984$\pm$0.029&AAA1&9.26&
8.86&8.37&3&
HII470 HD23289 Tr149
\\
56.218887&24.113285&4.078$\pm$0.302&4.086$\pm$0.222&3.922$\pm$0.033&DDE1&3.58&
3.70&3.78&3&
HII468 17Tau Electra HD23302
\\
56.220917&26.142029&10.589$\pm$0.024&10.027$\pm$0.033&9.929$\pm$0.016&AAA1&13.49
&12.45&\nodata&4&
PELS137 AKIb205
\\
56.224304&23.921267&9.312$\pm$0.047&8.935$\pm$0.055&8.816$\pm$0.019&AAA1&11.58&
10.78&9.87&1&
HII476 Tr151
\\
56.225384&24.446379&13.617$\pm$0.019&12.979$\pm$0.027&12.750$\pm$0.020&AAA2&
\nodata&18.50&15.10&21&
HHJ183 DH360
\\
56.233303&23.931536&12.795$\pm$0.015&12.146$\pm$0.026&11.916$\pm$0.019&AAA2&
99.99&17.30&14.40&21&
HCG171 HHJ304
\\
56.234989&24.432623&9.218$\pm$0.021&8.945$\pm$0.029&8.866$\pm$0.017&AAA1&11.04&
10.42&9.69&13&
HII489 Tr153
\\
56.236198&23.606585&13.163$\pm$0.019&12.608$\pm$0.028&12.332$\pm$0.020&AAA2&
\nodata&17.60&14.60&21&
HHJ269 DH361
\\
56.241749&23.408674&13.272$\pm$0.015&12.664$\pm$0.027&12.360$\pm$0.020&AAA2&
\nodata&18.00&14.90&21&
HHJ223 DH362
\\
56.244091&23.928066&13.062$\pm$0.015&12.395$\pm$0.027&12.111$\pm$0.020&AAA2&
\nodata&17.50&14.60&21&
HHJ274 DH363
\\
56.245522&22.032455&8.520$\pm$0.005&8.349$\pm$0.029&8.278$\pm$0.017&AAA1&9.97&
9.48&\nodata&4&
PELS140 HD23312 TrS61 AKIa076
\\
56.245682&23.388947&11.274$\pm$0.015&10.389$\pm$0.998&10.480$\pm$0.019&AFA2&
15.16&13.85&99.99&2&
HII513 DH364
\\
56.247803&23.355124&14.274$\pm$0.016&13.692$\pm$0.027&13.384$\pm$0.020&AAA2&
\nodata&19.60&16.00&21&
HHJ54 DH365
\\
56.254707&24.778107&13.443$\pm$0.016&12.827$\pm$0.026&12.570$\pm$0.020&AAA2&
99.99&18.00&15.00&21&
HCG172 SK538 HHJ216 DH366
\\
56.255020&25.351633&13.948$\pm$0.026&13.383$\pm$0.035&13.040$\pm$0.030&AAA1&
\nodata&\nodata&15.70&22&
DH367
\\
56.256958&19.559372&8.404$\pm$0.013&8.225$\pm$0.027&8.152$\pm$0.015&AAA1&9.92&
9.42&\nodata&4&
PELS135
\\
56.261963&25.088852&13.743$\pm$0.021&13.161$\pm$0.039&12.851$\pm$0.020&AAA1&
\nodata&18.54&15.37&7&
HHJ139 DH368
\\
56.263603&23.839439&10.261$\pm$0.015&9.835$\pm$0.021&9.730$\pm$0.016&AAA1&12.87&
11.97&10.97&1&
HII522 DH369
\\
56.266689&25.257841&9.435$\pm$0.017&9.146$\pm$0.032&9.041$\pm$0.016&AAA1&11.43&
10.73&9.97&1&
HII514 DH370
\\
56.267509&26.679132&13.595$\pm$0.026&12.954$\pm$0.032&12.735$\pm$0.025&AAA1&
\nodata&\nodata&15.10&21&
HHJ185 DH371
\\
56.270782&23.768494&13.750$\pm$0.021&13.197$\pm$0.030&12.863$\pm$0.022&AAA2&
\nodata&19.30&15.60&21&
HHJ113 DH372
\\
56.272011&23.702707&8.205$\pm$0.021&8.041$\pm$0.011&8.000$\pm$0.015&AAA1&9.35&
8.96&8.49&3&
HII530 HD23326 Tr163
\\
56.272141&25.486446&12.376$\pm$0.024&11.717$\pm$0.029&11.484$\pm$0.016&AAA1&
\nodata&15.99&13.77&20&
SK534 HHJ381 DH373
\\
56.276005&28.705364&13.594$\pm$0.025&13.107$\pm$0.039&12.777$\pm$0.022&AAA1&
\nodata&\nodata&15.26&22&
DH374
\\
56.277229&24.263523&7.892$\pm$0.015&7.767$\pm$0.029&7.738$\pm$0.019&AAA1&8.92&
8.58&8.16&3&
HII531 HD23325 Tr162
\\
56.278255&23.614344&13.594$\pm$0.019&13.013$\pm$0.029&12.661$\pm$0.020&AAA2&
99.99&19.40&15.40&21&
HCG176 HHJ136
\\
56.284180&26.292517&9.947$\pm$0.023&9.509$\pm$0.029&9.443$\pm$0.016&AAA1&12.31&
11.49&\nodata&4&
PELS045 DH375 AKIII904
\\
56.286163&22.641857&13.346$\pm$0.019&12.734$\pm$0.024&12.483$\pm$0.020&AAA1&
\nodata&18.10&15.00&21&
HHJ204 BPL70 DH376
\\
56.287640&25.547020&13.663$\pm$0.024&12.989$\pm$0.033&12.715$\pm$0.018&AAA1&
\nodata&18.20&15.20&21&
HHJ164 DH377
\\
56.290581&24.839277&5.741$\pm$0.009&5.842$\pm$0.031&5.812$\pm$0.017&AAA1&5.58&
5.65&5.68&3&
HII541 18Tau HD23324 Tr166
\\
56.291157&21.704592&8.902$\pm$0.011&8.694$\pm$0.021&8.586$\pm$0.018&AAA1&10.52&
9.95&\nodata&4&
PELS040
\\
56.295063&23.049507&13.229$\pm$0.015&12.556$\pm$0.027&12.345$\pm$0.021&AAA2&
\nodata&17.81&15.35&20&
HCG186 SK535
\\
56.299938&24.586178&11.411$\pm$0.018&10.755$\pm$0.026&10.556$\pm$0.019&AAA2&
15.14&13.82&99.99&20&
HII554 DH378
\\
56.300629&23.364792&13.150$\pm$0.015&12.516$\pm$0.027&12.244$\pm$0.019&AAA2&
\nodata&17.64&14.91&20&
HCG185 SK532 HHJ255 DH379
\\
56.301788&22.697536&13.190$\pm$0.019&12.535$\pm$0.023&12.267$\pm$0.016&AAA1&
\nodata&17.80&15.00&21&
BPL71 SK533 HHJ254 DH380
\\
56.302097&24.467264&4.674$\pm$0.266&4.589$\pm$0.033&4.502$\pm$0.015&DEE1&4.20&
4.30&4.37&3&
HII563 19Tau Taygete HD23338
\\
56.302544&23.895882&14.830$\pm$0.018&14.214$\pm$0.030&13.883$\pm$0.023&AAA2&
\nodata&20.41&16.55&1&
HHJ14 PPL7
\\
56.304733&24.256607&14.077$\pm$0.020&13.439$\pm$0.028&13.168$\pm$0.026&AAA2&
99.99&19.80&15.60&21&
HCG180 HHJ118 DH381
\\
56.306339&25.087755&11.029$\pm$0.025&10.396$\pm$0.033&10.220$\pm$0.016&AAA1&
14.44&13.33&11.94&1&
HII559
\\
56.308006&26.588402&10.389$\pm$0.024&9.925$\pm$0.030&9.805$\pm$0.018&AAA1&12.92&
12.02&\nodata&4&
PELS047 DH382 AKIII908
\\
56.309212&25.088799&11.661$\pm$0.025&10.928$\pm$0.033&10.782$\pm$0.016&AAA1&
15.77&13.60&99.99&20&
HII566 HCG174
\\
56.313946&25.289476&9.709$\pm$0.025&9.323$\pm$0.040&9.228$\pm$0.020&AAA1&12.04&
11.26&10.35&1&
HII571
\\
56.315907&25.110260&11.872$\pm$0.023&11.223$\pm$0.029&11.028$\pm$0.017&AAA1&
99.99&15.61&13.27&20&
SK526 HHJ425
\\
56.317177&24.121185&12.480$\pm$0.018&11.854$\pm$0.027&11.627$\pm$0.023&AAA2&
\nodata&16.00&13.63&21&
HCG183 HHJ394 DH383
\\
56.318409&23.567165&14.434$\pm$0.017&13.805$\pm$0.029&13.516$\pm$0.021&AAA2&
\nodata&\nodata&16.38&22&
DH384
\\
56.319359&24.575708&12.316$\pm$0.019&11.651$\pm$0.028&11.430$\pm$0.019&AAA2&
17.75&16.18&13.70&1&
HCG181 B196 HHJ405 DH385
\\
56.320770&25.263279&12.027$\pm$0.023&11.421$\pm$0.030&11.179$\pm$0.018&AAA1&
17.85&16.20&13.52&1&
HCG178 SK525 A28 HHJ410
\\
56.325584&25.099545&11.473$\pm$0.023&10.791$\pm$0.030&10.651$\pm$0.017&AAA1&
15.73&14.37&12.65&1&
HII590 HCG179 SK524 T45
\\
56.336918&24.922075&8.079$\pm$0.011&7.933$\pm$0.081&7.838$\pm$0.017&AAA1&9.44&
9.00&8.43&3&
HII605 HD23351
\\
56.338284&23.727499&10.153$\pm$0.017&9.609$\pm$0.019&9.402$\pm$0.015&AAA1&13.88&
12.68&11.24&10&
HII625 Tr186
\\
56.340298&24.543709&13.252$\pm$0.015&12.617$\pm$0.028&12.312$\pm$0.019&AAA2&
\nodata&17.60&14.60&21&
HHJ273 DH388
\\
56.341225&26.478432&13.546$\pm$0.026&12.795$\pm$0.029&12.591$\pm$0.020&AAA1&
\nodata&\nodata&15.03&22&
DH389
\\
56.342480&23.471731&10.471$\pm$0.017&9.959$\pm$0.015&9.848$\pm$0.015&AAA1&13.42&
12.40&11.28&1&
HII636 Tr190 DH390
\\
56.347889&24.850800&11.925$\pm$0.018&11.212$\pm$0.026&11.037$\pm$0.019&AAA2&
16.81&15.28&13.14&1&
HII624 HCG188 HHJ436 DH391
\\
56.349140&21.877420&14.073$\pm$0.022&13.470$\pm$0.028&13.217$\pm$0.028&AAA1&
\nodata&\nodata&15.98&19&
BPL72
\\
56.350533&24.885977&8.686$\pm$0.011&8.572$\pm$0.041&8.419$\pm$0.017&AAA1&10.17&
9.65&9.05&3&
HII627 HD23352 Tr187
\\
56.353249&24.345961&13.169$\pm$0.015&12.514$\pm$0.027&12.245$\pm$0.019&AAA2&
\nodata&\nodata&14.41&22&
DH392
\\
56.358242&23.430206&10.318$\pm$0.022&9.818$\pm$0.026&9.704$\pm$0.023&EEE1&12.98&
12.04&10.91&1&
HII659 Tr197
\\
56.358902&24.035139&7.563$\pm$0.025&7.497$\pm$0.029&7.459$\pm$0.013&AAA1&8.26&
8.05&7.78&3&
HII652 HD23361 Tr195
\\
56.360634&22.525623&13.101$\pm$0.017&12.555$\pm$0.021&12.249$\pm$0.018&AAA1&
\nodata&17.40&14.70&21&
HHJ267 BPL73 DH393
\\
56.362411&24.224075&14.224$\pm$0.020&13.586$\pm$0.030&13.287$\pm$0.025&AAA2&
\nodata&18.60&15.80&21&
HHJ99
\\
56.364624&23.632532&14.114$\pm$0.017&13.539$\pm$0.029&13.261$\pm$0.020&AAA2&
\nodata&18.80&15.70&21&
HHJ106
\\
56.365524&23.170357&12.626$\pm$0.019&11.952$\pm$0.027&11.691$\pm$0.019&AAA2&
\nodata&16.88&14.25&20&
SK520
\\
56.370358&27.468779&12.073$\pm$0.025&11.453$\pm$0.028&11.188$\pm$0.020&AAA1&
\nodata&\nodata&13.19&22&
DH394
\\
56.373203&23.760529&10.971$\pm$0.998&10.401$\pm$0.033&10.341$\pm$0.035&FAA2&
14.94&13.64&12.12&1&
HII676 Tr203 HCG190 DH395
\\
56.374344&22.404209&15.210$\pm$0.042&14.656$\pm$0.055&14.268$\pm$0.059&AAA1&
\nodata&\nodata&17.16&19&
BPL74
\\
56.375916&24.312651&12.050$\pm$0.015&11.352$\pm$0.028&11.129$\pm$0.019&AAA2&
\nodata&15.74&13.35&1&
HII673
\\
56.387222&24.303242&11.061$\pm$0.016&10.397$\pm$0.035&10.220$\pm$0.077&AAA2&
14.91&13.52&12.02&1&
HII686 Tr206 HCG192
\\
56.391602&23.185205&13.861$\pm$0.020&13.292$\pm$0.028&13.007$\pm$0.020&AAA2&
\nodata&\nodata&15.78&22&
DH396
\\
56.393559&24.463299&7.852$\pm$0.013&7.710$\pm$0.065&7.670$\pm$0.013&AAA1&8.94&
8.59&8.33&3&
HII697 HD23375 Tr208
\\
56.397484&24.083210&8.921$\pm$0.024&8.673$\pm$0.032&8.562$\pm$0.020&AAA1&10.73&
10.11&9.37&3&
HII708 Tr213
\\
56.402985&24.651888&12.255$\pm$0.019&11.601$\pm$0.028&11.354$\pm$0.020&AAA2&
\nodata&16.66&13.83&7&
HCG194 HHJ380 DH397
\\
56.407410&24.335646&6.715$\pm$0.021&6.629$\pm$0.033&6.627$\pm$0.019&AAA1&7.38&
7.22&6.96&3&
HII717 HD23387 Tr215
\\
56.412647&25.224415&11.850$\pm$0.023&11.116$\pm$0.029&10.938$\pm$0.018&AAA1&
\nodata&14.76&12.75&20&
HCG196 SK510
\\
56.412983&22.073175&14.071$\pm$0.024&13.382$\pm$0.029&13.086$\pm$0.022&AAA1&
\nodata&\nodata&16.03&19&
BPL75
\\
56.413677&24.139048&13.959$\pm$0.020&13.337$\pm$0.027&13.061$\pm$0.026&AAA2&
\nodata&18.90&15.50&21&
HHJ130 DH398
\\
56.414200&23.754284&9.767$\pm$0.016&9.224$\pm$0.025&9.007$\pm$0.018&AAA1&13.47&
12.32&10.83&10&
HII738 Tr220
\\
56.417370&24.627245&8.624$\pm$0.021&8.337$\pm$0.053&8.294$\pm$0.019&AAA1&10.27&
9.71&9.05&3&
HII727
\\
56.419819&28.535042&14.078$\pm$0.023&13.505$\pm$0.036&13.177$\pm$0.025&AAA1&
\nodata&\nodata&16.06&22&
DH399
\\
56.422436&24.288599&8.360$\pm$0.009&8.123$\pm$0.043&8.040$\pm$0.021&AAA1&9.99&
9.46&8.79&3&
HII745
\\
56.423695&25.686813&11.780$\pm$0.023&11.066$\pm$0.029&10.881$\pm$0.020&AAA1&
16.77&15.30&13.00&1&
HCG195 T78 DH400
\\
56.424374&24.431513&9.801$\pm$0.026&9.528$\pm$0.033&9.398$\pm$0.020&AAA1&12.07&
11.30&10.42&1&
HII746
\\
56.425480&24.905998&8.286$\pm$0.009&8.040$\pm$0.041&7.939$\pm$0.033&AAA1&10.15&
9.50&8.82&13&
HII739 HD23386 Tr221
\\
56.426872&25.057091&11.267$\pm$0.023&10.654$\pm$0.032&10.504$\pm$0.019&AAA1&
14.46&13.40&12.11&1&
HII740
\\
56.429886&26.040777&13.254$\pm$0.026&12.562$\pm$0.029&12.326$\pm$0.020&AAA1&
\nodata&17.50&14.70&21&
HHJ264 DH401
\\
56.433640&24.074102&11.512$\pm$0.018&10.828$\pm$0.028&10.638$\pm$0.024&AAA2&
15.63&14.23&12.51&1&
HII762 Tr228a HCG200
\\
56.435040&24.220335&9.262$\pm$0.015&8.847$\pm$0.051&8.753$\pm$0.019&AAA1&11.27&
10.56&9.77&3&
HII761 Tr228
\\
56.438400&22.979160&15.425$\pm$0.054&14.716$\pm$0.058&14.485$\pm$0.071&AAA1&
\nodata&\nodata&17.61&19&
BPL76
\\
56.445538&21.747053&13.774$\pm$0.021&13.158$\pm$0.019&12.822$\pm$0.026&AAA1&
\nodata&19.10&15.50&21&
HHJ128
\\
56.453377&23.147167&6.701$\pm$0.007&6.732$\pm$0.009&6.816$\pm$0.995&AAF1&6.89&
6.85&6.78&3&
HII801 HD23410 Tr234
\\
56.453922&23.852869&11.500$\pm$0.019&10.854$\pm$0.030&10.701$\pm$0.017&AAA2&
15.74&14.27&12.51&1&
HII793 HCG201 DH402
\\
56.455212&25.412870&15.740$\pm$0.063&14.934$\pm$0.081&14.747$\pm$0.095&AAA1&
\nodata&\nodata&17.63&22&
DH403
\\
56.455654&24.418707&12.695$\pm$0.028&12.036$\pm$0.030&11.803$\pm$0.023&AAA1&
\nodata&\nodata&14.09&19&
BPL77
\\
56.456676&24.367701&4.059$\pm$0.276&4.122$\pm$0.033&3.986$\pm$0.009&DEE1&3.80&
3.87&3.88&3&
HII785 20Tau Maia HD23408
\\
56.460045&22.601679&16.243$\pm$0.103&15.528$\pm$0.112&15.024$\pm$0.109&ABB1&
\nodata&\nodata&18.73&19&
BPL78
\\
56.460346&23.873947&10.865$\pm$0.027&10.400$\pm$0.039&10.170$\pm$0.035&AAA1&
15.00&13.66&12.09&1&
HII799
\\
56.461048&24.151049&15.808$\pm$0.031&15.063$\pm$0.038&14.639$\pm$0.032&AAA2&
\nodata&\nodata&18.43&19&
BPL79
\\
56.465149&24.038902&7.456$\pm$0.025&7.362$\pm$0.033&7.332$\pm$0.007&AAA1&8.08&
7.88&7.63&3&
HII804 HD23409 Tr235
\\
56.466434&25.167200&13.682$\pm$0.021&13.053$\pm$0.032&12.811$\pm$0.022&AAA1&
\nodata&18.70&15.20&21&
HHJ166 BPL80 DH404
\\
56.469116&25.916685&12.830$\pm$0.023&12.181$\pm$0.030&11.904$\pm$0.019&AAA1&
\nodata&17.03&14.63&20&
SK499 DH405
\\
56.469345&25.861740&11.567$\pm$0.031&10.949$\pm$0.037&10.712$\pm$0.026&AAA1&
16.76&15.27&12.86&1&
HCG199 SK500 MT61 DH406
\\
56.469788&23.465073&13.262$\pm$0.019&12.589$\pm$0.027&12.326$\pm$0.019&AAA2&
99.99&18.08&15.08&20&
HCG202 SK504 HHJ227 DH407
\\
56.471653&25.215521&15.993$\pm$0.081&15.333$\pm$0.091&14.923$\pm$0.099&AAA1&
\nodata&\nodata&18.55&19&
BPL81
\\
56.474026&24.469128&11.460$\pm$0.019&10.820$\pm$0.028&10.569$\pm$0.019&AAA2&
\nodata&\nodata&12.86&22&
HII813 DH408
\\
56.476978&24.554506&5.755$\pm$0.023&5.826$\pm$0.045&5.777$\pm$0.011&AAA1&5.72&
5.76&5.74&3&
HII817 21 Tau Asterope HD23432 Tr240
\\
56.479099&24.223949&12.739$\pm$0.020&12.102$\pm$0.028&11.845$\pm$0.019&AAA2&
\nodata&\nodata&14.45&19&
BPL82
\\
56.487328&23.024780&13.407$\pm$0.019&12.796$\pm$0.027&12.578$\pm$0.019&AAA2&
99.99&17.90&15.10&21&
HCG205 HHJ199 DH410
\\
56.488621&25.186930&12.375$\pm$0.021&11.754$\pm$0.031&11.448$\pm$0.018&AAA1&
\nodata&\nodata&13.75&18&
SK497 HHJ379 BPL83 DH411
\\
56.490410&24.051449&14.717$\pm$0.022&14.119$\pm$0.031&13.787$\pm$0.024&AAA2&
\nodata&\nodata&16.50&21&
HHJ27
\\
56.491261&24.144756&14.584$\pm$0.022&13.994$\pm$0.032&13.677$\pm$0.022&AAA2&
\nodata&\nodata&16.57&22&
DH412
\\
56.494980&26.333887&14.094$\pm$0.023&13.494$\pm$0.032&13.184$\pm$0.027&AAA1&
\nodata&20.40&15.90&21&
HHJ67 DH413
\\
56.496639&23.813051&13.959$\pm$0.016&13.353$\pm$0.027&13.078$\pm$0.020&AAA2&
\nodata&18.70&15.50&21&
HHJ127
\\
56.503819&22.208258&14.825$\pm$0.030&14.208$\pm$0.043&13.887$\pm$0.037&AAA1&
\nodata&20.46&16.83&7&
HHJ11 BPL84
\\
56.509327&25.611307&12.140$\pm$0.023&11.577$\pm$0.029&11.310$\pm$0.019&AAA1&
99.99&16.04&13.67&20&
SK491 HHJ399
\\
56.511482&23.737392&9.923$\pm$0.018&9.455$\pm$0.021&9.257$\pm$0.017&AAA1&13.86&
12.61&11.05&1&
HII870 Tr249
\\
56.512035&24.527870&6.399$\pm$0.019&6.484$\pm$0.039&6.433$\pm$0.019&AAA1&6.41&
6.43&6.41&3&
HII859 22Tau HD23441 Tr247
\\
56.512310&24.682182&14.091$\pm$0.020&13.462$\pm$0.029&13.139$\pm$0.020&AAA2&
\nodata&\nodata&16.02&19&
BPL85 DH414
\\
56.514374&24.349207&13.479$\pm$0.019&12.867$\pm$0.028&12.557$\pm$0.019&AAA2&
\nodata&\nodata&15.20&19&
HCG206 BPL86 DH415
\\
56.515266&25.874746&13.568$\pm$0.028&12.934$\pm$0.035&12.705$\pm$0.021&AAA1&
\nodata&18.20&15.10&21&
HHJ182 DH416
\\
56.515877&25.453009&11.644$\pm$0.023&10.985$\pm$0.032&10.770$\pm$0.017&AAA1&
15.94&14.51&12.69&5&
SK490 DH417
\\
56.516426&24.385818&14.484$\pm$0.021&13.856$\pm$0.028&13.501$\pm$0.021&AAA2&
\nodata&\nodata&16.27&19&
BPL87
\\
56.517178&23.405537&10.540$\pm$0.016&10.014$\pm$0.019&9.836$\pm$0.015&AAA1&14.00
&12.78&11.62&10&
HII882 Tr256 DH418
\\
56.517899&23.928019&12.769$\pm$0.019&12.075$\pm$0.029&11.816$\pm$0.017&AAA2&
\nodata&16.70&13.90&21&
HHJ363
\\
56.518993&24.165571&14.060$\pm$0.020&13.452$\pm$0.029&13.184$\pm$0.020&AAA2&
\nodata&\nodata&15.83&19&
BPL88
\\
56.521854&22.981655&11.330$\pm$0.015&10.654$\pm$0.019&10.500$\pm$0.016&AAA1&
\nodata&14.21&12.34&20&
HCG214 DH419
\\
56.523464&24.612358&12.346$\pm$0.021&11.663$\pm$0.031&11.442$\pm$0.021&AAA2&
\nodata&15.81&13.50&5&
SK488
\\
56.526863&25.419909&13.799$\pm$0.021&13.265$\pm$0.035&12.837$\pm$0.025&AAA1&
\nodata&17.60&15.10&21&
HHJ194
\\
56.527061&24.567419&10.793$\pm$0.025&10.236$\pm$0.028&10.113$\pm$0.017&AAA1&
13.86&12.79&11.59&1&
HII879 Tr253 DH420
\\
56.527157&23.838995&11.949$\pm$0.019&11.147$\pm$0.030&10.919$\pm$0.018&AAA2&
\nodata&15.20&13.10&21&
HHJ435
\\
56.527699&22.392721&12.072$\pm$0.017&11.418$\pm$0.017&11.171$\pm$0.016&AAA1&
\nodata&\nodata&13.67&19&
BPL89
\\
56.528744&24.562807&10.907$\pm$0.057&10.336$\pm$0.025&10.286$\pm$0.065&AAA1&
14.13&13.05&11.75&1&
HII883 Tr257 HCG208
\\
56.531269&24.374380&11.706$\pm$0.019&11.042$\pm$0.028&10.860$\pm$0.019&AAA2&
16.04&14.71&12.83&1&
HII890 HCG210
\\
56.532360&24.866802&10.057$\pm$0.026&9.521$\pm$0.033&9.357$\pm$0.021&AAA1&13.10&
12.08&10.87&1&
HII885 DH421
\\
56.534836&23.347523&11.255$\pm$0.022&10.413$\pm$0.035&10.403$\pm$0.051&AAA2&
15.02&13.79&12.26&1&
HII915 HCG215
\\
56.536221&24.675913&13.583$\pm$0.019&12.978$\pm$0.028&12.706$\pm$0.019&AAA2&
\nodata&\nodata&15.25&19&
HCG209 BPL90 DH422
\\
56.539562&26.138826&9.968$\pm$0.025&9.420$\pm$0.030&9.301$\pm$0.019&AAA1&12.93&
11.88&\nodata&9&
AK1B288 DH423
\\
56.539940&22.710398&12.779$\pm$0.019&12.149$\pm$0.023&11.903$\pm$0.021&AAA1&
\nodata&17.30&14.64&20&
HCG217 SK487 HHJ297 BPL91
\\
56.541157&21.097990&13.111$\pm$0.019&12.442$\pm$0.021&12.247$\pm$0.023&AAA1&
\nodata&\nodata&14.62&22&
DH425
\\
56.541225&24.673626&11.468$\pm$0.019&10.853$\pm$0.030&10.593$\pm$0.020&AAA2&
16.72&15.20&12.81&1&
HII906 HCG211 SK482 DH426
\\
56.541874&23.340015&8.969$\pm$0.011&8.704$\pm$0.013&8.659$\pm$0.013&AAA1&10.76&
10.15&9.46&13&
HII923 Tr270 DH427
\\
56.542019&26.002575&14.148$\pm$0.030&13.471$\pm$0.036&13.244$\pm$0.031&AAA1&
\nodata&19.30&15.80&21&
HHJ80
\\
56.548939&24.622314&10.062$\pm$0.023&9.629$\pm$0.032&9.545$\pm$0.017&AAA1&12.58&
11.71&99.99&3&
HII916 Tr268 DH428
\\
56.552853&23.128571&7.573$\pm$0.007&7.327$\pm$0.015&7.285$\pm$0.019&AAA1&9.26&
8.66&8.00&3&
HII948 HD23464
\\
56.553612&24.054377&11.428$\pm$0.019&10.785$\pm$0.031&10.600$\pm$0.019&AAA2&
15.46&14.20&12.48&1&
HII930 DH429
\\
56.554153&27.036673&14.252$\pm$0.028&13.633$\pm$0.041&13.449$\pm$0.034&AAA1&
\nodata&\nodata&15.98&22&
DH430
\\
56.557697&22.705519&13.367$\pm$0.020&12.791$\pm$0.021&12.461$\pm$0.021&AAA1&
\nodata&18.30&15.00&21&
HHJ200 BPL92 DH431
\\
56.559753&23.850643&14.003$\pm$0.020&13.334$\pm$0.035&12.969$\pm$0.021&AAA2&
\nodata&\nodata&16.00&21&
HHJ56 DH432
\\
56.565964&22.044744&12.766$\pm$0.017&12.115$\pm$0.019&11.835$\pm$0.017&AAA1&
\nodata&\nodata&14.52&19&
BPL93
\\
56.566689&24.189842&7.294$\pm$0.019&7.179$\pm$0.021&7.115$\pm$0.017&AAA1&8.29&
7.97&7.57&3&
HII956 HD23479 Tr281b
\\
56.570175&24.440922&13.658$\pm$0.019&12.992$\pm$0.029&12.769$\pm$0.020&AAA2&
\nodata&\nodata&15.21&19&
BPL94
\\
56.574726&24.686003&12.557$\pm$0.015&11.913$\pm$0.027&11.688$\pm$0.019&AAA2&
\nodata&16.20&13.90&21&
HHJ367 BPL95 DH433
\\
56.574959&23.486664&8.911$\pm$0.007&8.589$\pm$0.021&8.504$\pm$0.017&AAA1&11.42&
10.58&9.59&1&
HII975 Tr285
\\
56.580566&20.879786&9.995$\pm$0.016&9.609$\pm$0.015&9.519$\pm$0.015&AAA1&12.39&
11.55&\nodata&4&
PELS050 DH434 AKIII551
\\
56.580856&23.015503&14.102$\pm$0.020&13.492$\pm$0.029&13.178$\pm$0.021&AAA2&
\nodata&\nodata&16.10&21&
HHJ47 BPL96 DH435
\\
56.580929&26.043274&11.811$\pm$0.015&11.146$\pm$0.017&10.968$\pm$0.015&AAA1&
\nodata&14.74&12.82&5&
SK474 DH436
\\
56.581600&23.948381&4.233$\pm$0.240&4.309$\pm$0.154&4.220$\pm$0.005&DBE1&4.12&
4.18&4.16&3&
HII980 23Tau Merope HD23480
\\
56.582733&24.983765&12.838$\pm$0.019&12.194$\pm$0.027&11.965$\pm$0.020&AAA2&
\nodata&17.40&14.40&21&
HHJ303 BPL97 DH437
\\
56.585312&24.785480&11.340$\pm$0.015&10.688$\pm$0.030&10.538$\pm$0.019&AAA2&
15.30&13.96&12.34&1&
HII974 Tr284 SK475 DH438
\\
56.588970&24.564585&13.983$\pm$0.016&13.349$\pm$0.027&13.075$\pm$0.021&AAA2&
\nodata&18.90&15.70&21&
HHJ105 BPL98 DH439
\\
56.589149&23.085882&14.628$\pm$0.021&14.010$\pm$0.030&13.703$\pm$0.022&AAA2&
\nodata&\nodata&16.40&21&
HHJ33
\\
56.590103&23.066956&13.652$\pm$0.019&13.007$\pm$0.028&12.748$\pm$0.020&AAA2&
\nodata&\nodata&15.59&22&
DH440
\\
56.592484&23.878132&13.047$\pm$0.019&12.366$\pm$0.028&12.088$\pm$0.018&AAA2&
\nodata&\nodata&14.72&22&
DH441
\\
56.594479&24.570177&9.274$\pm$0.016&8.994$\pm$0.012&8.923$\pm$0.013&AAA1&11.06&
10.41&9.71&13&
HII996 HD282963 Tr289
\\
56.595936&24.605053&13.612$\pm$0.016&12.994$\pm$0.028&12.716$\pm$0.020&AAA2&
\nodata&\nodata&15.25&19&
BPL99 DH442
\\
56.596302&24.343422&16.315$\pm$0.039&15.610$\pm$0.054&15.064$\pm$0.042&AAA2&
\nodata&\nodata&19.07&19&
BPL100
\\
56.597767&24.030945&13.687$\pm$0.020&13.092$\pm$0.029&12.853$\pm$0.019&AAA2&
99.99&18.50&15.10&21&
HCG218 HHJ195 DH443
\\
56.598846&26.573168&13.705$\pm$0.023&13.133$\pm$0.029&12.844$\pm$0.025&AAA1&
\nodata&18.60&15.20&21&
HHJ175 DH444
\\
56.600491&24.503605&14.752$\pm$0.021&14.137$\pm$0.032&13.836$\pm$0.023&AAA2&
\nodata&\nodata&16.46&19&
BPL101
\\
56.602627&24.479601&13.413$\pm$0.019&12.776$\pm$0.028&12.538$\pm$0.019&AAA2&
\nodata&18.30&14.80&21&
HHJ249 BPL102 DH445
\\
56.604877&21.438231&12.371$\pm$0.015&11.746$\pm$0.014&11.517$\pm$0.015&AAA1&
\nodata&\nodata&14.10&22&
DH446
\\
56.605766&24.160105&12.021$\pm$0.019&11.369$\pm$0.027&11.136$\pm$0.019&AAA2&
\nodata&15.83&13.37&1&
HCG219 A2 HHJ429
\\
56.612507&24.453926&12.935$\pm$0.019&12.254$\pm$0.027&12.047$\pm$0.019&AAA2&
\nodata&17.10&14.20&21&
HHJ326 BPL103 DH447
\\
56.613670&24.255032&7.119$\pm$0.007&7.111$\pm$0.009&7.125$\pm$0.019&AAA1&7.51&
7.40&7.28&3&
HII1028 HD23489 Tr295
\\
56.613968&25.135563&9.366$\pm$0.014&9.063$\pm$0.015&8.993$\pm$0.013&AAA1&11.17&
10.52&9.81&13&
HII1015 HD282952 TrR13 DH448
\\
56.615376&23.812695&13.704$\pm$0.020&13.020$\pm$0.028&12.648$\pm$0.020&AAA2&
\nodata&19.10&15.20&21&
HHJ161
\\
56.615738&23.592699&10.594$\pm$0.015&10.007$\pm$0.019&9.821$\pm$0.015&AAA1&14.23
&13.02&11.52&10&
HII1039 Tr297 HCG223 DH449
\\
56.617348&22.816141&14.146$\pm$0.020&13.508$\pm$0.033&13.228$\pm$0.030&AAA1&
\nodata&19.70&15.80&21&
HHJ87 BPL104
\\
56.618378&24.433918&9.638$\pm$0.016&9.270$\pm$0.015&9.159$\pm$0.013&AAA1&11.85&
11.10&10.26&1&
HII1032 Tr296 DH450
\\
56.619274&24.758995&11.507$\pm$0.015&10.820$\pm$0.027&10.647$\pm$0.019&AAA2&
15.73&14.34&12.59&1&
HII1029 HCG222 SK472 B212
\\
56.623833&21.038082&13.461$\pm$0.021&12.805$\pm$0.023&12.550$\pm$0.023&AAA1&
\nodata&\nodata&15.55&22&
DH452
\\
56.629223&23.026346&14.616$\pm$0.022&13.997$\pm$0.029&13.728$\pm$0.023&AAA2&
\nodata&19.77&16.47&7&
HHJ30 DH453
\\
56.629910&24.117350&11.290$\pm$0.019&10.650$\pm$0.029&10.338$\pm$0.039&AAA2&
15.60&14.21&12.39&1&
HII1061 HCG224 SK469 DH454
\\
56.630470&22.305523&13.384$\pm$0.019&12.823$\pm$0.026&12.503$\pm$0.026&AAA1&
\nodata&18.10&15.20&21&
HHJ160 BPL105
\\
56.633430&24.476236&15.235$\pm$0.025&14.687$\pm$0.036&14.243$\pm$0.029&AAA2&
\nodata&\nodata&17.15&19&
BPL106
\\
56.636131&22.338285&13.620$\pm$0.019&12.876$\pm$0.024&12.649$\pm$0.021&AAA1&
\nodata&17.53&15.18&20&
SK471
\\
56.636597&19.291840&13.316$\pm$0.020&12.725$\pm$0.030&12.422$\pm$0.020&AAA1&
\nodata&\nodata&15.22&22&
DH455
\\
56.636982&23.305323&11.637$\pm$0.019&10.955$\pm$0.027&10.782$\pm$0.019&AAA2&
16.03&14.61&12.72&1&
HII1081 SK468 DH456
\\
56.642521&23.624010&7.241$\pm$0.013&7.116$\pm$0.015&7.067$\pm$0.013&AAA1&8.53&
8.16&7.65&3&
HII1084 HD23512 Tr311
\\
56.647205&23.411737&11.692$\pm$0.019&10.974$\pm$0.028&10.723$\pm$0.018&AAA2&
16.25&14.77&12.85&1&
HII1103 HCG229 SK466 HHJ434
\\
56.648033&24.026529&13.693$\pm$0.019&13.109$\pm$0.029&12.779$\pm$0.020&AAA2&
\nodata&19.00&15.40&21&
HHJ140 DH458
\\
56.649624&23.967031&11.511$\pm$0.019&10.829$\pm$0.028&10.656$\pm$0.019&AAA2&
15.42&14.02&99.99&3&
HII1094 HCG227
\\
56.650269&23.071491&12.913$\pm$0.019&12.302$\pm$0.027&12.054$\pm$0.019&AAA2&
\nodata&17.70&15.01&20&
SK465 HHJ282 DH459
\\
56.655285&24.343527&10.123$\pm$0.016&9.524$\pm$0.012&9.400$\pm$0.013&AAA1&13.35&
12.25&10.97&1&
HII1100 HCG228 Tr318 DH460
\\
56.656994&23.787771&8.925$\pm$0.009&8.583$\pm$0.009&8.527$\pm$0.013&AAA1&10.93&
10.20&9.43&3&
HII1117 HD282975 Tr324
\\
56.657391&24.747698&10.217$\pm$0.016&9.784$\pm$0.015&9.669$\pm$0.017&AAA1&12.75&
11.83&10.89&1&
HII1095 Tr316 DH462
\\
56.659985&22.919804&8.479$\pm$0.017&8.291$\pm$0.017&8.153$\pm$0.017&AAA1&9.92&
9.42&8.84&3&
HII1132 HD23514
\\
56.661587&24.959629&9.105$\pm$0.014&8.851$\pm$0.012&8.763$\pm$0.013&AAA1&10.86&
10.25&9.55&13&
HII1101 HD282954 Tr319
\\
56.662018&24.520338&11.099$\pm$0.019&10.479$\pm$0.013&10.274$\pm$0.059&AAA2&
14.48&13.29&11.89&1&
HII1110 Tr322
\\
56.663857&24.103243&8.432$\pm$0.015&8.230$\pm$0.017&8.191$\pm$0.010&AAA1&9.75&
9.29&8.75&3&
HII1122 HD23511 Tr327
\\
56.664104&24.029688&10.454$\pm$0.016&9.986$\pm$0.015&9.859$\pm$0.018&AAA1&13.30&
12.32&11.24&1&
HII1124 Tr329 DH463
\\
56.666656&23.110371&8.473$\pm$0.019&8.280$\pm$0.011&8.243$\pm$0.019&AAA1&9.85&
9.37&8.83&3&
HII1139 HD23513 Tr331
\\
56.667671&23.497789&10.031$\pm$0.017&9.496$\pm$0.019&9.340$\pm$0.016&AAA1&13.18&
12.18&10.93&1&
HII1136 Tr330
\\
56.667728&25.731573&12.927$\pm$0.019&12.268$\pm$0.023&12.020$\pm$0.026&AAA1&
\nodata&17.11&14.46&20&
SK461 HHJ316 DH464
\\
56.667778&24.931030&11.090$\pm$0.998&10.562$\pm$0.031&10.384$\pm$0.063&FAA2&
15.48&14.09&12.30&18&
HII1114 HCG231 SK463 T44B
\\
56.668331&22.844402&14.110$\pm$0.022&13.483$\pm$0.033&13.184$\pm$0.031&AAA1&
\nodata&\nodata&15.97&19&
BPL107
\\
56.679070&24.414103&15.545$\pm$0.027&14.853$\pm$0.036&14.420$\pm$0.027&AAA2&
\nodata&\nodata&18.27&19&
BPL108
\\
56.679920&23.622803&14.093$\pm$0.019&13.395$\pm$0.028&13.100$\pm$0.020&AAA2&
\nodata&18.90&15.70&21&
HHJ104 DH466
\\
56.681622&23.995152&12.471$\pm$0.017&11.856$\pm$0.019&11.575$\pm$0.020&AAA1&
\nodata&\nodata&13.75&22&
DH467
\\
56.686565&24.749580&14.224$\pm$0.017&13.628$\pm$0.029&13.354$\pm$0.022&AAA2&
\nodata&19.50&15.90&21&
HHJ75 BPL109
\\
56.690704&25.458466&12.810$\pm$0.019&12.194$\pm$0.021&11.958$\pm$0.021&AAA1&
18.43&16.87&14.21&1&
HCG233 SK458 T25B HHJ319
\\
56.696087&22.914593&9.307$\pm$0.018&9.032$\pm$0.018&8.928$\pm$0.017&AAA1&11.12&
10.48&9.77&3&
HII1182
\\
56.696598&25.348185&13.406$\pm$0.020&12.765$\pm$0.027&12.532$\pm$0.025&AAA1&
\nodata&18.70&15.00&21&
HHJ208 DH469
\\
56.701302&24.301674&12.564$\pm$0.019&11.918$\pm$0.029&11.717$\pm$0.020&AAA2&
17.77&16.24&13.57&1&
HCG236 J311
\\
56.703251&23.068752&12.331$\pm$0.019&11.695$\pm$0.029&11.423$\pm$0.019&AAA2&
\nodata&16.04&13.83&20&
HCG245 HHJ370 DH470
\\
56.705051&24.600019&11.904$\pm$0.015&11.203$\pm$0.027&10.996$\pm$0.020&AAA2&
16.63&15.10&13.05&1&
HII1173 HCG237 HHJ431 DH471
\\
56.708675&23.532301&13.227$\pm$0.020&12.658$\pm$0.029&12.391$\pm$0.019&AAA2&
99.99&17.80&14.80&21&
HCG240 HHJ253 DH472
\\
56.709076&22.211847&14.443$\pm$0.028&13.776$\pm$0.033&13.478$\pm$0.038&AAA1&
\nodata&\nodata&16.42&19&
BPL110
\\
56.710571&23.239195&8.868$\pm$0.027&8.593$\pm$0.015&8.546$\pm$0.018&AEA1&10.48&
9.94&9.27&3&
HII1200 Tr346
\\
56.719055&24.288054&14.269$\pm$0.020&13.625$\pm$0.033&13.327$\pm$0.027&AAA2&
\nodata&\nodata&15.85&19&
BPL111
\\
56.719170&23.645351&13.181$\pm$0.015&12.475$\pm$0.027&12.198$\pm$0.019&AAA2&
\nodata&18.50&14.80&21&
HHJ247 DH473
\\
56.720680&24.252222&15.125$\pm$0.023&14.507$\pm$0.033&14.120$\pm$0.029&AAA2&
\nodata&\nodata&17.04&19&
BPL112
\\
56.721920&22.880943&10.232$\pm$0.016&9.820$\pm$0.021&9.719$\pm$0.017&AAA1&12.62&
11.74&99.99&3&
HII1220
\\
56.723351&24.287514&12.055$\pm$0.018&11.463$\pm$0.027&11.212$\pm$0.023&AAA2&
\nodata&16.27&13.53&12&
HCG244 SK454 BPL113 DH474
\\
56.723911&23.583599&9.350$\pm$0.016&9.092$\pm$0.017&8.996$\pm$0.018&AAA1&11.17&
10.55&9.85&1&
HII1215 Tr350
\\
56.725128&25.245825&12.409$\pm$0.023&11.710$\pm$0.029&11.489$\pm$0.020&AAA1&
17.84&16.19&13.76&1&
HCG241 SK453 B267 BPL114
\\
56.728638&24.466667&14.957$\pm$0.019&14.330$\pm$0.030&14.002$\pm$0.027&AAA2&
\nodata&\nodata&16.74&19&
BPL115 DH476
\\
56.728828&24.796349&9.274$\pm$0.017&9.005$\pm$0.029&8.977$\pm$0.017&AAA1&11.13&
10.49&9.79&13&
HII1207 HD282962 Tr348 DH477
\\
56.730438&23.380434&14.191$\pm$0.021&13.589$\pm$0.028&13.332$\pm$0.020&AAA2&
\nodata&19.40&15.80&21&
HHJ95 DH479
\\
56.730465&24.188021&13.765$\pm$0.019&13.170$\pm$0.029&12.882$\pm$0.024&AAA2&
\nodata&\nodata&15.68&19&
BPL116 DH478
\\
56.730633&25.858217&14.727$\pm$0.033&14.045$\pm$0.040&13.782$\pm$0.044&AAA1&
\nodata&\nodata&16.40&21&
HHJ31
\\
56.732403&23.940079&13.234$\pm$0.019&12.599$\pm$0.027&12.314$\pm$0.020&AAA2&
\nodata&18.40&14.70&21&
HHJ257 DH480
\\
56.737892&23.250679&12.007$\pm$0.019&11.348$\pm$0.028&11.128$\pm$0.019&AAA2&
\nodata&15.47&13.24&5&
HCG247 SK452 HHJ415 DH481
\\
56.742352&23.560827&13.683$\pm$0.020&13.081$\pm$0.028&12.854$\pm$0.020&AAA2&
\nodata&18.10&15.20&21&
HHJ174 DH482
\\
56.743908&24.461136&13.025$\pm$0.015&12.383$\pm$0.027&12.150$\pm$0.020&AAA2&
\nodata&\nodata&14.56&19&
HCG246 HHJ296 BPL117 DH483
\\
56.744938&24.368979&13.151$\pm$0.015&12.518$\pm$0.027&12.233$\pm$0.021&AAA2&
\nodata&\nodata&14.76&19&
BPL118
\\
56.747135&24.028616&13.005$\pm$0.018&12.400$\pm$0.028&12.110$\pm$0.024&AAA2&
\nodata&17.60&14.40&21&
HHJ299 DH484
\\
56.747517&24.520117&6.699$\pm$0.023&6.733$\pm$0.057&6.692$\pm$0.019&AAA1&6.85&
6.83&6.76&3&
HII1234 HD23568 Tr354
\\
56.747803&24.879539&13.222$\pm$0.020&12.655$\pm$0.028&12.351$\pm$0.024&AAA2&
\nodata&18.40&14.90&21&
HHJ222 BPL119 DH485
\\
56.751217&24.473555&13.158$\pm$0.015&12.550$\pm$0.026&12.252$\pm$0.020&AAA2&
\nodata&17.80&14.80&21&
HHJ252 BPL120
\\
56.754147&24.982632&13.208$\pm$0.020&12.596$\pm$0.028&12.335$\pm$0.024&AAA2&
\nodata&\nodata&14.96&19&
BPL121
\\
56.755909&23.494984&10.037$\pm$0.017&9.637$\pm$0.021&9.534$\pm$0.018&AAA1&12.28&
11.45&10.58&1&
HII1275 Tr361 DH486
\\
56.757675&24.224529&14.972$\pm$0.022&14.411$\pm$0.034&14.098$\pm$0.029&AAA2&
\nodata&\nodata&16.87&19&
BPL122
\\
56.759743&23.543383&14.312$\pm$0.020&13.670$\pm$0.029&13.352$\pm$0.020&AAA2&
\nodata&\nodata&16.61&22&
DH487
\\
56.760567&25.229342&15.667$\pm$0.067&14.885$\pm$0.053&14.649$\pm$0.074&AAA1&
\nodata&\nodata&17.14&19&
BPL123
\\
56.764782&24.819933&7.537$\pm$0.015&7.367$\pm$0.035&7.334$\pm$0.023&AAA1&8.63&
8.27&7.83&3&
HII1266 HD23567 Tr359b
\\
56.764931&24.159710&11.603$\pm$0.018&10.885$\pm$0.027&10.717$\pm$0.024&AAA2&
15.92&14.56&12.72&18&
HII1280 HCG249 T27B DH488
\\
56.765728&23.616325&11.561$\pm$0.015&10.851$\pm$0.027&10.596$\pm$0.019&AAA2&
17.03&15.35&12.89&1&
HII1286 HCG251 SK444 DH489
\\
56.765804&20.195889&11.521$\pm$0.013&10.823$\pm$0.017&10.679$\pm$0.013&AAA1&
\nodata&\nodata&12.79&22&
DH490
\\
56.767551&23.995174&7.770$\pm$0.005&7.658$\pm$0.049&7.642$\pm$0.017&AAA1&8.66&
8.36&8.02&3&
HII1284 HD23585 Tr365
\\
56.769783&25.380619&12.179$\pm$0.023&11.534$\pm$0.029&11.262$\pm$0.018&AAA1&
17.91&16.35&13.61&1&
HCG248 SK443 B180 HHJ390
\\
56.773621&20.010380&14.179$\pm$0.025&13.524$\pm$0.032&13.282$\pm$0.034&AAA1&
\nodata&\nodata&16.16&22&
DH492
\\
56.773762&24.667715&15.469$\pm$0.025&14.870$\pm$0.041&14.505$\pm$0.037&AAA2&
\nodata&\nodata&17.56&19&
BPL124
\\
56.778252&23.715170&10.421$\pm$0.019&9.995$\pm$0.022&9.839$\pm$0.016&AAA1&13.33&
12.33&11.25&1&
HII1298 Tr369
\\
56.780609&23.226339&11.178$\pm$0.019&10.271$\pm$0.089&10.397$\pm$0.057&AAA2&
14.71&13.52&12.09&1&
HII1305 HCG255 DH493
\\
56.782818&24.393866&14.013$\pm$0.016&13.433$\pm$0.029&13.102$\pm$0.021&AAA2&
\nodata&\nodata&15.71&19&
BPL125 DH494
\\
56.783916&24.306835&12.781$\pm$0.015&12.184$\pm$0.026&11.901$\pm$0.019&AAA2&
\nodata&16.95&14.26&7&
HCG253 SK440 BPL126 DH495
\\
56.784630&22.552736&15.392$\pm$0.051&14.834$\pm$0.067&14.428$\pm$0.080&AAA1&
\nodata&\nodata&17.41&19&
BPL127
\\
56.785580&23.710819&10.720$\pm$0.019&10.097$\pm$0.022&9.902$\pm$0.018&AAA1&14.86
&13.51&99.99&2&
HII1306 Tr370a HCG256
\\
56.789215&24.259703&14.480$\pm$0.020&13.917$\pm$0.029&13.563$\pm$0.026&AAA2&
\nodata&19.71&16.26&7&
HHJ37 BPL128 DH496
\\
56.789314&23.742186&11.548$\pm$0.015&10.923$\pm$0.026&10.656$\pm$0.019&AAA2&
16.69&15.22&12.85&1&
HII1321 HCG257 DH497
\\
56.789635&23.432364&13.913$\pm$0.020&13.364$\pm$0.028&13.053$\pm$0.020&AAA2&
\nodata&\nodata&15.71&22&
DH498
\\
56.791893&24.276672&8.533$\pm$0.019&8.329$\pm$0.033&8.282$\pm$0.019&AAA1&9.93&
9.46&8.92&3&
HII1309 HD23584 Tr372
\\
56.795921&24.231030&14.314$\pm$0.020&13.690$\pm$0.030&13.389$\pm$0.026&AAA2&
\nodata&19.34&16.03&7&
HCG254 BPL129
\\
56.799099&24.225414&14.865$\pm$0.021&14.229$\pm$0.032&13.881$\pm$0.027&AAA2&
\nodata&\nodata&16.98&19&
BPL130
\\
56.799419&24.231649&14.055$\pm$0.020&13.485$\pm$0.029&13.134$\pm$0.026&AAA2&
\nodata&19.52&15.89&7&
HHJ92 BPL131 DH499
\\
56.800392&24.475582&16.186$\pm$0.031&15.530$\pm$0.050&15.047$\pm$0.041&AAA2&
\nodata&\nodata&18.81&19&
BPL132
\\
56.806374&23.714310&10.624$\pm$0.017&10.148$\pm$0.022&10.009$\pm$0.016&AAA1&
13.55&12.53&11.43&1&
HII1332 Tr378
\\
56.806915&23.831503&11.943$\pm$0.015&11.335$\pm$0.026&11.086$\pm$0.019&AAA2&
17.13&15.78&13.31&1&
HCG258 SK437 B363 DH500
\\
56.811691&25.371840&10.046$\pm$0.025&9.515$\pm$0.029&9.517$\pm$0.020&AAA1&12.48&
11.63&\nodata&4&
PELS142 DH501 AKIb356
\\
56.813702&25.115416&12.388$\pm$0.023&11.760$\pm$0.029&11.485$\pm$0.018&AAA1&
\nodata&16.48&13.82&7&
SK432 HHJ376 BPL133 DH502
\\
56.814060&23.435032&13.425$\pm$0.020&12.858$\pm$0.027&12.501$\pm$0.019&AAA2&
\nodata&18.10&15.00&21&
HHJ203 DH503
\\
56.814346&24.391975&13.702$\pm$0.016&13.082$\pm$0.028&12.810$\pm$0.021&AAA2&
\nodata&\nodata&15.51&19&
BPL134
\\
56.815548&22.354769&13.222$\pm$0.019&12.682$\pm$0.020&12.374$\pm$0.019&AAA1&
\nodata&\nodata&15.13&19&
HCG267 BPL135 HHJ211
\\
56.818508&24.747318&13.407$\pm$0.019&12.797$\pm$0.028&12.508$\pm$0.025&AAA2&
\nodata&\nodata&15.21&19&
BPL136
\\
56.819008&24.128347&7.770$\pm$0.015&7.542$\pm$0.055&7.486$\pm$0.013&AAA1&9.11&
8.64&8.09&3&
HII1338 HD23608 Tr381
\\
56.824661&24.375467&16.238$\pm$0.035&15.591$\pm$0.052&15.182$\pm$0.048&AAA2&
\nodata&\nodata&18.96&19&
BPL137
\\
56.825268&24.390772&10.490$\pm$0.025&9.831$\pm$0.029&9.719$\pm$0.017&AAA1&13.85&
12.70&11.33&1&
HII1348 Tr383 DH504
\\
56.825546&24.230921&13.184$\pm$0.018&12.576$\pm$0.029&12.285$\pm$0.024&AAA2&
\nodata&\nodata&15.01&19&
BPL138 DH505
\\
56.825562&24.036524&11.021$\pm$0.018&10.268$\pm$0.061&10.191$\pm$0.024&AAA2&
15.42&14.02&12.14&1&
HII1355 HCG262
\\
56.830624&24.139126&7.767$\pm$0.023&7.627$\pm$0.035&7.639$\pm$0.013&AAA1&8.52&
8.27&7.97&3&
HII1362 HD23607 Tr390
\\
56.836803&25.086767&12.106$\pm$0.025&11.365$\pm$0.036&11.136$\pm$0.016&AAA1&
\nodata&15.93&13.52&20&
SK428 HHJ417 DH506
\\
56.837021&25.525862&8.720$\pm$0.019&8.463$\pm$0.053&8.435$\pm$0.029&AAA1&10.41&
9.85&\nodata&4&
PELS060 HD23598 AKIb365
\\
56.837345&23.803366&6.848$\pm$0.011&6.920$\pm$0.013&6.895$\pm$0.011&AAA1&7.07&
7.04&7.01&3&
HII1380 HD23632 Tr397
\\
56.837662&24.116304&6.228$\pm$0.009&6.248$\pm$0.025&6.257$\pm$0.015&AAA1&6.34&
6.32&6.30&3&
HII1375 24Tau HD23629 Tr395
\\
56.840977&25.897928&11.927$\pm$0.016&11.225$\pm$0.017&11.028$\pm$0.015&AAA1&
\nodata&15.20&13.10&5&
SK424 DH507
\\
56.841373&26.379892&13.474$\pm$0.021&12.889$\pm$0.021&12.562$\pm$0.025&AAA1&
\nodata&18.20&14.90&21&
HHJ219 DH508
\\
56.843243&24.238590&14.113$\pm$0.016&13.512$\pm$0.029&13.210$\pm$0.024&AAA2&
\nodata&\nodata&16.02&19&
BPL139
\\
56.843552&22.519772&14.249$\pm$0.024&13.680$\pm$0.027&13.372$\pm$0.034&AAA1&
\nodata&\nodata&16.18&19&
BPL140
\\
56.844494&23.735275&13.305$\pm$0.019&12.688$\pm$0.028&12.438$\pm$0.019&AAA2&
\nodata&17.50&\nodata&21&
HCG266 DH509
\\
56.844746&23.032822&14.868$\pm$0.022&14.268$\pm$0.030&14.008$\pm$0.022&AAA2&
\nodata&\nodata&16.50&21&
HHJ23
\\
56.845417&22.922121&7.618$\pm$0.013&7.543$\pm$0.011&7.520$\pm$0.015&AAA1&8.38&
8.12&7.83&3&
HII1407 HD23610 TrS108
\\
56.845722&24.848948&12.690$\pm$0.018&12.100$\pm$0.028&11.851$\pm$0.024&AAA2&
\nodata&17.16&14.36&7&
HCG261 SK425 HHJ335 BPL141
\\
56.846786&22.244535&11.684$\pm$0.016&11.019$\pm$0.021&10.838$\pm$0.015&AAA1&
15.93&14.54&12.72&1&
HCG274 SK429 T30B
\\
56.849384&23.149191&12.939$\pm$0.019&12.323$\pm$0.028&12.072$\pm$0.018&AAA2&
\nodata&17.33&14.51&7&
HCG270 SK427 HHJ275 DH511
\\
56.849895&22.710384&15.343$\pm$0.049&14.839$\pm$0.071&14.524$\pm$0.081&AAA1&
\nodata&\nodata&17.87&19&
BPL142
\\
56.850220&24.588472&7.154$\pm$0.017&7.044$\pm$0.007&7.003$\pm$0.013&AAA1&7.92&
7.71&7.45&3&
HII1384 HD23628 Tr399
\\
56.851677&23.914713&7.143$\pm$0.011&7.159$\pm$0.015&7.137$\pm$0.011&AAA1&7.31&
7.24&7.11&3&
HII1397 HD23631 Tr402
\\
56.854614&24.254812&13.926$\pm$0.016&13.346$\pm$0.028&13.055$\pm$0.025&AAA2&
\nodata&19.10&15.10&21&
HHJ198 BPL143
\\
56.855595&24.049170&12.649$\pm$0.015&12.038$\pm$0.026&11.808$\pm$0.024&AAA2&
\nodata&\nodata&13.79&22&
HHJ427 DH512
\\
56.857452&25.142515&12.357$\pm$0.017&11.710$\pm$0.017&11.446$\pm$0.018&AAA1&
18.68&16.91&13.98&1&
HCG263 SK423 T6B BPL144 DH513
\\
56.857658&22.349335&11.212$\pm$0.039&10.575$\pm$0.050&10.372$\pm$0.035&EEE1&
16.53&14.98&12.22&1&
HCG275 T18
\\
56.861523&23.634071&13.141$\pm$0.021&12.580$\pm$0.028&12.288$\pm$0.020&AAA2&
99.99&17.80&14.70&21&
HCG269 HHJ263 DH514
\\
56.861771&23.678368&7.406$\pm$0.032&7.370$\pm$0.021&7.343$\pm$0.017&AAA1&7.95&
7.79&7.61&3&
HII1425 HD23643 Tr410
\\
56.867142&23.448219&12.809$\pm$0.019&12.138$\pm$0.028&11.901$\pm$0.019&AAA2&
\nodata&17.11&14.32&20&
SK417 HHJ315 DH515
\\
56.868343&26.534967&13.260$\pm$0.018&12.661$\pm$0.021&12.386$\pm$0.019&AAA1&
\nodata&\nodata&15.15&22&
DH516
\\
56.868435&24.675905&13.734$\pm$0.016&13.145$\pm$0.027&12.873$\pm$0.025&AAA2&
\nodata&\nodata&15.30&19&
BPL145 DH517
\\
56.869934&22.376574&11.444$\pm$0.019&10.789$\pm$0.022&10.596$\pm$0.018&AAA1&
\nodata&14.60&12.55&5&
HCG276 SK418
\\
56.871189&24.105122&2.735$\pm$0.240&2.735$\pm$0.214&2.636$\pm$0.234&DCD1&2.78&
2.87&2.88&3&
HII1432 25Tau Alcyone HD23630
\\
56.872746&24.288340&6.635$\pm$0.015&6.641$\pm$0.021&6.607$\pm$0.019&AAA1&6.90&
6.83&6.74&3&
HII1431 HD23642 Tr413
\\
56.874683&23.554222&14.775$\pm$0.021&14.143$\pm$0.028&13.820$\pm$0.022&AAA2&
\nodata&\nodata&16.62&11&
HHJ16
\\
56.877377&26.279125&12.918$\pm$0.019&12.258$\pm$0.022&12.041$\pm$0.018&AAA1&
\nodata&17.00&14.40&21&
HCG260 HHJ310 DH518
\\
56.877476&24.370550&12.253$\pm$0.015&11.571$\pm$0.026&11.371$\pm$0.024&AAA2&
\nodata&15.87&13.60&7&
HCG273 HHJ408
\\
56.877678&25.225277&15.020$\pm$0.043&14.350$\pm$0.057&14.218$\pm$0.075&AAA1&
\nodata&\nodata&16.57&19&
BPL146
\\
56.879707&21.180962&13.702$\pm$0.018&13.147$\pm$0.026&12.820$\pm$0.025&AAA1&
\nodata&\nodata&15.49&22&
DH519
\\
56.883312&24.173588&13.710$\pm$0.017&13.100$\pm$0.028&12.833$\pm$0.026&AAA2&
\nodata&\nodata&15.44&19&
BPL147
\\
56.889400&23.692505&11.760$\pm$0.019&11.132$\pm$0.028&10.929$\pm$0.019&AAA2&
17.21&15.74&13.16&1&
HCG277 SK413 T105 HHJ424
\\
56.890320&24.684223&10.807$\pm$0.017&10.244$\pm$0.013&10.128$\pm$0.018&AAA1&
13.94&12.86&11.62&1&
HII1454 HCG278 DH521
\\
56.892330&25.718382&13.285$\pm$0.019&12.669$\pm$0.024&12.425$\pm$0.022&AAA1&
\nodata&17.70&14.80&21&
HHJ238 DH522
\\
56.892342&21.746843&10.530$\pm$0.021&10.013$\pm$0.020&9.895$\pm$0.016&AAA1&13.46
&12.43&\nodata&4&
PELS066
\\
56.893787&24.039755&13.690$\pm$0.016&13.104$\pm$0.028&12.801$\pm$0.025&AAA2&
\nodata&\nodata&15.12&22&
DH523
\\
56.894920&22.801352&13.018$\pm$0.019&12.382$\pm$0.023&12.147$\pm$0.020&AAA1&
\nodata&\nodata&14.84&19&
HCG284 HHJ278 BPL148 DH524
\\
56.896706&25.543968&11.705$\pm$0.016&11.019$\pm$0.015&10.834$\pm$0.018&AAA1&
\nodata&14.62&12.77&5&
SK410 DH525
\\
56.899403&24.874151&13.665$\pm$0.019&13.092$\pm$0.028&12.839$\pm$0.024&AAA2&
\nodata&18.78&15.31&7&
HCG279 HHJ157 BPL149
\\
56.900127&23.474146&14.150$\pm$0.020&13.546$\pm$0.027&13.284$\pm$0.020&AAA2&
\nodata&19.20&15.90&21&
HHJ73 DH526
\\
56.906883&24.406471&13.705$\pm$0.999&13.102$\pm$0.031&12.833$\pm$0.999&UAU2&
\nodata&\nodata&15.39&19&
BPL150
\\
56.908363&23.468056&11.081$\pm$0.019&10.544$\pm$0.053&10.325$\pm$0.057&AAA2&
14.77&13.51&12.10&1&
HII1512 Tr428a DH527
\\
56.908524&24.819742&12.573$\pm$0.018&11.937$\pm$0.027&11.697$\pm$0.024&AAA2&
\nodata&16.35&13.86&20&
SK409 HHJ360 BPL151 DH528
\\
56.908653&24.891832&11.459$\pm$0.018&10.785$\pm$0.027&10.608$\pm$0.024&AAA2&
15.55&14.22&12.50&18&
HII1485 HCG280 B271 DH529
\\
56.912544&24.606226&15.634$\pm$0.024&14.984$\pm$0.036&14.632$\pm$0.036&AAA2&
\nodata&\nodata&17.73&19&
BPL152
\\
56.913971&24.458933&13.050$\pm$0.015&12.440$\pm$0.026&12.162$\pm$0.024&AAA2&
\nodata&17.56&14.74&7&
HCG282 HHJ272 BPL153 DH530
\\
56.915768&23.001301&14.126$\pm$0.019&13.547$\pm$0.029&13.218$\pm$0.021&AAA2&
\nodata&18.73&15.68&7&
HHJ94
\\
56.918228&24.301937&11.142$\pm$0.015&10.521$\pm$0.027&10.342$\pm$0.024&AAA2&
15.31&13.97&12.30&1&
HII1516 HCG283
\\
56.918537&24.364594&9.340$\pm$0.017&9.071$\pm$0.013&8.953$\pm$0.016&AAA1&11.17&
10.51&9.79&13&
HII1514 HD282967 Tr430
\\
56.920734&22.930014&10.057$\pm$0.016&9.511$\pm$0.021&9.356$\pm$0.016&AAA1&13.58&
12.49&11.14&1&
HII1553 HCG290
\\
56.921581&23.740294&11.379$\pm$0.019&10.753$\pm$0.029&10.570$\pm$0.018&AAA2&
15.26&13.98&12.37&10&
HII1532 HCG286 SK405 B270
\\
56.922657&23.971945&11.066$\pm$0.016&10.461$\pm$0.014&10.312$\pm$0.018&AAA1&
14.85&13.58&12.11&1&
HII1531 Tr435 HCG285 DH532
\\
56.928513&28.316530&14.271$\pm$0.028&13.606$\pm$0.033&13.293$\pm$0.037&AAA1&
\nodata&\nodata&16.22&22&
DH533
\\
56.932789&26.224201&13.718$\pm$0.021&13.104$\pm$0.030&12.824$\pm$0.029&AAA1&
\nodata&\nodata&15.76&22&
DH534
\\
56.933502&24.065710&15.109$\pm$0.020&14.483$\pm$0.031&14.192$\pm$0.028&AAA2&
\nodata&\nodata&16.69&6&
HHJ26 DH535
\\
56.936035&22.212326&14.784$\pm$0.036&14.181$\pm$0.042&13.833$\pm$0.043&AAA1&
\nodata&20.00&16.45&7&
HHJ15 BPL154
\\
56.936039&23.700907&13.573$\pm$0.020&12.941$\pm$0.028&12.698$\pm$0.019&AAA2&
\nodata&18.20&15.14&6&
HHJ152 DH536
\\
56.936115&22.398155&13.513$\pm$0.023&12.844$\pm$0.026&12.578$\pm$0.023&AAA1&
\nodata&\nodata&15.42&19&
HCG299 HHJ163 BPL155
\\
56.941284&24.633736&13.457$\pm$0.016&12.845$\pm$0.028&12.544$\pm$0.024&AAA2&
\nodata&\nodata&15.23&19&
HCG287 HHJ168 BPL156
\\
56.943283&24.050699&12.185$\pm$0.015&11.529$\pm$0.026&11.327$\pm$0.024&AAA2&
\nodata&\nodata&13.45&6&
HHJ438
\\
56.949383&25.226257&13.007$\pm$0.019&12.384$\pm$0.021&12.088$\pm$0.020&AAA1&
\nodata&18.03&14.70&20&
SK398 HHJ266 BPL157 DH537
\\
56.949680&22.555561&11.438$\pm$0.023&10.792$\pm$0.021&10.538$\pm$0.016&AAA1&
16.82&15.25&12.81&1&
HCG298 SK399 T83 HHJ433
\\
56.950462&23.218140&9.760$\pm$0.016&9.436$\pm$0.021&9.324$\pm$0.015&AAA1&11.92&
11.15&10.33&1&
HII1593 Tr444
\\
56.957409&24.428701&13.540$\pm$0.015&12.939$\pm$0.028&12.693$\pm$0.024&AAA2&
\nodata&18.18&15.23&7&
HCG292 HHJ202 BPL158 DH538
\\
56.962280&24.505226&12.347$\pm$0.015&11.679$\pm$0.026&11.467$\pm$0.023&AAA2&
17.72&16.13&13.78&7&
HCG295 HHJ389 BPL159 DH539
\\
56.966473&23.663397&13.895$\pm$0.020&13.321$\pm$0.028&13.067$\pm$0.020&AAA2&
\nodata&19.00&15.55&6&
HHJ122 DH540
\\
56.968838&23.941282&8.853$\pm$0.019&8.639$\pm$0.021&8.574$\pm$0.016&AAA1&10.41&
9.87&9.24&3&
HII1613 HD282973 Tr448
\\
56.970276&22.992798&13.040$\pm$0.019&12.440$\pm$0.029&12.160$\pm$0.020&AAA2&
\nodata&17.64&14.96&20&
SK394 HHJ258 BPL160 DH541
\\
56.975632&22.657190&13.737$\pm$0.024&13.172$\pm$0.026&12.880$\pm$0.024&AAA1&
\nodata&18.20&15.30&21&
HHJ145 BPL161
\\
56.980289&23.318333&12.998$\pm$0.019&12.362$\pm$0.028&12.149$\pm$0.019&AAA2&
\nodata&17.33&14.70&20&
HCG302 SK392 HHJ289 DH542
\\
56.985966&24.258871&14.197$\pm$0.016&13.568$\pm$0.028&13.308$\pm$0.021&AAA2&
\nodata&\nodata&15.91&19&
BPL162
\\
56.986000&26.530914&11.899$\pm$0.015&11.291$\pm$0.022&11.028$\pm$0.018&AAA1&
\nodata&15.80&13.30&21&
HHJ423 DH543
\\
56.989990&26.629278&10.132$\pm$0.015&9.710$\pm$0.019&9.609$\pm$0.015&AAA1&12.61&
11.72&\nodata&4&
PELS143
\\
56.991753&22.114201&15.315$\pm$0.051&14.764$\pm$0.069&14.319$\pm$0.066&AAA1&
\nodata&\nodata&17.61&19&
BPL163
\\
56.997372&24.593704&14.486$\pm$0.017&13.920$\pm$0.030&13.602$\pm$0.022&AAA2&
\nodata&\nodata&16.15&19&
BPL164 DH544
\\
56.998894&24.731342&10.952$\pm$0.015&10.321$\pm$0.015&10.159$\pm$0.016&AAA1&
14.71&13.51&12.00&17&
HII1653 HCG300 DH545
\\
56.998959&22.641808&11.843$\pm$0.021&11.312$\pm$0.021&11.002$\pm$0.016&AAA1&
\nodata&16.70&13.90&21&
HHJ365 BPL165
\\
57.020718&23.403799&14.845$\pm$0.021&14.251$\pm$0.028&13.940$\pm$0.023&AAA2&
\nodata&20.17&16.57&7&
HHJ21 DH546
\\
57.023800&22.636011&13.279$\pm$0.026&12.713$\pm$0.022&12.399$\pm$0.018&AAA1&
99.99&17.90&15.00&21&
HCG314 HHJ210 DH547
\\
57.024258&23.034147&12.431$\pm$0.019&11.788$\pm$0.028&11.550$\pm$0.019&AAA2&
17.85&16.16&13.74&1&
HCG309 SK385 T154 HHJ375 DH548
\\
57.027660&24.001932&13.417$\pm$0.019&12.851$\pm$0.028&12.544$\pm$0.020&AAA2&
\nodata&18.00&15.02&6&
HHJ240 DH549
\\
57.029949&24.142099&8.220$\pm$0.009&7.987$\pm$0.003&7.939$\pm$0.009&AAA1&9.83&
9.28&8.64&3&
HII1726 HD23713 Tr486
\\
57.031975&25.315348&11.167$\pm$0.017&10.501$\pm$0.013&10.336$\pm$0.015&AAA1&
\nodata&\nodata&12.26&22&
DH550
\\
57.033176&23.739923&13.033$\pm$0.019&12.427$\pm$0.028&12.181$\pm$0.019&AAA2&
99.99&17.30&14.50&21&
HCG307 HHJ288 DH551
\\
57.036713&25.029392&12.201$\pm$0.013&11.484$\pm$0.013&11.254$\pm$0.018&AAA1&
\nodata&\nodata&13.55&19&
BPL167
\\
57.037277&23.706537&13.613$\pm$0.020&13.009$\pm$0.029&12.767$\pm$0.019&AAA2&
\nodata&18.40&15.26&6&
HHJ156 DH552
\\
57.038399&23.977999&13.521$\pm$0.020&12.904$\pm$0.027&12.647$\pm$0.020&AAA2&
\nodata&17.90&15.10&6&
HHJ225 DH553
\\
57.042397&23.988985&14.415$\pm$0.021&13.790$\pm$0.030&13.512$\pm$0.021&AAA2&
\nodata&\nodata&16.43&22&
DH555
\\
57.042400&23.001144&11.808$\pm$0.016&11.172$\pm$0.025&11.004$\pm$0.016&AAA1&
\nodata&\nodata&12.87&22&
DH554
\\
57.042969&19.302561&10.943$\pm$0.021&10.348$\pm$0.027&10.217$\pm$0.018&AAA1&
\nodata&\nodata&12.14&22&
DH556
\\
57.045776&23.507023&11.531$\pm$0.019&10.874$\pm$0.029&10.686$\pm$0.019&AAA2&
15.47&14.10&12.48&1&
HII1756 SK378 DH557
\\
57.047558&20.778521&13.121$\pm$0.018&12.499$\pm$0.022&12.242$\pm$0.018&AAA1&
\nodata&\nodata&15.01&22&
DH558
\\
57.051865&26.583826&11.148$\pm$0.013&10.489$\pm$0.017&10.360$\pm$0.017&AAA1&
\nodata&13.80&\nodata&21&
HCG304 DH559
\\
57.055473&23.979725&13.265$\pm$0.019&12.667$\pm$0.027&12.387$\pm$0.019&AAA2&
18.85&17.81&14.83&1&
HCG311 T155 DH560
\\
57.056450&24.318428&7.526$\pm$0.009&7.393$\pm$0.015&7.352$\pm$0.017&AAA1&8.63&
8.27&7.83&3&
HII1762 HD23733 Tr493
\\
57.057373&23.633196&13.006$\pm$0.019&12.385$\pm$0.028&12.108$\pm$0.018&AAA2&
\nodata&17.72&14.79&20&
HCG315 SK374 HHJ281 DH561
\\
57.059570&24.264124&15.246$\pm$0.020&14.621$\pm$0.033&14.243$\pm$0.026&AAA2&
\nodata&\nodata&17.33&19&
BPL169
\\
57.063499&23.434900&13.417$\pm$0.020&12.791$\pm$0.028&12.565$\pm$0.019&AAA2&
\nodata&17.60&14.90&21&
HHJ232
\\
57.063622&23.701002&12.669$\pm$0.019&12.043$\pm$0.027&11.778$\pm$0.018&AAA2&
\nodata&16.80&14.10&21&
HHJ336 DH562
\\
57.064503&25.243538&13.964$\pm$0.021&13.349$\pm$0.022&12.987$\pm$0.024&AAA1&
\nodata&\nodata&15.61&19&
BPL170 DH563
\\
57.067009&23.587627&13.562$\pm$0.019&12.976$\pm$0.027&12.652$\pm$0.019&AAA2&
\nodata&18.90&15.30&21&
HHJ151 DH564
\\
57.068169&26.334990&13.200$\pm$0.022&12.570$\pm$0.022&12.292$\pm$0.023&AAA1&
\nodata&17.50&\nodata&21&
HCG305
\\
57.068428&22.544590&11.553$\pm$0.016&10.899$\pm$0.020&10.695$\pm$0.015&AAA1&
\nodata&\nodata&12.73&23&
HCG318
\\
57.069267&26.503345&13.417$\pm$0.017&12.845$\pm$0.022&12.549$\pm$0.023&AAA1&
\nodata&18.20&15.00&21&
HHJ215 DH565
\\
57.070267&25.215170&8.137$\pm$0.007&7.912$\pm$0.013&7.862$\pm$0.015&AAA1&9.60&
9.13&8.55&3&
HII1766 HD23732
\\
57.070457&23.636806&9.041$\pm$0.018&8.817$\pm$0.013&8.736$\pm$0.018&AAA1&10.69&
10.13&9.48&3&
HII1797 Tr500
\\
57.071342&23.890385&9.264$\pm$0.033&8.976$\pm$0.024&8.891$\pm$0.018&AAA1&11.02&
10.40&9.72&1&
HII1794 HD282972 Tr499
\\
57.072041&24.504429&11.509$\pm$0.015&10.861$\pm$0.028&10.688$\pm$0.020&AAA2&
15.69&14.29&99.99&2&
HII1785 HCG312 DH566
\\
57.072330&23.806593&13.647$\pm$0.019&13.086$\pm$0.027&12.784$\pm$0.019&AAA2&
\nodata&18.40&15.26&6&
HHJ188
\\
57.073349&22.067030&13.446$\pm$0.023&12.860$\pm$0.024&12.612$\pm$0.025&AAA1&
\nodata&17.80&15.10&21&
HHJ187 BPL171
\\
57.073719&25.047886&9.593$\pm$0.013&9.256$\pm$0.015&9.158$\pm$0.016&AAA1&11.66&
10.94&10.15&1&
HII1776 Tr495 DH567
\\
57.079185&24.420275&16.023$\pm$0.030&15.273$\pm$0.045&14.953$\pm$0.041&AAA2&
\nodata&\nodata&18.30&19&
BPL172
\\
57.082642&23.603336&12.385$\pm$0.019&11.707$\pm$0.029&11.472$\pm$0.018&AAA2&
\nodata&\nodata&13.65&22&
DH568
\\
57.084534&24.915321&12.495$\pm$0.019&11.858$\pm$0.027&11.596$\pm$0.020&AAA2&
18.77&17.09&14.11&1&
HCG313 SK371 T23 BPL173
\\
57.085754&23.517082&14.420$\pm$0.020&13.825$\pm$0.030&13.509$\pm$0.021&AAA2&
\nodata&\nodata&16.47&22&
HCG321 DH570
\\
57.086723&23.421272&5.504$\pm$0.023&5.590$\pm$0.025&5.560$\pm$0.009&AAA1&5.38&
5.45&5.46&3&
HII1823 HD23753 Tr506
\\
57.089699&24.578793&13.816$\pm$0.016&13.214$\pm$0.028&12.959$\pm$0.021&AAA2&
\nodata&\nodata&15.49&19&
BPL174 DH571
\\
57.094372&22.872700&12.344$\pm$0.016&11.726$\pm$0.022&11.484$\pm$0.018&AAA1&
17.64&16.14&13.67&1&
HCG323 SK370 A91 BPL175 DH572
\\
57.094582&23.461969&13.636$\pm$0.019&13.031$\pm$0.029&12.810$\pm$0.020&AAA2&
\nodata&18.50&15.20&21&
HHJ171 DH573
\\
57.094868&23.972546&11.394$\pm$0.019&10.755$\pm$0.032&10.511$\pm$0.020&AAA2&
16.34&14.84&12.66&1&
HII1827 HCG319 SK369
\\
57.095013&24.814903&12.890$\pm$0.015&12.278$\pm$0.027&12.020$\pm$0.019&AAA2&
\nodata&17.10&14.48&7&
SK368 HHJ309 BPL176 DH574
\\
57.096794&28.659973&11.411$\pm$0.018&10.723$\pm$0.019&10.557$\pm$0.014&AAA1&
\nodata&\nodata&12.93&22&
DH575
\\
57.098423&24.376467&14.921$\pm$0.020&14.337$\pm$0.032&13.941$\pm$0.026&AAA2&
\nodata&\nodata&16.80&19&
BPL177
\\
57.099663&23.135681&14.086$\pm$0.020&13.500$\pm$0.028&13.152$\pm$0.020&AAA2&
\nodata&\nodata&15.88&22&
DH576
\\
57.103413&22.407301&11.707$\pm$0.018&11.106$\pm$0.021&10.859$\pm$0.015&AAA1&
16.99&15.44&13.03&1&
HCG325 SK367 T86 HHJ420
\\
57.105152&24.240564&12.853$\pm$0.015&12.252$\pm$0.027&11.990$\pm$0.019&AAA2&
\nodata&17.63&14.44&20&
HCG322 SK363 HHJ314 BPL178
\\
57.106274&22.211596&11.383$\pm$0.018&10.785$\pm$0.021&10.602$\pm$0.015&AAA1&
\nodata&\nodata&12.36&23&
HCG329
\\
57.108486&25.244755&11.963$\pm$0.017&11.333$\pm$0.017&11.089$\pm$0.015&AAA1&
\nodata&\nodata&13.43&22&
HCG317 DH578
\\
57.109024&24.048445&8.985$\pm$0.015&8.719$\pm$0.015&8.663$\pm$0.015&AAA1&10.57&
10.01&9.39&3&
HII1856 HD282971 Tr514
\\
57.110798&23.191612&12.185$\pm$0.015&11.598$\pm$0.026&11.361$\pm$0.020&AAA2&
\nodata&17.87&14.45&20&
HCG332 SK362 HHJ339
\\
57.116787&23.300774&10.515$\pm$0.021&9.964$\pm$0.025&9.836$\pm$0.015&AAA1&13.69&
12.66&11.43&1&
HII1883 Tr520 HCG331 DH579
\\
57.123997&23.968334&13.916$\pm$0.020&13.300$\pm$0.028&13.023$\pm$0.020&AAA2&
99.99&19.30&15.50&21&
HCG328 HHJ132
\\
57.125381&24.345591&6.614$\pm$0.007&6.595$\pm$0.007&6.563$\pm$0.011&AAA1&7.08&
6.95&6.79&3&
HII1876 HD23763 Tr518
\\
57.129375&24.281488&12.247$\pm$0.019&11.595$\pm$0.030&11.340$\pm$0.019&AAA2&
17.56&15.97&13.58&12&
HCG324 VM46 HHJ404 BPL180 DH580
\\
57.132645&24.033014&13.731$\pm$0.020&13.116$\pm$0.027&12.846$\pm$0.021&AAA2&
99.99&18.30&15.10&21&
HCG327 HHJ197 DH581
\\
57.140739&24.033060&13.777$\pm$0.020&13.175$\pm$0.029&12.931$\pm$0.021&AAA2&
\nodata&18.20&15.43&6&
HHJ184 DH582
\\
57.143806&23.434818&9.197$\pm$0.021&8.980$\pm$0.025&8.868$\pm$0.018&AAA1&10.95&
10.34&9.66&13&
HII1924
\\
57.145004&24.181202&8.061$\pm$0.027&7.848$\pm$0.009&7.769$\pm$0.013&AAA1&9.52&
9.05&8.45&3&
HII1912 HD23778 Tr528b
\\
57.146606&22.895149&14.800$\pm$0.030&14.099$\pm$0.047&13.747$\pm$0.045&AAA1&
\nodata&20.70&17.02&7&
HHJ10 BPL181 PPL10
\\
57.147865&24.200916&14.102$\pm$0.020&13.491$\pm$0.029&13.212$\pm$0.021&AAA2&
\nodata&19.67&16.12&5&
HCG335 HHJ96 BPL182 DH583
\\
57.151382&25.261534&14.889$\pm$0.036&14.251$\pm$0.047&13.886$\pm$0.046&AAA1&
\nodata&\nodata&16.59&19&
BPL183
\\
57.156845&22.769320&11.502$\pm$0.018&10.825$\pm$0.021&10.650$\pm$0.015&AAA1&
16.01&14.57&12.69&1&
HCG341 T87 DH584
\\
57.163754&24.838917&14.300$\pm$0.021&13.745$\pm$0.029&13.421$\pm$0.022&AAA2&
\nodata&\nodata&16.12&22&
DH585
\\
57.166275&24.211941&12.718$\pm$0.019&12.037$\pm$0.028&11.850$\pm$0.020&AAA2&
\nodata&16.68&14.12&5&
HCG337 SK353 HHJ347 BPL184
\\
57.168446&24.609516&13.201$\pm$0.019&12.599$\pm$0.029&12.331$\pm$0.020&AAA2&
\nodata&17.71&15.09&20&
HCG333 SK351 BPL185 DH586
\\
57.169140&25.022268&14.602$\pm$0.028&13.987$\pm$0.039&13.613$\pm$0.035&AAA1&
\nodata&\nodata&16.33&19&
BPL186
\\
57.170750&23.238203&12.884$\pm$0.015&12.329$\pm$0.028&12.034$\pm$0.020&AAA2&
\nodata&17.66&14.91&20&
HCG343 SK352
\\
57.175571&25.007936&12.586$\pm$0.018&11.954$\pm$0.019&11.720$\pm$0.018&AAA1&
18.24&16.61&14.04&1&
HCG339 SK349 B207 BPL187
\\
57.177849&24.455458&14.372$\pm$0.021&13.815$\pm$0.030&13.492$\pm$0.022&AAA2&
\nodata&19.29&16.09&7&
HHJ44 BPL188 DH587
\\
57.179688&26.539261&13.247$\pm$0.019&12.622$\pm$0.020&12.375$\pm$0.022&AAA1&
\nodata&17.70&14.80&21&
HHJ246 DH588
\\
57.182880&23.259859&7.758$\pm$0.017&7.700$\pm$0.015&7.631$\pm$0.009&AAA1&8.65&
8.39&8.05&3&
HII1993 HD23791 Tr551
\\
57.183495&25.106304&13.489$\pm$0.020&12.894$\pm$0.026&12.622$\pm$0.023&AAA1&
\nodata&\nodata&15.16&19&
BPL189 DH589
\\
57.186188&24.623243&14.926$\pm$0.023&14.351$\pm$0.035&14.035$\pm$0.024&AAA2&
\nodata&\nodata&16.91&22&
DH590
\\
57.188961&24.624012&14.014$\pm$0.020&13.481$\pm$0.030&13.174$\pm$0.022&AAA2&
\nodata&\nodata&15.75&19&
HCG346 HHJ111 BPL190
\\
57.189312&23.338873&11.065$\pm$0.998&10.384$\pm$0.047&10.375$\pm$0.067&FAA2&
14.77&13.55&12.08&1&
HII2016 Tr557 HCG344
\\
57.190331&25.700514&12.628$\pm$0.019&11.970$\pm$0.020&11.683$\pm$0.014&AAA1&
\nodata&16.90&14.20&21&
HHJ333 DH591
\\
57.191715&24.170187&13.517$\pm$0.019&12.927$\pm$0.028&12.664$\pm$0.020&AAA2&
\nodata&18.00&15.18&6&
HHJ207 DH592
\\
57.203255&23.413395&14.062$\pm$0.016&13.471$\pm$0.028&13.208$\pm$0.022&AAA2&
\nodata&19.70&15.80&21&
HHJ86
\\
57.203949&24.267435&9.330$\pm$0.017&8.908$\pm$0.013&8.810$\pm$0.015&AAA1&11.78&
10.93&10.01&1&
HII2027 Tr562
\\
57.205509&23.977320&10.658$\pm$0.015&10.133$\pm$0.015&9.992$\pm$0.017&AAA1&13.61
&12.65&11.50&1&
HII2034 Tr563 HCG348
\\
57.210140&25.298620&15.132$\pm$0.041&14.504$\pm$0.054&14.117$\pm$0.061&AAA1&
\nodata&\nodata&17.16&19&
BPL192
\\
57.210144&22.741737&15.094$\pm$0.041&14.492$\pm$0.054&14.130$\pm$0.058&AAA1&
\nodata&21.24&17.51&7&
HHJ3 BPL191
\\
57.210407&24.140930&15.537$\pm$0.026&14.904$\pm$0.039&14.709$\pm$0.034&AAA2&
\nodata&\nodata&17.68&22&
DH593
\\
57.211086&23.075073&13.991$\pm$0.020&13.421$\pm$0.027&13.110$\pm$0.020&AAA2&
\nodata&19.20&15.60&21&
HHJ116
\\
57.214775&24.204830&12.190$\pm$0.019&11.511$\pm$0.028&11.260$\pm$0.019&AAA2&
17.55&16.09&13.60&1&
BPL193 ALR728
\\
57.230083&22.845106&13.969$\pm$0.023&13.406$\pm$0.026&13.118$\pm$0.031&AAA1&
\nodata&\nodata&15.77&19&
BPL194
\\
57.231857&24.361214&15.043$\pm$0.025&14.434$\pm$0.034&14.101$\pm$0.027&AAA2&
\nodata&20.60&16.85&7&
HHJ8
\\
57.237648&26.615034&11.548$\pm$0.019&10.925$\pm$0.030&10.701$\pm$0.019&AAA1&
\nodata&\nodata&13.25&22&
DH594
\\
57.238956&24.328848&11.906$\pm$0.019&11.322$\pm$0.032&11.014$\pm$0.019&AAA2&
\nodata&16.00&13.34&20&
HCG349 SK340
\\
57.242847&23.094244&12.537$\pm$0.019&11.907$\pm$0.029&11.669$\pm$0.019&AAA2&
\nodata&16.20&14.00&21&
HHJ353 DH595
\\
57.243690&23.201229&9.909$\pm$0.018&9.520$\pm$0.025&9.377$\pm$0.015&AAA1&12.41&
11.54&10.59&1&
HII2106
\\
57.245682&25.103958&11.406$\pm$0.025&10.745$\pm$0.030&10.571$\pm$0.016&AAA1&
15.26&13.91&12.33&1&
HII2082
\\
57.254082&24.902826&12.686$\pm$0.015&12.073$\pm$0.027&11.814$\pm$0.020&AAA2&
\nodata&17.11&14.40&20&
HCG351 SK335 HHJ332 BPL195
\\
57.254169&22.980446&12.030$\pm$0.016&11.355$\pm$0.025&11.150$\pm$0.016&AAA1&
16.94&15.39&13.23&1&
HCG353 SK336 A55 HHJ414
\\
57.254772&23.637695&14.472$\pm$0.020&13.866$\pm$0.028&13.583$\pm$0.022&AAA2&
\nodata&\nodata&16.54&22&
DH598
\\
57.256214&24.193983&13.367$\pm$0.015&12.775$\pm$0.027&12.511$\pm$0.019&AAA2&
\nodata&17.70&14.90&21&
HHJ231 BPL196 DH599
\\
57.259705&23.252468&10.135$\pm$0.017&9.758$\pm$0.021&9.657$\pm$0.016&AAA1&12.56&
11.71&10.80&1&
HII2126 Tr584
\\
57.262318&21.913120&14.232$\pm$0.024&13.595$\pm$0.030&13.366$\pm$0.033&AAA1&
\nodata&\nodata&16.17&19&
BPL197
\\
57.274410&23.739756&11.641$\pm$0.019&10.999$\pm$0.027&10.786$\pm$0.020&AAA2&
16.76&15.31&12.94&1&
HCG354 SK331 T157 HHJ440
\\
57.274666&23.106136&13.126$\pm$0.020&12.493$\pm$0.028&12.244$\pm$0.020&AAA2&
\nodata&17.52&14.94&20&
HCG357 SK332 DH602
\\
57.275452&23.781273&9.166$\pm$0.018&8.719$\pm$0.039&8.603$\pm$0.015&AAA1&11.69&
10.87&9.89&3&
HII2147 Tr588
\\
57.277252&22.004869&14.779$\pm$0.034&14.109$\pm$0.041&13.802$\pm$0.045&AAA1&
\nodata&\nodata&16.67&19&
BPL198
\\
57.286800&25.896910&12.308$\pm$0.023&11.683$\pm$0.028&11.384$\pm$0.024&AAA1&
\nodata&16.07&13.57&5&
SK327 HHJ387 DH603
\\
57.290600&24.053375&3.800$\pm$0.270&3.864$\pm$0.234&3.879$\pm$0.318&DDD1&3.53&
3.62&3.65&3&
HII2168 27Tau Atlas HD23850
\\
57.295956&24.347589&13.048$\pm$0.018&12.420$\pm$0.027&12.178$\pm$0.024&AAA2&
\nodata&17.43&14.64&12&
HCG355 HHJ287 BPL199 DH604
\\
57.296722&24.136675&5.087$\pm$0.033&5.067$\pm$0.045&4.937$\pm$0.015&EAA1&5.01&
5.09&5.08&3&
HII2181 28Tau Pleione HD23862
\\
57.296814&22.176792&10.892$\pm$0.018&10.289$\pm$0.020&10.103$\pm$0.016&AAA1&
15.11&13.80&12.10&1&
HCG360 T54B
\\
57.296989&23.555243&11.411$\pm$0.018&10.768$\pm$0.031&10.575$\pm$0.019&AAA2&
15.60&14.23&12.50&1&
HII2193 HCG358 SK326 DH605
\\
57.297535&24.240187&13.736$\pm$0.016&13.165$\pm$0.028&12.847$\pm$0.021&AAA2&
\nodata&\nodata&15.43&19&
BPL200 DH606
\\
57.298859&24.636606&9.246$\pm$0.043&9.028$\pm$0.030&8.949$\pm$0.016&AAA1&11.06&
10.44&9.74&13&
HII2172 HD282965
\\
57.300808&23.886839&7.673$\pm$0.015&7.599$\pm$0.027&7.576$\pm$0.011&AAA1&8.35&
8.13&7.88&3&
HII2195 HD23863 Tr607
\\
57.301277&23.228354&11.527$\pm$0.019&10.900$\pm$0.028&10.721$\pm$0.019&AAA2&
15.85&14.48&12.66&1&
HII2209 DH607
\\
57.302151&24.186924&16.412$\pm$0.039&15.600$\pm$0.052&15.286$\pm$0.049&AAA2&
\nodata&\nodata&19.34&19&
BPL201
\\
57.302666&25.702093&12.598$\pm$0.018&11.954$\pm$0.027&11.698$\pm$0.024&AAA1&
\nodata&17.11&14.47&20&
HCG365 SK325 HHJ331 DH608
\\
57.312984&24.606314&15.393$\pm$0.025&14.823$\pm$0.038&14.481$\pm$0.031&AAA2&
\nodata&\nodata&17.53&19&
BPL202
\\
57.314083&24.567284&11.341$\pm$0.018&10.666$\pm$0.027&10.494$\pm$0.019&AAA2&
15.78&14.42&12.55&1&
HII2208 HCG359 SK324
\\
57.315067&23.380386&14.336$\pm$0.019&13.707$\pm$0.032&13.413$\pm$0.020&AAA2&
\nodata&19.47&16.05&7&
HHJ36
\\
57.318363&24.063673&11.688$\pm$0.999&11.021$\pm$0.027&10.754$\pm$0.019&UAA2&
\nodata&15.00&\nodata&21&
HCG362
\\
57.319969&24.396139&7.280$\pm$0.013&7.290$\pm$0.043&7.257$\pm$0.027&AAA1&7.57&
7.46&7.34&3&
HII2220 HD23872 Tr613
\\
57.320011&24.016356&13.085$\pm$0.022&12.578$\pm$0.033&12.240$\pm$0.023&AAA1&
\nodata&18.10&14.40&21&
HHJ308 DH609
\\
57.327724&23.780285&14.310$\pm$0.019&13.647$\pm$0.029&13.420$\pm$0.021&AAA2&
\nodata&\nodata&15.62&22&
DH610
\\
57.334572&25.428505&13.210$\pm$0.021&12.605$\pm$0.028&12.326$\pm$0.023&AAA1&
99.99&17.40&14.80&21&
HCG366 HHJ251 DH611
\\
57.335648&25.818016&11.320$\pm$0.020&10.670$\pm$0.028&10.487$\pm$0.022&AAA1&
15.32&13.97&12.34&1&
HCG367 T32B DH612
\\
57.335793&24.776670&10.624$\pm$0.019&10.030$\pm$0.027&9.925$\pm$0.019&AAA1&13.61
&12.60&11.40&10&
HII2244 Tr616 HCG369 DH613
\\
57.336147&24.876501&14.631$\pm$0.017&14.050$\pm$0.031&13.754$\pm$0.023&AAA2&
\nodata&\nodata&16.18&19&
BPL203
\\
57.337318&26.192724&15.901$\pm$0.071&15.182$\pm$0.076&14.969$\pm$0.101&AAA1&
\nodata&\nodata&18.12&22&
DH614
\\
57.338516&24.694727&14.407$\pm$0.020&13.787$\pm$0.028&13.513$\pm$0.023&AAA2&
\nodata&20.30&16.10&21&
HHJ51 BPL204 DH615
\\
57.339542&23.651802&12.830$\pm$0.018&12.237$\pm$0.028&11.985$\pm$0.020&AAA2&
\nodata&17.15&14.41&20&
HCG363 SK319 HHJ306 DH616
\\
57.340572&24.380976&6.602$\pm$0.003&6.630$\pm$0.023&6.651$\pm$0.009&AAA1&6.55&
6.57&6.57&3&
HII2263 HD23873 Tr622
\\
57.341343&24.912077&13.623$\pm$0.016&13.053$\pm$0.030&12.754$\pm$0.020&AAA2&
\nodata&17.48&15.23&20&
SK316 BPL205 DH617
\\
57.342262&25.793869&13.456$\pm$0.023&12.815$\pm$0.028&12.566$\pm$0.026&AAA1&
\nodata&18.00&15.10&21&
HHJ196 DH618
\\
57.343777&21.632334&13.542$\pm$0.019&12.982$\pm$0.022&12.658$\pm$0.026&AAA1&
\nodata&\nodata&15.31&22&
DH619
\\
57.350216&23.839287&9.854$\pm$0.016&9.482$\pm$0.022&9.378$\pm$0.016&AAA1&12.13&
11.35&99.99&3&
HII2284 Tr628
\\
57.356430&22.312429&14.213$\pm$0.028&13.576$\pm$0.030&13.324$\pm$0.033&AAA1&
\nodata&\nodata&16.17&19&
BPL206
\\
57.356651&23.047304&14.086$\pm$0.020&13.470$\pm$0.029&13.206$\pm$0.021&AAA2&
\nodata&18.92&15.72&7&
HHJ79 BPL207 DH620
\\
57.357094&24.937620&9.284$\pm$0.021&8.937$\pm$0.031&8.805$\pm$0.018&AAA1&11.81&
10.94&10.00&1&
HII2278 Tr626
\\
57.358269&24.247681&7.587$\pm$0.015&7.548$\pm$0.027&7.515$\pm$0.021&AAA1&8.17&
7.99&7.79&3&
HII2289 HD23886 Tr629
\\
57.360939&22.848576&13.398$\pm$0.023&12.724$\pm$0.024&12.511$\pm$0.023&AAA1&
\nodata&18.23&15.22&21&
SK315 BPL208
\\
57.364906&24.403845&13.546$\pm$0.019&12.936$\pm$0.028&12.680$\pm$0.024&AAA2&
\nodata&18.10&15.22&6&
HHJ192 DH621
\\
57.365147&24.531731&12.119$\pm$0.018&11.475$\pm$0.027&11.258$\pm$0.024&AAA2&
\nodata&15.97&13.52&7&
HCG370 DH622
\\
57.366203&26.513500&14.273$\pm$0.026&13.711$\pm$0.036&13.473$\pm$0.031&AAA1&
\nodata&\nodata&15.74&22&
DH623
\\
57.369747&23.712238&9.914$\pm$0.018&9.543$\pm$0.022&9.428$\pm$0.020&AAA1&12.17&
11.35&10.50&1&
HII2311
\\
57.374203&23.648733&13.564$\pm$0.019&12.962$\pm$0.028&12.700$\pm$0.020&AAA2&
\nodata&18.30&15.20&21&
HHJ158 DH624
\\
57.380081&23.688850&13.639$\pm$0.020&13.024$\pm$0.027&12.761$\pm$0.019&AAA2&
\nodata&18.60&15.40&21&
HHJ142 DH625
\\
57.383984&23.271732&14.301$\pm$0.024&13.767$\pm$0.033&13.440$\pm$0.037&AAA1&
\nodata&\nodata&15.97&22&
DH626
\\
57.385563&23.928522&13.329$\pm$0.019&12.728$\pm$0.028&12.436$\pm$0.019&AAA2&
99.99&17.91&15.27&20&
HCG371 SK310 HHJ221 DH627
\\
57.385700&23.411463&13.210$\pm$0.015&12.640$\pm$0.028&12.354$\pm$0.019&AAA2&
\nodata&17.92&14.85&7&
HHJ245
\\
57.386341&23.380413&8.258$\pm$0.013&8.097$\pm$0.019&8.036$\pm$0.017&AAA1&9.58&
9.14&8.63&3&
HII2345 HD23912 Tr651
\\
57.386642&25.796438&13.501$\pm$0.021&12.925$\pm$0.025&12.619$\pm$0.022&AAA1&
\nodata&18.30&15.00&21&
HHJ209 DH628
\\
57.387638&24.534067&12.617$\pm$0.018&11.957$\pm$0.027&11.738$\pm$0.020&AAA2&
18.10&16.58&13.99&12&
HCG372 SK309 T90 HHJ346
\\
57.387951&24.218021&14.626$\pm$0.023&14.026$\pm$0.032&13.754$\pm$0.027&AAA2&
\nodata&\nodata&16.38&19&
BPL210
\\
57.388004&23.795427&9.595$\pm$0.016&9.294$\pm$0.021&9.214$\pm$0.018&AAA1&11.65&
10.93&10.19&1&
HII2341 Tr649
\\
57.395473&23.454689&11.240$\pm$0.019&10.578$\pm$0.027&10.420$\pm$0.020&AAA2&
\nodata&13.92&12.19&20&
HII2368 HCG374 DH629
\\
57.396961&25.993065&13.538$\pm$0.019&12.929$\pm$0.024&12.693$\pm$0.025&AAA1&
\nodata&18.30&15.30&21&
HHJ155 DH630
\\
57.397701&22.390697&13.944$\pm$0.023&13.323$\pm$0.026&13.055$\pm$0.028&AAA1&
\nodata&18.80&15.60&21&
HHJ112 BPL211
\\
57.398956&20.108042&13.785$\pm$0.022&13.274$\pm$0.028&12.917$\pm$0.026&AAA1&
\nodata&\nodata&16.17&22&
DH631
\\
57.399490&22.151480&10.869$\pm$0.020&10.218$\pm$0.022&10.022$\pm$0.018&AAA1&
\nodata&13.40&\nodata&21&
HCG376 MT104
\\
57.400475&23.939840&13.192$\pm$0.019&12.549$\pm$0.028&12.276$\pm$0.019&AAA2&
99.99&17.46&14.76&20&
HCG373 SK307 HHJ286 DH632
\\
57.401237&26.037956&14.364$\pm$0.026&13.786$\pm$0.033&13.436$\pm$0.033&AAA1&
\nodata&20.40&16.20&21&
HHJ42 DH633
\\
57.402180&24.303963&13.321$\pm$0.020&12.702$\pm$0.028&12.434$\pm$0.024&AAA2&
\nodata&17.23&14.68&5&
HCG375 HHJ250 BPL212 DH634
\\
57.402245&24.296135&10.029$\pm$0.018&9.634$\pm$0.020&9.550$\pm$0.016&AAA1&12.31&
11.49&10.63&1&
HII2366 Tr657
\\
57.409279&26.851675&13.086$\pm$0.018&12.466$\pm$0.020&12.263$\pm$0.019&AAA1&
\nodata&\nodata&14.92&22&
DH635
\\
57.414158&23.290129&9.693$\pm$0.016&9.364$\pm$0.022&9.256$\pm$0.018&AAA1&11.86&
11.10&99.99&3&
HII2406 Tr667
\\
57.420506&23.341612&7.700$\pm$0.011&7.657$\pm$0.013&7.648$\pm$0.011&AAA1&8.35&
8.14&7.91&1&
HII2415 HD23924 Tr670
\\
57.421669&22.944704&15.069$\pm$0.040&14.423$\pm$0.050&14.012$\pm$0.047&AAA1&
\nodata&\nodata&16.78&19&
BPL213
\\
57.422226&26.148220&12.819$\pm$0.018&12.164$\pm$0.021&11.946$\pm$0.021&AAA1&
\nodata&16.70&14.40&21&
HHJ305 DH636
\\
57.423744&21.938759&14.767$\pm$0.034&14.072$\pm$0.041&13.762$\pm$0.047&AAA1&
\nodata&\nodata&16.83&19&
BPL214
\\
57.426128&24.463060&10.355$\pm$0.017&9.909$\pm$0.017&9.783$\pm$0.015&AAA1&13.14&
12.19&11.17&1&
HII2407 Tr668 DH637
\\
57.429871&24.662975&15.120$\pm$0.023&14.498$\pm$0.036&14.159$\pm$0.026&AAA2&
\nodata&\nodata&16.85&19&
BPL215
\\
57.431374&23.711880&6.163$\pm$0.005&6.225$\pm$0.007&6.216$\pm$0.017&AAA1&6.12&
6.17&6.18&3&
HII2425 HD23923 Tr671
\\
57.445961&25.710295&12.918$\pm$0.018&12.304$\pm$0.021&12.006$\pm$0.016&AAA1&
\nodata&\nodata&14.95&22&
DH638
\\
57.451813&22.180164&12.948$\pm$0.019&12.242$\pm$0.022&11.994$\pm$0.021&AAA1&
\nodata&\nodata&14.67&19&
BPL216 DH639
\\
57.459827&23.705631&10.067$\pm$0.018&9.699$\pm$0.021&9.595$\pm$0.016&AAA1&12.33&
11.49&10.63&1&
HII2462 Tr680
\\
57.465805&21.307348&11.808$\pm$0.016&11.162$\pm$0.022&10.921$\pm$0.016&AAA1&
\nodata&\nodata&13.31&22&
HCG378 DH640
\\
57.470463&25.647491&8.489$\pm$0.011&8.332$\pm$0.009&8.254$\pm$0.013&AAA1&10.09&
9.57&\nodata&4&
PELS150 HD23935 TrS144y
\\
57.481174&24.101456&13.529$\pm$0.016&12.887$\pm$0.028&12.630$\pm$0.024&AAA2&
\nodata&\nodata&14.98&22&
DH641
\\
57.482403&24.742126&12.422$\pm$0.015&11.801$\pm$0.027&11.568$\pm$0.020&AAA2&
17.74&16.26&13.74&1&
HCG380 SK294 T92 BPL217
\\
57.485363&23.218641&9.145$\pm$0.018&8.854$\pm$0.011&8.796$\pm$0.016&AAA1&10.87&
10.27&9.58&3&
HII2506
\\
57.485859&24.349070&7.346$\pm$0.011&7.367$\pm$0.007&7.350$\pm$0.009&AAA1&7.63&
7.55&7.48&3&
HII2488 HD23948 Tr688
\\
57.486488&25.373075&13.400$\pm$0.021&12.857$\pm$0.024&12.579$\pm$0.021&AAA1&
\nodata&\nodata&15.00&22&
DH643
\\
57.486641&24.985392&15.191$\pm$0.046&14.532$\pm$0.058&14.429$\pm$0.071&AAA1&
\nodata&\nodata&17.12&19&
BPL218
\\
57.490124&23.724539&14.299$\pm$0.019&13.730$\pm$0.027&13.388$\pm$0.022&AAA2&
\nodata&\nodata&16.18&22&
DH644
\\
57.491905&23.858738&6.545$\pm$0.019&6.587$\pm$0.059&6.514$\pm$0.023&AAA1&6.78&
6.72&6.59&3&
HII2507 HD23964 Tr697
\\
57.493019&25.105911&14.251$\pm$0.025&13.737$\pm$0.037&13.405$\pm$0.036&AAA1&
\nodata&\nodata&15.96&19&
BPL219
\\
57.493065&23.709436&12.468$\pm$0.019&11.833$\pm$0.027&11.567$\pm$0.019&AAA2&
\nodata&15.92&13.69&5&
SK293
\\
57.498066&24.196119&14.454$\pm$0.021&13.866$\pm$0.031&13.554$\pm$0.026&AAA2&
\nodata&\nodata&16.20&19&
BPL220
\\
57.502674&25.398848&10.631$\pm$0.018&9.991$\pm$0.020&9.845$\pm$0.014&AAA1&14.60&
13.29&11.67&1&
HCG384 SK292 T108 DH645
\\
57.506516&25.400528&12.270$\pm$0.018&11.715$\pm$0.015&11.459$\pm$0.017&AAA1&
\nodata&15.83&13.70&20&
SK291 DH646
\\
57.506973&24.613527&14.431$\pm$0.020&13.865$\pm$0.028&13.563$\pm$0.023&AAA2&
\nodata&\nodata&16.15&19&
BPL221
\\
57.507755&25.211456&13.276$\pm$0.018&12.661$\pm$0.020&12.420$\pm$0.024&AAA1&
\nodata&17.64&15.00&21&
HCG385 SK289 BPL222 DH647
\\
57.509048&23.862457&12.864$\pm$0.019&12.228$\pm$0.031&11.992$\pm$0.020&AAA2&
\nodata&\nodata&13.95&22&
HCG382 DH648
\\
57.516270&23.976154&13.307$\pm$0.019&12.728$\pm$0.028&12.484$\pm$0.019&AAA2&
\nodata&17.30&14.70&21&
HHJ256
\\
57.516422&24.934174&15.194$\pm$0.020&14.514$\pm$0.033&14.202$\pm$0.027&AAA2&
\nodata&\nodata&16.91&19&
BPL223
\\
57.517666&23.179070&13.264$\pm$0.015&12.553$\pm$0.028&12.335$\pm$0.020&AAA2&
\nodata&17.33&14.81&20&
SK287 DH649
\\
57.520805&23.304855&14.302$\pm$0.019&13.694$\pm$0.028&13.400$\pm$0.021&AAA2&
\nodata&\nodata&16.19&22&
DH650
\\
57.521084&24.123985&11.414$\pm$0.019&10.749$\pm$0.028&10.586$\pm$0.019&AAA2&
15.37&14.03&12.39&16&
HII2548 DH651
\\
57.526733&26.971972&13.801$\pm$0.022&13.160$\pm$0.025&12.928$\pm$0.026&AAA1&
\nodata&\nodata&15.74&22&
DH652
\\
57.527294&24.996281&12.883$\pm$0.015&12.325$\pm$0.028&12.034$\pm$0.020&AAA2&
\nodata&\nodata&14.61&19&
BPL224 DH653
\\
57.535046&25.548910&13.228$\pm$0.020&12.619$\pm$0.019&12.380$\pm$0.021&AAA1&
\nodata&\nodata&15.02&22&
HCG386 DH654
\\
57.535908&24.671646&14.281$\pm$0.021&13.649$\pm$0.029&13.386$\pm$0.024&AAA2&
\nodata&\nodata&16.27&22&
DH655
\\
57.544861&24.478228&13.749$\pm$0.016&13.153$\pm$0.028&12.884$\pm$0.021&AAA2&
\nodata&\nodata&15.48&19&
BPL225 DH656
\\
57.551086&23.995897&11.702$\pm$0.019&11.078$\pm$0.029&10.845$\pm$0.019&AAA2&
17.12&15.49&13.04&1&
HII2602 HCG391 SK280 DH657
\\
57.551674&24.532957&10.983$\pm$0.013&10.433$\pm$0.013&10.271$\pm$0.016&AAA1&
14.47&13.29&11.98&16&
HII2588 HCG387 Tr712 DH658
\\
57.551868&23.926731&13.045$\pm$0.019&12.386$\pm$0.028&12.123$\pm$0.019&AAA2&
\nodata&18.15&15.29&20&
SK279 DH659
\\
57.552471&23.813648&14.454$\pm$0.020&13.881$\pm$0.030&13.585$\pm$0.021&AAA2&
\nodata&\nodata&16.25&22&
DH660
\\
57.553776&24.351862&11.416$\pm$0.015&10.891$\pm$0.029&10.627$\pm$0.021&AAE2&
16.54&15.01&12.68&1&
HII2601 HCG390 SK278 DH661
\\
57.561443&25.425056&13.790$\pm$0.021&13.141$\pm$0.025&12.922$\pm$0.027&AAA1&
\nodata&\nodata&15.69&22&
DH662
\\
57.563602&24.226727&13.223$\pm$0.019&12.634$\pm$0.029&12.377$\pm$0.020&AAA2&
19.51&17.54&14.64&1&
HCG394 SK276 B214 BPL226
\\
57.573242&22.933102&14.306$\pm$0.026&13.663$\pm$0.037&13.371$\pm$0.035&AAA1&
\nodata&\nodata&16.28&22&
DH664
\\
57.573582&25.379555&8.645$\pm$0.021&8.469$\pm$0.029&8.382$\pm$0.017&AAA1&10.14&
9.64&\nodata&8&
TrS151x HD23975
\\
57.575878&24.587667&13.726$\pm$0.019&13.132$\pm$0.028&12.891$\pm$0.020&AAA2&
\nodata&\nodata&15.40&19&
BPL227 DH665
\\
57.579758&24.276148&15.178$\pm$0.023&14.540$\pm$0.032&14.222$\pm$0.026&AAA2&
\nodata&\nodata&17.08&19&
BPL228
\\
57.587078&24.466755&9.746$\pm$0.013&9.397$\pm$0.013&9.307$\pm$0.015&AAA1&11.86&
11.09&10.32&1&
HII2644 Tr727
\\
57.588753&23.096392&9.863$\pm$0.016&9.512$\pm$0.025&9.385$\pm$0.018&AAA1&12.19&
11.36&99.99&3&
HII2665
\\
57.588787&27.144409&9.836$\pm$0.018&9.448$\pm$0.017&9.356$\pm$0.016&AAA1&12.14&
11.33&\nodata&9&
AKIV131
\\
57.591812&22.625748&13.230$\pm$0.019&12.562$\pm$0.024&12.299$\pm$0.021&AAA1&
\nodata&18.09&15.30&20&
HCG399 DH666
\\
57.595463&22.188366&11.462$\pm$0.018&10.786$\pm$0.021&10.585$\pm$0.018&AAA1&
\nodata&14.80&12.60&23&
HCG398 DH667
\\
57.603951&20.705051&11.812$\pm$0.016&11.118$\pm$0.021&10.935$\pm$0.020&AAA1&
\nodata&\nodata&13.02&22&
DH668
\\
57.604778&23.928335&13.636$\pm$0.020&13.017$\pm$0.028&12.765$\pm$0.020&AAA2&
\nodata&\nodata&15.20&22&
HCG396 DH669
\\
57.613922&23.379217&13.410$\pm$0.019&12.826$\pm$0.029&12.542$\pm$0.020&AAA2&
\nodata&18.16&15.44&20&
SK273 DH670
\\
57.615929&23.065313&13.796$\pm$0.015&13.226$\pm$0.027&12.938$\pm$0.020&AAA2&
\nodata&\nodata&15.71&22&
DH671
\\
57.622074&24.943014&13.632$\pm$0.016&12.928$\pm$0.027&12.697$\pm$0.021&AAA2&
\nodata&\nodata&15.33&19&
BPL229
\\
57.624825&25.051985&12.638$\pm$0.020&12.016$\pm$0.022&11.762$\pm$0.021&AAA1&
18.15&16.57&14.00&1&
HCG403 SK272 B213 BPL230
\\
57.633099&22.146605&13.042$\pm$0.018&12.364$\pm$0.022&12.118$\pm$0.021&AAA1&
\nodata&16.00&\nodata&21&
HCG401 DH673
\\
57.637821&24.339430&13.409$\pm$0.019&12.843$\pm$0.027&12.547$\pm$0.020&AAA2&
\nodata&\nodata&15.05&19&
BPL231 DH674
\\
57.644051&24.507822&10.698$\pm$0.015&10.197$\pm$0.015&10.080$\pm$0.015&AAA1&
13.66&12.65&11.52&1&
HII2741 DH675
\\
57.648823&25.426512&10.256$\pm$0.017&9.731$\pm$0.019&9.582$\pm$0.015&AAA1&13.14&
12.18&\nodata&4&
PELS072 DH676
\\
57.655857&22.468994&13.285$\pm$0.016&12.661$\pm$0.024&12.372$\pm$0.019&AAA1&
\nodata&\nodata&15.16&22&
HCG404 DH677
\\
57.662136&23.217440&12.643$\pm$0.015&11.992$\pm$0.027&11.749$\pm$0.019&AAA2&
\nodata&17.12&14.40&20&
SK263 DH678
\\
57.663731&25.393772&10.218$\pm$0.018&9.593$\pm$0.017&9.434$\pm$0.015&AAA1&
\nodata&\nodata&11.06&22&
DH679
\\
57.663811&26.267818&14.894$\pm$0.038&14.263$\pm$0.050&14.014$\pm$0.060&AAA1&
\nodata&\nodata&17.36&22&
DH680
\\
57.666985&23.933065&9.181$\pm$0.018&8.941$\pm$0.020&8.853$\pm$0.016&AAA1&10.90&
10.29&9.61&3&
HII2786 HD283067 Tr772
\\
57.670094&24.667467&14.260$\pm$0.021&13.674$\pm$0.028&13.341$\pm$0.022&AAA2&
\nodata&\nodata&15.87&22&
DH681
\\
57.671638&25.658566&14.193$\pm$0.028&13.578$\pm$0.027&13.282$\pm$0.032&AAA1&
\nodata&\nodata&16.20&22&
DH682
\\
57.676811&24.215456&14.037$\pm$0.020&13.456$\pm$0.028&13.162$\pm$0.021&AAA2&
\nodata&\nodata&15.45&22&
DH683
\\
57.681179&26.041243&9.781$\pm$0.015&9.482$\pm$0.019&9.400$\pm$0.016&AAA1&11.86&
11.15&\nodata&4&
PELS151 AKIV144
\\
57.703983&22.670065&12.196$\pm$0.026&11.485$\pm$0.024&11.271$\pm$0.018&AAA1&
\nodata&16.21&13.48&20&
HCG409 DH684
\\
57.714333&23.329100&10.632$\pm$0.016&10.108$\pm$0.021&10.015$\pm$0.018&AAA1&
13.52&12.51&11.40&1&
HII2870 DH685
\\
57.718502&23.961548&6.643$\pm$0.009&6.628$\pm$0.011&6.580$\pm$0.007&AAA1&7.02&
6.93&6.81&3&
HII2866 HD24076 Tr791
\\
57.724388&22.548111&10.683$\pm$0.021&10.112$\pm$0.021&9.987$\pm$0.016&AAA1&
\nodata&\nodata&11.69&22&
DH686
\\
57.726337&23.834896&9.677$\pm$0.023&9.230$\pm$0.025&9.054$\pm$0.016&AAA1&12.54&
11.57&10.47&1&
HII2881 Tr796
\\
57.727699&24.365543&13.600$\pm$0.019&13.039$\pm$0.027&12.776$\pm$0.020&AAA2&
\nodata&\nodata&15.14&22&
DH687
\\
57.729527&24.197466&10.116$\pm$0.018&9.740$\pm$0.020&9.629$\pm$0.015&AAA1&12.61&
11.75&99.99&3&
HII2880 Tr795
\\
57.735867&25.585190&12.462$\pm$0.017&11.844$\pm$0.015&11.581$\pm$0.017&AAA1&
\nodata&16.87&14.22&20&
HCG412 SK253 DH688
\\
57.739239&24.108593&12.693$\pm$0.019&12.067$\pm$0.028&11.838$\pm$0.020&AAA2&
\nodata&16.70&14.17&20&
HCG415 SK251 DH689
\\
57.742352&23.928570&13.632$\pm$0.019&13.004$\pm$0.031&12.771$\pm$0.019&AAA2&
\nodata&\nodata&15.08&22&
HCG414 DH690
\\
57.759632&25.055477&11.044$\pm$0.015&10.493$\pm$0.013&10.372$\pm$0.016&AAA1&
14.61&13.47&12.12&1&
HII2908 HCG417
\\
57.765015&24.543182&13.279$\pm$0.020&12.682$\pm$0.028&12.414$\pm$0.019&AAA2&
\nodata&\nodata&14.80&22&
DH691
\\
57.771137&26.614311&14.450$\pm$0.030&13.781$\pm$0.028&13.458$\pm$0.040&AAA1&
\nodata&\nodata&16.39&22&
DH692
\\
57.773258&24.736776&11.285$\pm$0.019&10.432$\pm$0.027&10.447$\pm$0.019&AAA2&
15.18&13.92&12.35&16&
HII2927 HCG418 DH693
\\
57.775490&22.633614&13.925$\pm$0.026&13.343$\pm$0.030&12.977$\pm$0.029&AAA1&
\nodata&\nodata&15.96&22&
DH694
\\
57.779591&23.349382&13.701$\pm$0.015&13.123$\pm$0.027&12.885$\pm$0.019&AAA2&
\nodata&\nodata&15.36&22&
DH695
\\
57.793945&26.587688&11.414$\pm$0.016&10.777$\pm$0.013&10.599$\pm$0.019&AAA1&
\nodata&\nodata&12.68&22&
DH696
\\
57.798080&24.387018&12.187$\pm$0.015&11.597$\pm$0.026&11.301$\pm$0.019&AAA2&
\nodata&16.15&13.59&5&
HCG422 SK245 DH697
\\
57.799484&23.745398&14.304$\pm$0.016&13.719$\pm$0.029&13.418$\pm$0.021&AAA2&
\nodata&\nodata&15.87&19&
BPL232
\\
57.800304&23.932636&11.772$\pm$0.015&11.095$\pm$0.027&10.903$\pm$0.019&AAA2&
16.36&14.86&12.90&1&
HII2966 SK244 DH698
\\
57.815891&23.282274&11.704$\pm$0.018&11.031$\pm$0.026&10.821$\pm$0.019&AAA2&
16.27&14.84&12.87&1&
HCG423 SK239 T95 DH699
\\
57.819229&21.059750&13.309$\pm$0.021&12.732$\pm$0.028&12.381$\pm$0.021&AAA1&
\nodata&\nodata&15.13&22&
DH700
\\
57.820232&23.826605&10.616$\pm$0.017&10.077$\pm$0.028&9.957$\pm$0.019&AAA1&13.41
&12.41&11.33&1&
HII2984 Tr833
\\
57.824772&26.022882&13.759$\pm$0.024&13.130$\pm$0.024&12.843$\pm$0.029&AAA1&
\nodata&\nodata&15.64&22&
DH701
\\
57.825802&24.340622&13.846$\pm$0.016&13.299$\pm$0.026&13.067$\pm$0.021&AAA2&
\nodata&17.89&15.52&20&
SK236
\\
57.828587&26.052504&12.355$\pm$0.019&11.690$\pm$0.019&11.431$\pm$0.023&AAA1&
\nodata&16.23&13.53&5&
SK237
\\
57.829441&24.170362&12.270$\pm$0.015&11.617$\pm$0.028&11.400$\pm$0.019&AAA2&
\nodata&16.11&13.61&5&
HCG424 SK235 BPL233 DH702
\\
57.831146&23.163797&13.054$\pm$0.019&12.438$\pm$0.027&12.171$\pm$0.019&AAA2&
\nodata&\nodata&14.72&22&
DH703
\\
57.832367&23.067848&14.223$\pm$0.020&13.621$\pm$0.028&13.338$\pm$0.021&AAA2&
\nodata&\nodata&16.25&22&
DH704
\\
57.836102&19.643932&12.622$\pm$0.021&11.999$\pm$0.027&11.748$\pm$0.019&AAA1&
\nodata&\nodata&14.70&22&
DH705
\\
57.849216&22.841484&11.448$\pm$0.018&10.781$\pm$0.028&10.595$\pm$0.020&AAA1&
\nodata&\nodata&12.79&22&
DH706
\\
57.849464&22.113394&10.944$\pm$0.019&10.336$\pm$0.025&10.196$\pm$0.017&AAA1&
\nodata&12.00&\nodata&21&
HCG420 DH707
\\
57.849522&25.098026&12.621$\pm$0.020&12.000$\pm$0.013&11.768$\pm$0.022&AAA1&
\nodata&16.40&13.68&20&
SK231 DH708
\\
57.850693&26.053247&12.570$\pm$0.019&11.967$\pm$0.019&11.678$\pm$0.023&AAA1&
18.35&16.68&14.02&1&
HCG427 SK232 T29 DH709
\\
57.851673&24.087425&10.941$\pm$0.045&10.281$\pm$0.091&10.278$\pm$0.029&AAA1&
14.74&13.53&12.08&1&
HII3019 HCG429 DH710
\\
57.855595&23.889364&11.402$\pm$0.015&10.745$\pm$0.029&10.599$\pm$0.020&AAA2&
\nodata&14.03&12.40&20&
HCG430 SK229 DH711
\\
57.856525&23.755955&16.134$\pm$0.026&15.463$\pm$0.043&15.060$\pm$0.039&AAA2&
\nodata&\nodata&18.66&19&
BPL235
\\
57.857784&24.794147&12.047$\pm$0.019&11.458$\pm$0.027&11.192$\pm$0.019&AAA2&
\nodata&15.83&13.58&20&
HCG428 SK230 DH712
\\
57.863419&24.518692&8.059$\pm$0.015&7.930$\pm$0.009&7.877$\pm$0.017&AAA1&9.25&
8.87&8.40&3&
HII3031 HD24132 Tr848
\\
57.874737&23.899223&11.113$\pm$0.015&10.380$\pm$0.061&10.363$\pm$0.081&AAA2&
14.73&13.53&12.06&10&
HII3063 Tr862 HCG431 DH713
\\
57.877438&27.380505&13.845$\pm$0.025&13.259$\pm$0.024&12.910$\pm$0.033&AAA1&
\nodata&\nodata&15.99&22&
DH714
\\
57.891678&24.569189&13.400$\pm$0.020&12.803$\pm$0.028&12.519$\pm$0.020&AAA2&
\nodata&\nodata&14.83&22&
DH715
\\
57.892700&23.797207&13.894$\pm$0.016&13.290$\pm$0.027&13.011$\pm$0.020&AAA2&
\nodata&\nodata&15.50&19&
BPL236 DH716
\\
57.901688&25.228006&12.958$\pm$0.019&12.356$\pm$0.022&12.086$\pm$0.020&AAA1&
\nodata&17.77&14.77&20&
DH717
\\
57.908424&23.183170&10.849$\pm$0.020&10.190$\pm$0.024&10.032$\pm$0.019&AAA1&
14.74&13.47&11.85&1&
HII3104 HCG435
\\
57.912624&22.750286&10.435$\pm$0.018&10.013$\pm$0.028&9.837$\pm$0.020&AAA1&
\nodata&\nodata&11.16&22&
DH718
\\
57.912777&23.367950&13.968$\pm$0.024&13.376$\pm$0.038&13.118$\pm$0.032&AAA1&
\nodata&\nodata&15.57&19&
BPL237
\\
57.912956&24.591480&13.507$\pm$0.019&12.870$\pm$0.028&12.611$\pm$0.019&AAA2&
\nodata&\nodata&14.96&22&
HCG432 DH719
\\
57.913280&23.855104&13.822$\pm$0.024&13.159$\pm$0.034&12.947$\pm$0.026&AAA1&
\nodata&\nodata&15.50&19&
BPL238 DH720
\\
57.913651&24.548941&10.418$\pm$0.016&9.921$\pm$0.017&9.808$\pm$0.020&AAA1&13.02&
12.09&11.06&1&
HII3096 Tr879 DH721
\\
57.918503&24.983185&9.535$\pm$0.018&9.219$\pm$0.013&9.137$\pm$0.020&AAA1&11.68&
10.94&10.12&3&
HII3097 Tr880 DH722
\\
57.925350&21.668364&9.903$\pm$0.019&9.568$\pm$0.021&9.452$\pm$0.016&AAA1&12.42&
11.57&\nodata&4&
PELS068
\\
57.926292&24.361547&13.601$\pm$0.019&13.007$\pm$0.028&12.734$\pm$0.019&AAA2&
\nodata&\nodata&15.15&19&
BPL239 DH723
\\
57.937160&23.444319&16.100$\pm$0.098&15.608$\pm$0.154&14.747$\pm$0.099&ABA1&
\nodata&\nodata&18.45&19&
BPL240
\\
57.960770&22.895733&12.972$\pm$0.022&12.297$\pm$0.021&12.060$\pm$0.021&AAA1&
\nodata&17.58&14.47&20&
HCG437 SK212 DH724
\\
57.964752&23.580414&14.331$\pm$0.032&13.698$\pm$0.031&13.386$\pm$0.032&AAA1&
\nodata&\nodata&15.95&19&
BPL242
\\
57.972446&24.387018&10.630$\pm$0.016&10.027$\pm$0.018&9.883$\pm$0.020&AAA1&13.78
&12.77&11.54&1&
HII3163 Tr911 HCG444 DH725
\\
57.974667&24.047691&12.333$\pm$0.015&11.789$\pm$0.028&11.514$\pm$0.021&AAA2&
18.68&16.92&13.96&1&
HCG441 SK211 BPL243 DH726
\\
57.977097&23.558823&12.689$\pm$0.019&12.059$\pm$0.021&11.782$\pm$0.016&AAA1&
\nodata&17.53&14.13&20&
HCG439 SK210 BPL244 DH727
\\
57.979340&23.961754&13.499$\pm$0.020&12.925$\pm$0.024&12.619$\pm$0.027&AAA1&
\nodata&\nodata&15.03&19&
HCG440 BPL245 DH728
\\
57.986889&23.901966&8.983$\pm$0.011&8.711$\pm$0.017&8.632$\pm$0.015&AAA1&10.62&
10.05&9.38&3&
HII3179 HD24194 TrR21
\\
57.987965&24.951813&15.356$\pm$0.023&14.764$\pm$0.036&14.506$\pm$0.028&AAA2&
\nodata&\nodata&16.96&22&
DH729
\\
57.988895&23.339439&10.986$\pm$0.020&10.353$\pm$0.021&10.198$\pm$0.018&AAA1&
14.34&13.16&11.81&16&
HII3187 DH730
\\
57.989632&25.808764&13.164$\pm$0.019&12.602$\pm$0.019&12.302$\pm$0.022&AAA1&
\nodata&17.59&14.96&20&
HCG446 SK207 DH731
\\
57.993095&23.972116&13.626$\pm$0.023&13.004$\pm$0.024&12.754$\pm$0.032&AAA1&
\nodata&\nodata&15.13&19&
BPL246 DH732
\\
58.003353&19.596888&9.267$\pm$0.020&8.981$\pm$0.020&8.873$\pm$0.016&AAA1&11.18&
10.52&\nodata&4&
PELS146
\\
58.006554&24.336597&15.195$\pm$0.023&14.459$\pm$0.033&14.323$\pm$0.028&AAA2&
\nodata&\nodata&16.68&19&
BPL247
\\
58.006824&25.024866&13.460$\pm$0.024&12.855$\pm$0.015&12.647$\pm$0.029&AAA1&
\nodata&\nodata&15.11&19&
HCG447 BPL248 DH733
\\
58.008713&23.262535&17.195$\pm$0.230&15.876$\pm$0.177&15.425$\pm$0.175&DCC1&
\nodata&\nodata&19.74&19&
BPL249
\\
58.009331&24.663309&9.797$\pm$0.014&9.207$\pm$0.013&9.072$\pm$0.018&AAA1&13.17&
12.10&10.77&1&
HII3197 HCG448
\\
58.009426&24.363386&12.238$\pm$0.019&11.590$\pm$0.026&11.372$\pm$0.020&AAA2&
\nodata&\nodata&12.87&22&
SK204 DH734
\\
58.010311&21.610495&15.940$\pm$0.078&15.272$\pm$0.107&14.961$\pm$0.113&AAB1&
\nodata&\nodata&17.71&22&
DH735
\\
58.010952&25.104206&13.646$\pm$0.025&13.114$\pm$0.018&12.840$\pm$0.032&AAA1&
\nodata&\nodata&15.42&19&
BPL250 DH736
\\
58.014900&25.020552&13.860$\pm$0.028&13.209$\pm$0.020&12.968$\pm$0.033&AAA1&
\nodata&\nodata&15.51&19&
BPL251 DH737
\\
58.015064&23.289318&13.806$\pm$0.023&13.098$\pm$0.024&12.821$\pm$0.025&AAA1&
\nodata&17.90&15.31&20&
SK202
\\
58.018227&21.760900&14.231$\pm$0.023&13.613$\pm$0.029&13.292$\pm$0.031&AAA1&
\nodata&\nodata&16.24&22&
DH738
\\
58.018650&24.244398&13.803$\pm$0.019&13.190$\pm$0.028&12.930$\pm$0.019&AAA2&
\nodata&\nodata&15.34&19&
BPL252 DH739
\\
58.023212&22.582052&12.379$\pm$0.018&11.722$\pm$0.021&11.483$\pm$0.016&AAA1&
\nodata&16.13&13.69&5&
SK201 DH740
\\
58.024235&24.292034&15.256$\pm$0.023&14.603$\pm$0.032&14.281$\pm$0.028&AAA2&
\nodata&\nodata&16.99&19&
BPL253
\\
58.027733&22.020739&13.976$\pm$0.021&13.453$\pm$0.029&13.122$\pm$0.030&AAA1&
\nodata&\nodata&15.75&22&
DH741
\\
58.027950&24.266870&15.543$\pm$0.024&15.037$\pm$0.039&14.554$\pm$0.031&AAA2&
\nodata&\nodata&17.59&19&
BPL254
\\
58.033115&25.465219&14.155$\pm$0.026&13.610$\pm$0.028&13.267$\pm$0.036&AAA1&
\nodata&\nodata&15.91&19&
HCG449 BPL255 DH742
\\
58.036694&20.438606&9.849$\pm$0.019&9.294$\pm$0.022&9.137$\pm$0.016&AAA1&13.03&
11.93&\nodata&4&
PELS063
\\
58.045849&24.156031&13.801$\pm$0.019&13.167$\pm$0.028&12.928$\pm$0.021&AAA2&
\nodata&\nodata&15.20&19&
BPL256
\\
58.046703&20.876076&13.498$\pm$0.020&12.881$\pm$0.024&12.603$\pm$0.025&AAA1&
\nodata&\nodata&15.50&22&
DH743
\\
58.050766&26.369192&12.236$\pm$0.019&11.652$\pm$0.029&11.423$\pm$0.019&AAA1&
\nodata&\nodata&14.01&22&
HCG452 DH744
\\
58.054920&26.196014&12.221$\pm$0.019&11.562$\pm$0.028&11.324$\pm$0.016&AAA1&
\nodata&\nodata&13.89&22&
DH745
\\
58.055466&26.143641&12.728$\pm$0.019&12.102$\pm$0.030&11.831$\pm$0.017&AAA1&
\nodata&16.33&14.17&20&
HCG451 SK197 DH746
\\
58.062492&24.339924&12.141$\pm$0.019&11.396$\pm$0.029&11.186$\pm$0.021&AAA2&
\nodata&\nodata&13.51&19&
BPL257
\\
58.063240&27.943844&14.867$\pm$0.041&14.245$\pm$0.051&14.032$\pm$0.048&AAA1&
\nodata&\nodata&16.40&22&
DH747
\\
58.071835&24.400221&8.599$\pm$0.025&8.087$\pm$0.047&7.918$\pm$0.013&AAA1&11.28&
10.66&\nodata&4&
PELS126 AKIII361
\\
58.072659&25.103350&14.048$\pm$0.025&13.417$\pm$0.031&13.137$\pm$0.031&AAA1&
\nodata&\nodata&15.62&19&
BPL258
\\
58.073093&24.455492&13.319$\pm$0.020&12.711$\pm$0.029&12.478$\pm$0.020&AAA2&
\nodata&\nodata&15.03&19&
BPL259 DH748
\\
58.076874&22.014896&12.290$\pm$0.016&11.621$\pm$0.018&11.390$\pm$0.020&AAA1&
\nodata&\nodata&13.50&22&
DH749
\\
58.077957&23.876900&14.034$\pm$0.021&13.469$\pm$0.030&13.194$\pm$0.025&AAA2&
\nodata&\nodata&15.65&19&
BPL260
\\
58.086052&24.565498&12.050$\pm$0.019&11.368$\pm$0.026&11.148$\pm$0.019&AAA2&
16.93&15.44&13.27&1&
HCG454 SK188 T159 DH750
\\
58.107998&21.842197&13.094$\pm$0.020&12.419$\pm$0.023&12.180$\pm$0.022&AAA1&
\nodata&\nodata&14.51&22&
DH752
\\
58.127197&19.677778&13.426$\pm$0.022&12.829$\pm$0.027&12.560$\pm$0.022&AAA1&
\nodata&\nodata&15.88&22&
DH753
\\
58.128777&24.544367&12.449$\pm$0.019&11.813$\pm$0.027&11.528$\pm$0.019&AAA2&
\nodata&17.56&13.93&20&
HCG456 SK178 BPL261 DH754
\\
58.130680&25.252174&12.779$\pm$0.025&12.152$\pm$0.030&11.910$\pm$0.020&AAA1&
\nodata&16.70&14.16&20&
SK179 BPL262 DH755
\\
58.131577&25.330528&15.243$\pm$0.044&14.682$\pm$0.060&14.362$\pm$0.055&AAA1&
\nodata&\nodata&16.85&19&
BPL263
\\
58.138905&23.851933&13.425$\pm$0.020&12.811$\pm$0.028&12.541$\pm$0.024&AAA2&
\nodata&\nodata&14.94&19&
BPL264 DH756
\\
58.143593&22.502174&12.290$\pm$0.020&11.609$\pm$0.021&11.390$\pm$0.016&AAA1&
\nodata&15.79&13.55&5&
HCG458 SK174 sk174 DH757
\\
58.147133&25.017994&13.629$\pm$0.023&13.049$\pm$0.030&12.724$\pm$0.026&AAA1&
\nodata&\nodata&15.52&19&
BPL265 DH758
\\
58.149204&21.356459&13.619$\pm$0.022&12.997$\pm$0.027&12.773$\pm$0.025&AAA1&
\nodata&\nodata&15.52&22&
DH759
\\
58.162125&25.840460&13.129$\pm$0.021&12.502$\pm$0.029&12.215$\pm$0.019&AAA1&
99.99&17.80&14.80&21&
HCG461 HHJ244 DH760
\\
58.174236&26.769659&13.859$\pm$0.029&13.338$\pm$0.037&13.061$\pm$0.026&AAA1&
\nodata&\nodata&15.75&22&
DH761
\\
58.175800&25.178453&14.608$\pm$0.037&13.984$\pm$0.051&13.765$\pm$0.048&AAA1&
\nodata&\nodata&16.32&22&
DH762
\\
58.180122&24.466312&13.721$\pm$0.026&13.146$\pm$0.033&12.931$\pm$0.025&AAA1&
\nodata&\nodata&15.41&19&
BPL266 DH763
\\
58.181084&27.472492&14.806$\pm$0.033&14.173$\pm$0.047&13.918$\pm$0.055&AAA1&
\nodata&\nodata&16.15&22&
DH764
\\
58.184498&23.904209&14.555$\pm$0.032&13.976$\pm$0.046&13.658$\pm$0.045&AAA1&
\nodata&\nodata&16.20&19&
BPL267 DH765
\\
58.185287&24.349888&13.987$\pm$0.026&13.365$\pm$0.035&13.134$\pm$0.038&AAA1&
\nodata&\nodata&15.72&19&
BPL268 DH766
\\
58.188946&25.279867&11.252$\pm$0.019&10.589$\pm$0.030&10.521$\pm$0.019&AAA1&
\nodata&\nodata&12.47&22&
DH767
\\
58.190258&21.688936&12.852$\pm$0.020&12.198$\pm$0.020&11.957$\pm$0.018&AAA1&
\nodata&\nodata&14.55&22&
DH768
\\
58.193481&24.561449&13.522$\pm$0.021&12.917$\pm$0.031&12.655$\pm$0.025&AAA1&
\nodata&\nodata&15.20&19&
BPL270
\\
58.202885&21.707870&11.565$\pm$0.019&10.867$\pm$0.018&10.656$\pm$0.015&AAA1&
\nodata&\nodata&12.58&22&
HCG460 DH769
\\
58.215458&22.525869&12.823$\pm$0.019&12.151$\pm$0.021&11.911$\pm$0.016&AAA1&
\nodata&16.90&14.40&21&
HCG462 SK150 HHJ302 DH770
\\
58.215733&23.563438&14.783$\pm$0.037&14.072$\pm$0.039&13.785$\pm$0.046&AAA1&
\nodata&\nodata&16.60&21&
HHJ22 BPL272
\\
58.217064&25.174004&12.384$\pm$0.021&11.747$\pm$0.027&11.532$\pm$0.023&AAA1&
\nodata&16.01&13.73&20&
BPL273 SK152
\\
58.220840&21.781960&9.991$\pm$0.019&9.468$\pm$0.018&9.349$\pm$0.016&AAA1&12.50&
11.65&\nodata&4&
PELS069
\\
58.226009&25.295425&13.339$\pm$0.021&12.727$\pm$0.031&12.462$\pm$0.021&AAA1&
\nodata&18.02&15.08&20&
HCG464 SK151 BPL274 DH771
\\
58.232986&24.961664&15.112$\pm$0.043&14.539$\pm$0.071&14.317$\pm$0.062&AAA1&
\nodata&\nodata&16.99&19&
BPL275
\\
58.237335&22.433760&12.449$\pm$0.020&11.835$\pm$0.018&11.574$\pm$0.018&AAA1&
\nodata&15.94&13.69&20&
HCG463 SK143 HHJ358 DH772
\\
58.242149&21.424252&12.986$\pm$0.020&12.285$\pm$0.020&12.067$\pm$0.019&AAA1&
\nodata&\nodata&14.82&22&
DH773
\\
58.243122&21.088999&13.489$\pm$0.022&12.868$\pm$0.023&12.548$\pm$0.021&AAA1&
\nodata&\nodata&15.53&22&
DH774
\\
58.244881&25.438709&14.244$\pm$0.026&13.611$\pm$0.041&13.333$\pm$0.029&AAA1&
\nodata&\nodata&15.94&19&
BPL277
\\
58.246410&24.901539&11.600$\pm$0.017&10.888$\pm$0.027&10.707$\pm$0.018&AAA1&
\nodata&14.40&12.59&5&
SK145 DH775
\\
58.256760&22.980156&13.476$\pm$0.020&12.794$\pm$0.026&12.536$\pm$0.022&AAA1&
\nodata&18.10&15.10&21&
HHJ181 DH776
\\
58.259853&21.660198&9.313$\pm$0.019&8.965$\pm$0.051&8.833$\pm$0.015&AAA1&11.53&
10.72&\nodata&9&
AKV088
\\
58.268860&22.801392&11.177$\pm$0.019&10.538$\pm$0.020&10.376$\pm$0.015&AAA1&
\nodata&\nodata&11.99&22&
DH777
\\
58.271339&25.071041&14.806$\pm$0.038&14.185$\pm$0.044&13.854$\pm$0.049&AAA1&
\nodata&\nodata&16.80&21&
HHJ13 BPL278
\\
58.280315&25.789351&14.248$\pm$0.029&13.737$\pm$0.045&13.303$\pm$0.041&AAA1&
\nodata&20.40&16.10&21&
HHJ53 DH778
\\
58.281132&25.300993&14.574$\pm$0.040&13.899$\pm$0.040&13.591$\pm$0.042&AAA1&
\nodata&\nodata&16.41&19&
BPL279
\\
58.290108&23.563335&14.856$\pm$0.032&14.268$\pm$0.055&13.870$\pm$0.052&AAA1&
\nodata&\nodata&16.50&19&
BPL280
\\
58.292313&23.053041&12.578$\pm$0.020&11.952$\pm$0.021&11.668$\pm$0.016&AAA1&
\nodata&16.40&14.20&21&
HHJ330 DH779
\\
58.308289&19.716618&14.851$\pm$0.034&14.212$\pm$0.044&13.912$\pm$0.049&AAA1&
\nodata&\nodata&17.01&22&
DH780
\\
58.315392&22.870745&12.645$\pm$0.018&12.032$\pm$0.018&11.784$\pm$0.017&AAA1&
18.50&16.83&14.15&1&
HCG467 SK134 B369 HHJ323
\\
58.318481&23.349569&14.147$\pm$0.025&13.532$\pm$0.033&13.212$\pm$0.028&AAA1&
\nodata&\nodata&15.71&19&
BPL281
\\
58.339966&23.981735&12.672$\pm$0.021&12.049$\pm$0.027&11.773$\pm$0.019&AAA1&
\nodata&16.38&14.03&20&
SK132 DH782
\\
58.340286&24.057455&14.185$\pm$0.028&13.636$\pm$0.041&13.248$\pm$0.030&AAA1&
\nodata&\nodata&15.81&19&
BPL282
\\
58.346313&23.322317&16.043$\pm$0.085&15.279$\pm$0.112&14.745$\pm$0.103&ABA1&
\nodata&\nodata&18.34&19&
BPL283
\\
58.347252&25.097382&15.503$\pm$0.048&14.958$\pm$0.068&14.627$\pm$0.076&AAA1&
\nodata&\nodata&17.16&19&
BPL284
\\
58.348740&24.065062&9.949$\pm$0.018&9.564$\pm$0.026&9.439$\pm$0.019&AAA1&12.30&
11.49&\nodata&4&
PELS071 DH783 AKIb694
\\
58.350426&23.799654&13.394$\pm$0.019&12.775$\pm$0.023&12.553$\pm$0.022&AAA1&
\nodata&18.10&15.20&20&
HHJ173 BPL285 DH784
\\
58.352043&25.035339&13.418$\pm$0.024&12.844$\pm$0.032&12.552$\pm$0.025&AAA1&
\nodata&\nodata&15.07&19&
HCG471 HHJ170 BPL286 DH785
\\
58.353428&23.404202&11.488$\pm$0.019&10.787$\pm$0.020&10.601$\pm$0.015&AAA1&
\nodata&\nodata&12.77&22&
DH786
\\
58.378120&19.906799&12.788$\pm$0.018&12.115$\pm$0.020&11.862$\pm$0.018&AAA1&
\nodata&\nodata&14.67&22&
DH787
\\
58.380608&26.528090&9.945$\pm$0.019&9.427$\pm$0.027&9.242$\pm$0.020&AAA1&12.81&
11.90&\nodata&4&
PELS075 DH788 AKIV287
\\
58.381493&20.957546&13.790$\pm$0.019&13.176$\pm$0.027&12.921$\pm$0.028&AAA1&
\nodata&\nodata&15.82&22&
DH789
\\
58.393925&24.077295&15.592$\pm$0.063&14.880$\pm$0.073&14.826$\pm$0.099&AAA1&
\nodata&\nodata&17.18&19&
BPL287
\\
58.397949&26.118980&13.658$\pm$0.026&13.069$\pm$0.031&12.788$\pm$0.026&AAA1&
\nodata&19.00&15.60&21&
HHJ124 DH790
\\
58.420631&24.419390&12.499$\pm$0.017&11.831$\pm$0.027&11.583$\pm$0.022&AAA1&
\nodata&15.72&13.82&20&
HCG473 SK122 HHJ372 BPL288
\\
58.429241&20.833517&11.633$\pm$0.016&10.936$\pm$0.020&10.764$\pm$0.016&AAA1&
\nodata&\nodata&12.87&22&
DH792
\\
58.435505&24.011810&15.409$\pm$0.050&14.754$\pm$0.064&14.426$\pm$0.073&AAA1&
\nodata&\nodata&16.81&19&
BPL289
\\
58.448269&23.741959&13.181$\pm$0.019&12.582$\pm$0.021&12.280$\pm$0.020&AAA1&
\nodata&17.64&14.65&7&
HCG474 SK115 HHJ237 BPL290
\\
58.450191&23.819414&14.433$\pm$0.030&13.760$\pm$0.030&13.513$\pm$0.035&AAA1&
\nodata&\nodata&16.50&21&
HHJ28 BPL291
\\
58.450592&23.970078&15.013$\pm$0.042&14.409$\pm$0.056&14.214$\pm$0.061&AAA1&
\nodata&\nodata&16.53&19&
BPL292
\\
58.454525&23.547169&15.203$\pm$0.046&14.688$\pm$0.067&14.346$\pm$0.073&AAA1&
\nodata&\nodata&16.92&19&
BPL293
\\
58.459431&25.964615&9.682$\pm$0.020&9.371$\pm$0.025&9.299$\pm$0.018&AAA1&11.82&
11.10&\nodata&4&
PELS083 DH793 AKIb710
\\
58.468555&22.626177&12.935$\pm$0.020&12.269$\pm$0.020&12.015$\pm$0.016&AAA1&
\nodata&17.91&14.88&20&
SK109
\\
58.470093&22.418575&10.113$\pm$0.016&9.554$\pm$0.020&9.406$\pm$0.016&AAA1&
\nodata&\nodata&11.24&22&
DH794
\\
58.479633&23.393435&15.141$\pm$0.045&14.555$\pm$0.061&14.077$\pm$0.060&AAA1&
\nodata&\nodata&17.61&19&
BPL294
\\
58.488640&23.345341&11.315$\pm$0.018&10.653$\pm$0.018&10.480$\pm$0.016&AAA1&
15.60&14.26&12.48&1&
HCG477 SK106 T61
\\
58.492168&20.480457&11.831$\pm$0.019&11.160$\pm$0.018&10.920$\pm$0.018&AAA1&
\nodata&\nodata&13.21&22&
DH795
\\
58.492580&24.419182&15.288$\pm$0.054&14.645$\pm$0.064&14.261$\pm$0.064&AAA1&
\nodata&\nodata&17.23&19&
BPL295
\\
58.499687&23.683434&15.109$\pm$0.045&14.481$\pm$0.058&14.148$\pm$0.060&AAA1&
\nodata&\nodata&16.57&19&
BPL296
\\
58.501556&24.580564&14.829$\pm$0.036&14.223$\pm$0.051&13.895$\pm$0.044&AAA1&
\nodata&\nodata&16.69&19&
BPL297
\\
58.502895&23.983335&12.730$\pm$0.018&12.141$\pm$0.026&11.849$\pm$0.022&AAA1&
\nodata&17.00&14.30&21&
HHJ322 BPL298
\\
58.504658&23.328106&14.786$\pm$0.033&14.207$\pm$0.047&13.883$\pm$0.053&AAA1&
\nodata&\nodata&16.70&21&
HHJ20 BPL299
\\
58.504856&25.331059&15.149$\pm$0.043&14.576$\pm$0.059&14.262$\pm$0.059&AAA1&
\nodata&\nodata&16.97&19&
BPL300
\\
58.511341&23.583694&13.902$\pm$0.025&13.246$\pm$0.028&12.982$\pm$0.027&AAA1&
\nodata&\nodata&15.52&19&
BPL301
\\
58.522190&23.566603&16.518$\pm$0.152&15.776$\pm$0.167&15.287$\pm$0.171&BCC1&
\nodata&\nodata&19.43&19&
BPL303
\\
58.537193&24.333645&10.376$\pm$0.020&9.845$\pm$0.030&9.721$\pm$0.022&AAA1&13.51&
12.49&\nodata&9&
AKIV314
\\
58.547848&25.311954&13.628$\pm$0.027&13.002$\pm$0.029&12.723$\pm$0.028&AAA1&
\nodata&\nodata&15.25&19&
HCG484 BPL304 DH796
\\
58.554211&23.347506&12.664$\pm$0.018&12.053$\pm$0.020&11.809$\pm$0.019&AAA1&
\nodata&16.46&13.92&20&
HCG482 SK97 HHJ325 BPL305 DH797
\\
58.556320&20.977406&14.453$\pm$0.030&13.923$\pm$0.035&13.564$\pm$0.041&AAA1&
\nodata&\nodata&16.57&22&
DH798
\\
58.559036&25.632647&12.906$\pm$0.021&12.278$\pm$0.028&12.012$\pm$0.022&AAA1&
\nodata&16.41&14.22&20&
SK99 HHJ318
\\
58.563656&25.164530&16.198$\pm$0.103&15.531$\pm$0.127&14.946$\pm$0.122&ABB1&
\nodata&\nodata&18.84&19&
BPL306
\\
58.564999&24.346058&14.734$\pm$0.034&14.068$\pm$0.049&13.706$\pm$0.045&AAA1&
\nodata&\nodata&16.51&19&
BPL307
\\
58.565193&25.355280&14.506$\pm$0.034&13.829$\pm$0.039&13.509$\pm$0.037&AAA1&
\nodata&\nodata&16.29&19&
BPL309
\\
58.569950&22.004671&14.951$\pm$0.038&14.315$\pm$0.051&14.106$\pm$0.056&AAA1&
\nodata&\nodata&16.76&22&
DH799
\\
58.578457&25.495296&10.479$\pm$0.015&10.028$\pm$0.036&9.805$\pm$0.022&AAE1&
\nodata&\nodata&10.98&22&
DH800
\\
58.588425&23.396976&12.957$\pm$0.019&12.322$\pm$0.020&12.066$\pm$0.019&AAA1&
\nodata&\nodata&14.34&19&
BPL310
\\
58.589973&24.075645&8.687$\pm$0.013&8.480$\pm$0.031&8.424$\pm$0.019&AAA1&10.29&
9.75&\nodata&9&
AK1A317 HD24463
\\
58.593632&23.636736&13.468$\pm$0.021&12.825$\pm$0.026&12.574$\pm$0.023&AAA1&
\nodata&18.00&15.00&21&
HHJ214 BPL311 DH801
\\
58.604294&24.712147&13.702$\pm$0.027&13.074$\pm$0.033&12.758$\pm$0.030&AAA1&
\nodata&\nodata&15.49&19&
HCG487 HHJ131 BPL312 DH802
\\
58.615952&21.389771&9.601$\pm$0.018&9.255$\pm$0.020&9.183$\pm$0.016&AAA1&11.71&
10.97&\nodata&4&
PELS078 AKV136
\\
58.616493&23.835423&10.473$\pm$0.018&9.837$\pm$0.018&9.663$\pm$0.016&AAA1&
\nodata&13.04&11.42&5&
HCG489
\\
58.617119&23.943441&14.607$\pm$0.032&13.964$\pm$0.040&13.747$\pm$0.043&AAA1&
\nodata&\nodata&16.22&19&
BPL313
\\
58.618523&24.321157&11.449$\pm$0.015&10.784$\pm$0.026&10.620$\pm$0.018&AAA1&
\nodata&\nodata&12.58&22&
DH803
\\
58.640049&25.678812&11.259$\pm$0.015&10.592$\pm$0.027&10.369$\pm$0.019&AAA1&
16.19&14.72&12.55&1&
HCG491 SK 91 B127
\\
58.644974&21.883942&12.061$\pm$0.016&11.369$\pm$0.018&11.178$\pm$0.016&AAA1&
\nodata&\nodata&13.33&22&
HCG488 DH804
\\
58.655624&23.225822&13.421$\pm$0.021&12.758$\pm$0.023&12.546$\pm$0.018&AAA1&
\nodata&\nodata&15.38&22&
DH805
\\
58.662998&24.598509&14.609$\pm$0.033&13.976$\pm$0.046&13.770$\pm$0.044&AAA1&
\nodata&\nodata&16.33&19&
BPL315 DH806
\\
58.684135&25.253107&15.954$\pm$0.075&15.406$\pm$0.098&14.879$\pm$0.104&AAA1&
\nodata&\nodata&18.08&19&
BPL316
\\
58.691074&22.898666&16.668$\pm$0.130&15.753$\pm$0.124&15.544$\pm$0.187&BBC1&
\nodata&\nodata&18.27&22&
DH807
\\
58.693207&25.049849&14.166$\pm$0.037&13.762$\pm$0.055&13.340$\pm$0.052&AAA1&
\nodata&\nodata&15.74&19&
BPL317
\\
58.693855&25.526451&13.565$\pm$0.022&12.979$\pm$0.035&12.683$\pm$0.026&AAA1&
\nodata&\nodata&15.67&22&
DH808
\\
58.699924&25.208462&12.601$\pm$0.017&11.949$\pm$0.028&11.759$\pm$0.023&AAA1&
\nodata&\nodata&13.76&22&
SK82 HHJ371 BPL318 DH809
\\
58.718990&24.576248&10.635$\pm$0.018&9.991$\pm$0.019&9.831$\pm$0.013&AAA1&
\nodata&13.10&11.25&20&
HCG495
\\
58.730572&22.994583&14.235$\pm$0.024&13.617$\pm$0.027&13.275$\pm$0.033&AAA1&
\nodata&19.80&16.00&21&
HHJ62
\\
58.732224&25.151196&14.012$\pm$0.024&13.448$\pm$0.021&13.166$\pm$0.031&AAA1&
\nodata&\nodata&15.55&19&
BPL320
\\
58.741772&25.241491&12.907$\pm$0.020&12.240$\pm$0.021&11.982$\pm$0.020&AAA1&
\nodata&16.87&14.30&20&
SK76 BPL321 DH810
\\
58.765316&25.221357&14.187$\pm$0.027&13.616$\pm$0.021&13.255$\pm$0.034&AAA1&
\nodata&\nodata&15.76&19&
BPL322
\\
58.773853&23.054785&16.053$\pm$0.077&15.356$\pm$0.102&14.913$\pm$0.116&AAB1&
\nodata&\nodata&18.24&22&
DH811
\\
58.775589&25.185064&14.369$\pm$0.032&13.846$\pm$0.032&13.553$\pm$0.038&AAA1&
\nodata&\nodata&16.08&19&
BPL323
\\
58.787357&24.084129&12.774$\pm$0.018&12.142$\pm$0.021&11.886$\pm$0.019&AAA1&
\nodata&17.10&14.00&21&
SK65 HHJ313 BPL324 DH812
\\
58.799313&22.967484&13.921$\pm$0.024&13.232$\pm$0.027&12.921$\pm$0.022&AAA1&
\nodata&19.90&16.00&21&
HHJ61
\\
58.806763&19.504728&12.615$\pm$0.021&11.936$\pm$0.025&11.721$\pm$0.019&AAA1&
\nodata&\nodata&14.58&22&
DH813
\\
58.821526&23.888103&15.244$\pm$0.046&14.804$\pm$0.065&14.344$\pm$0.081&AAA1&
\nodata&\nodata&17.14&19&
BPL325
\\
58.825424&24.284950&15.075$\pm$0.043&14.483$\pm$0.052&14.309$\pm$0.083&AAA1&
\nodata&\nodata&16.74&19&
BPL326
\\
58.836151&22.535803&13.970$\pm$0.024&13.236$\pm$0.025&13.060$\pm$0.030&AAA1&
\nodata&18.10&15.30&21&
HHJ144 DH814
\\
58.846134&24.818130&15.578$\pm$0.054&14.870$\pm$0.071&14.831$\pm$0.131&AAB1&
\nodata&\nodata&17.72&19&
BPL327
\\
58.862698&25.246149&14.728$\pm$0.034&14.027$\pm$0.035&13.691$\pm$0.042&AAA1&
\nodata&\nodata&16.66&19&
BPL328
\\
58.870853&23.772451&11.419$\pm$0.019&10.784$\pm$0.023&10.593$\pm$0.018&AAA1&
15.53&14.18&\nodata&4&
PELS192 HCG498
\\
58.878731&23.397556&13.088$\pm$0.021&12.426$\pm$0.021&12.176$\pm$0.020&AAA1&
\nodata&17.21&14.44&20&
SK54 HHJ284 BPL329 DH815
\\
58.883072&21.079517&9.624$\pm$0.021&9.281$\pm$0.020&9.174$\pm$0.016&AAA1&11.83&
11.04&\nodata&4&
PELS079 AKV168
\\
58.887638&20.625212&13.793$\pm$0.026&13.157$\pm$0.028&12.921$\pm$0.030&AAA1&
\nodata&\nodata&15.40&22&
DH817
\\
58.891022&22.808905&11.338$\pm$0.019&10.672$\pm$0.025&10.442$\pm$0.019&AAA1&
16.13&14.63&12.62&1&
HCG499 T99 SK48
\\
58.893406&23.974606&14.135$\pm$0.025&13.498$\pm$0.024&13.263$\pm$0.035&AAA1&
\nodata&19.60&15.80&20&
HHJ78 BPL330 DH818
\\
58.943188&23.354513&12.360$\pm$0.023&11.689$\pm$0.022&11.489$\pm$0.022&AAA1&
\nodata&15.53&13.45&5&
SK40
\\
58.953022&23.926773&11.326$\pm$0.020&10.639$\pm$0.019&10.440$\pm$0.015&AAA1&
\nodata&13.79&11.69&20&
HCG502
\\
58.955402&24.896549&15.447$\pm$0.059&14.674$\pm$0.056&14.401$\pm$0.079&AAA1&
\nodata&\nodata&17.38&19&
BPL331
\\
58.957886&23.806326&14.628$\pm$0.036&13.969$\pm$0.036&13.724$\pm$0.040&AAA1&
\nodata&\nodata&16.20&19&
BPL332
\\
58.958714&21.724493&12.155$\pm$0.023&11.519$\pm$0.023&11.286$\pm$0.020&AAA1&
\nodata&\nodata&13.62&22&
DH819
\\
58.970905&20.278891&15.704$\pm$0.064&14.959$\pm$0.061&14.889$\pm$0.114&AAB1&
\nodata&\nodata&17.71&22&
DH820
\\
58.978748&20.131992&13.028$\pm$0.021&12.395$\pm$0.025&12.144$\pm$0.018&AAA1&
\nodata&\nodata&14.92&22&
DH821
\\
58.983471&23.567274&10.651$\pm$0.021&10.119$\pm$0.025&10.009$\pm$0.018&AAA1&
13.75&12.68&\nodata&4&
PELS114
\\
58.985050&25.300072&12.647$\pm$0.021&11.943$\pm$0.019&11.722$\pm$0.021&AAA1&
\nodata&16.23&13.83&20&
HCG504 SK37 DH822
\\
58.989742&21.177528&12.654$\pm$0.023&12.016$\pm$0.024&11.761$\pm$0.020&AAA1&
\nodata&\nodata&14.28&22&
DH823
\\
58.993286&24.549946&10.665$\pm$0.024&10.118$\pm$0.026&9.921$\pm$0.017&EEE1&13.77
&12.68&\nodata&4&
PELS115 DH824
\\
58.995129&24.961174&13.041$\pm$0.020&12.387$\pm$0.021&12.148$\pm$0.019&AAA1&
\nodata&17.80&14.70&21&
HHJ260 BPL333 DH825
\\
58.999664&26.999975&13.817$\pm$0.021&13.225$\pm$0.026&12.971$\pm$0.032&AAA1&
\nodata&\nodata&15.51&22&
DH826
\\
59.005959&23.126360&8.014$\pm$0.024&7.801$\pm$0.029&7.681$\pm$9.995&AAF1&9.62&
9.08&\nodata&8&
TrS183x HD24665
\\
59.024178&22.439503&10.936$\pm$0.021&10.297$\pm$0.025&10.161$\pm$0.019&AAA1&
\nodata&\nodata&11.88&22&
DH827
\\
59.046284&22.221218&9.906$\pm$0.021&9.524$\pm$0.024&9.414$\pm$0.020&AAA1&12.51&
11.63&\nodata&4&
PELS089 DH828 AKV201
\\
59.047169&20.575085&12.694$\pm$0.019&12.048$\pm$0.027&11.840$\pm$0.020&AAA1&
\nodata&\nodata&14.44&22&
DH829
\\
59.047417&25.060209&15.306$\pm$0.049&14.612$\pm$0.052&14.227$\pm$0.073&AAA1&
\nodata&\nodata&17.20&19&
BPL334
\\
59.051270&21.040857&9.440$\pm$0.021&9.074$\pm$0.021&8.967$\pm$0.018&AAA1&11.57&
10.86&\nodata&9&
AKV198
\\
59.053288&25.762081&9.166$\pm$0.022&8.914$\pm$0.023&8.830$\pm$0.018&AAA1&11.14&
10.47&\nodata&8&
TrS184x HD283132
\\
59.065811&25.487654&13.563$\pm$0.022&12.942$\pm$0.029&12.682$\pm$0.031&AAA1&
\nodata&\nodata&15.29&19&
BPL335
\\
59.077461&23.964449&12.175$\pm$0.017&11.508$\pm$0.023&11.277$\pm$0.015&AAA1&
\nodata&15.80&13.44&5&
SK22 HHJ386 DH830
\\
59.090511&25.352919&15.335$\pm$0.046&14.670$\pm$0.062&14.301$\pm$0.080&AAA1&
\nodata&\nodata&17.18&19&
BPL336
\\
59.092937&21.121443&12.938$\pm$0.021&12.308$\pm$0.025&12.016$\pm$0.020&AAA1&
\nodata&\nodata&14.55&22&
DH831
\\
59.093071&24.623196&16.158$\pm$0.095&15.788$\pm$0.162&15.578$\pm$0.250&ACD1&
\nodata&\nodata&17.88&22&
DH832
\\
59.097885&24.832436&11.374$\pm$0.016&10.711$\pm$0.023&10.547$\pm$0.014&AAA1&
\nodata&\nodata&12.40&22&
HCG508 DH833
\\
59.104092&23.090816&11.967$\pm$0.021&11.304$\pm$0.020&11.078$\pm$0.015&AAA1&
\nodata&15.15&13.07&5&
SK17 HHJ419
\\
59.108036&24.280998&11.913$\pm$0.017&11.177$\pm$0.018&11.011$\pm$0.018&AAA1&
\nodata&15.03&13.00&5&
SK18 HHJ416 DH834
\\
59.109142&23.784336&9.846$\pm$0.023&9.505$\pm$0.025&9.394$\pm$0.018&AAA1&\nodata
&\nodata&10.44&22&
DH835
\\
59.115120&26.065916&12.868$\pm$0.021&12.179$\pm$0.019&12.032$\pm$0.020&AAA1&
\nodata&\nodata&14.04&22&
DH836
\\
59.120422&24.031782&13.530$\pm$0.018&12.864$\pm$0.019&12.638$\pm$0.024&AAA1&
\nodata&17.90&15.20&21&
HHJ165 DH837
\\
59.142506&24.253668&16.524$\pm$0.127&15.796$\pm$0.145&15.372$\pm$0.211&BBC1&
\nodata&\nodata&18.19&22&
DH838
\\
59.150787&25.301619&14.710$\pm$0.036&14.101$\pm$0.032&13.813$\pm$0.054&AAA1&
\nodata&\nodata&16.46&19&
BPL337
\\
59.150848&20.118635&14.421$\pm$0.027&13.906$\pm$0.033&13.507$\pm$0.035&AAA1&
\nodata&\nodata&16.62&22&
DH839
\\
59.161442&21.585737&13.827$\pm$0.023&13.280$\pm$0.028&12.904$\pm$0.023&AAA1&
\nodata&\nodata&15.69&22&
DH841
\\
59.163898&24.528498&15.103$\pm$0.042&14.425$\pm$0.038&14.236$\pm$0.076&AAA1&
\nodata&\nodata&16.61&19&
BPL338
\\
59.165241&22.686749&15.674$\pm$0.065&14.906$\pm$0.066&14.776$\pm$0.093&AAA1&
\nodata&\nodata&17.74&22&
DH842
\\
59.194107&26.350218&13.984$\pm$0.024&13.372$\pm$0.033&13.052$\pm$0.031&AAA1&
\nodata&19.40&15.90&21&
HHJ64 DH843
\\
59.213776&25.040400&12.434$\pm$0.020&11.814$\pm$0.023&11.510$\pm$0.019&AAA1&
\nodata&\nodata&13.66&19&
BPL339
\\
59.217941&25.168154&14.829$\pm$0.035&14.199$\pm$0.039&13.975$\pm$0.053&AAA1&
\nodata&20.74&16.77&7&
HHJ17
\\
59.219707&20.083649&8.006$\pm$0.033&7.967$\pm$0.057&7.874$\pm$0.015&AAA1&\nodata
&\nodata&9.18&22&
DH845
\\
59.220394&23.428883&13.049$\pm$0.024&12.411$\pm$0.021&12.143$\pm$0.022&AAA1&
\nodata&17.60&14.60&21&
HHJ271 DH846
\\
59.231079&22.140184&14.150$\pm$0.023&13.472$\pm$0.022&13.269$\pm$0.035&AAA1&
\nodata&\nodata&16.04&22&
DH847
\\
59.237843&24.809643&12.158$\pm$0.017&11.453$\pm$0.019&11.228$\pm$0.015&AAA1&
99.99&16.10&13.60&21&
HCG511 HHJ393 DH848
\\
59.273804&22.820873&14.258$\pm$0.026&13.565$\pm$0.029&13.325$\pm$0.033&AAA1&
\nodata&\nodata&15.80&21&
HHJ85
\\
59.285778&20.128660&14.609$\pm$0.026&13.973$\pm$0.042&13.716$\pm$0.047&AAA1&
\nodata&\nodata&16.76&22&
DH849
\\
59.290844&21.607683&13.535$\pm$0.023&12.895$\pm$0.028&12.633$\pm$0.025&AAA1&
\nodata&\nodata&15.48&22&
DH850
\\
59.320171&24.009230&10.664$\pm$0.020&10.082$\pm$0.021&9.945$\pm$0.018&AAA1&
\nodata&\nodata&11.63&22&
DH851
\\
59.383339&22.433409&13.324$\pm$0.018&12.649$\pm$0.024&12.340$\pm$0.021&AAA1&
\nodata&\nodata&15.28&22&
DH852
\\
59.388798&24.053190&10.454$\pm$0.020&9.965$\pm$0.019&9.861$\pm$0.013&AAA1&13.06&
12.11&\nodata&4&
PELS162 DH853
\\
59.394142&22.925766&11.428$\pm$0.023&10.773$\pm$0.025&10.642$\pm$0.020&AAA1&
\nodata&\nodata&12.51&22&
DH854
\\
59.400311&23.931246&11.693$\pm$0.021&10.928$\pm$0.021&10.767$\pm$0.018&AAA1&
\nodata&\nodata&13.10&21&
HHJ439 DH855
\\
59.419441&25.267883&12.733$\pm$0.021&12.108$\pm$0.021&11.816$\pm$0.021&AAA1&
\nodata&\nodata&14.38&22&
DH856
\\
59.429035&25.385271&13.456$\pm$0.020&12.833$\pm$0.025&12.569$\pm$0.027&AAA1&
99.99&\nodata&15.10&21&
HCG516 HHJ180 DH857
\\
59.455681&22.142042&14.884$\pm$0.034&14.253$\pm$0.041&13.900$\pm$0.053&AAA1&
\nodata&\nodata&17.00&21&
HHJ7 DH858
\\
59.468094&21.037834&13.648$\pm$0.018&13.008$\pm$0.024&12.734$\pm$0.023&AAA1&
\nodata&\nodata&15.58&22&
DH859
\\
59.482658&21.269764&14.456$\pm$0.027&13.781$\pm$0.032&13.529$\pm$0.036&AAA1&
\nodata&\nodata&16.16&22&
DH860
\\
59.493687&24.335808&16.424$\pm$0.112&15.682$\pm$0.138&15.641$\pm$0.263&BBD1&
\nodata&\nodata&18.33&22&
DH861
\\
59.507069&20.676823&8.436$\pm$0.017&8.248$\pm$0.013&8.197$\pm$0.027&AAA1&10.13&
9.63&\nodata&4&
PELS086
\\
59.508156&23.898577&13.931$\pm$0.021&13.333$\pm$0.035&13.073$\pm$0.026&AAA1&
\nodata&\nodata&15.80&21&
HHJ84 DH862
\\
59.574600&20.452087&13.999$\pm$0.025&13.418$\pm$0.029&13.140$\pm$0.031&AAA1&
\nodata&\nodata&16.36&22&
DH863
\\
59.590111&21.257706&9.938$\pm$0.024&9.576$\pm$0.023&9.451$\pm$0.019&AAA1&12.28&
11.46&\nodata&9&
AKV308
\\
59.594700&21.899647&13.477$\pm$0.028&12.813$\pm$0.034&12.654$\pm$0.028&AAA1&
\nodata&\nodata&14.72&22&
DH864
\\
59.604721&24.016354&13.351$\pm$0.020&12.770$\pm$0.021&12.490$\pm$0.024&AAA1&
\nodata&\nodata&14.90&21&
HHJ220 DH865
\\
59.629074&23.070286&14.125$\pm$0.024&13.488$\pm$0.030&13.133$\pm$0.026&AAA1&
\nodata&\nodata&16.00&21&
HHJ60 DH866
\\
59.642365&22.669855&14.009$\pm$0.024&13.381$\pm$0.028&13.004$\pm$0.026&AAA1&
\nodata&\nodata&15.80&21&
HHJ93 DH867
\\
59.733913&23.464968&12.141$\pm$0.021&11.458$\pm$0.025&11.239$\pm$0.016&AAA1&
\nodata&\nodata&13.60&21&
HHJ388 DH868
\\
59.734997&24.309011&13.017$\pm$0.024&12.498$\pm$0.044&12.213$\pm$0.028&AAA1&
\nodata&\nodata&14.50&21&
HHJ292 DH869
\\
59.737621&23.708746&12.022$\pm$0.019&11.382$\pm$0.025&11.112$\pm$0.018&AAA1&
99.99&\nodata&13.50&21&
HCG519 HHJ411 DH870
\\
59.773869&26.407433&13.233$\pm$0.020&12.572$\pm$0.023&12.350$\pm$0.023&AAA1&
\nodata&\nodata&14.63&22&
DH871
\\
59.776257&25.055597&12.434$\pm$0.017&11.697$\pm$0.017&11.458$\pm$0.020&AAA1&
\nodata&\nodata&13.90&21&
HHJ366 DH872
\\
59.803818&24.288517&13.753$\pm$0.023&13.144$\pm$0.027&12.835$\pm$0.026&AAA1&
\nodata&\nodata&15.49&22&
DH873
\\
59.816074&25.902405&13.934$\pm$0.025&13.201$\pm$0.032&13.026$\pm$0.036&AAA1&
\nodata&\nodata&15.50&21&
HHJ133
\\
59.829075&23.523422&13.629$\pm$0.024&13.030$\pm$0.028&12.732$\pm$0.023&AAA1&
\nodata&\nodata&15.30&21&
HHJ150 DH874
\\
59.845402&22.571362&11.490$\pm$0.021&10.787$\pm$0.025&10.562$\pm$0.017&AAA1&
\nodata&\nodata&12.78&22&
DH875
\\
59.859776&22.356274&14.733$\pm$0.034&14.087$\pm$0.039&13.787$\pm$0.043&AAA1&
\nodata&\nodata&16.30&21&
HHJ39
\\
59.862160&21.805285&13.544$\pm$0.023&12.953$\pm$0.025&12.624$\pm$0.022&AAA1&
\nodata&\nodata&15.49&22&
DH876
\\
59.864700&23.123796&10.950$\pm$0.021&10.269$\pm$0.024&10.130$\pm$0.015&AAA1&
\nodata&\nodata&12.21&22&
DH877
\\
59.872150&21.665674&14.551$\pm$0.028&13.937$\pm$0.035&13.614$\pm$0.037&AAA1&
\nodata&\nodata&16.46&22&
DH878
\\
59.881058&21.271900&12.743$\pm$0.021&12.090$\pm$0.024&11.844$\pm$0.019&AAA1&
\nodata&\nodata&14.45&22&
DH879
\\
59.968391&22.366104&12.625$\pm$0.022&11.923$\pm$0.025&11.789$\pm$0.019&AAA1&
\nodata&\nodata&13.88&22&
DH880
\\
59.985321&23.671005&14.913$\pm$0.035&14.238$\pm$0.041&13.959$\pm$0.046&AAA1&
\nodata&\nodata&17.25&22&
DH882
\\
59.996426&23.684715&14.152$\pm$0.028&13.476$\pm$0.025&13.220$\pm$0.025&AAA1&
\nodata&\nodata&16.21&22&
DH883
\\
59.999355&22.091591&13.773$\pm$0.025&13.192$\pm$0.027&12.912$\pm$0.024&AAA1&
\nodata&\nodata&15.65&22&
DH884
\\
60.001587&23.785429&14.848$\pm$0.034&14.203$\pm$0.041&13.976$\pm$0.046&AAA1&
\nodata&\nodata&16.67&22&
DH885
\\
60.010517&26.600632&14.011$\pm$0.022&13.324$\pm$0.029&13.041$\pm$0.028&AAA1&
\nodata&\nodata&15.59&22&
DH886
\\
60.037495&24.057154&13.902$\pm$0.023&13.280$\pm$0.030&13.023$\pm$0.029&AAA1&
\nodata&\nodata&15.74&22&
DH887
\\
60.042843&22.038197&13.427$\pm$0.025&12.824$\pm$0.025&12.521$\pm$0.023&AAA1&
\nodata&\nodata&15.25&22&
DH888
\\
60.058750&24.814384&13.568$\pm$0.023&12.887$\pm$0.021&12.685$\pm$0.023&AAA1&
\nodata&\nodata&15.13&22&
DH889
\\
60.108917&23.438250&12.851$\pm$0.019&12.251$\pm$0.021&11.960$\pm$0.018&AAA1&
\nodata&\nodata&14.70&22&
DH891
\\
60.117409&23.856777&12.925$\pm$0.019&12.321$\pm$0.025&12.007$\pm$0.020&AAA1&
\nodata&\nodata&14.73&22&
DH892
\\
60.118103&27.348597&14.018$\pm$0.021&13.340$\pm$0.029&13.064$\pm$0.030&AAA1&
\nodata&\nodata&15.55&22&
DH893
\\
60.163445&26.738733&12.064$\pm$0.019&11.367$\pm$0.020&11.170$\pm$0.016&AAA1&
\nodata&\nodata&13.50&22&
DH894
\\
60.205482&25.203058&13.252$\pm$0.022&12.542$\pm$0.022&12.335$\pm$0.020&AAA1&
\nodata&\nodata&14.71&22&
DH895
\\
60.221325&23.193913&8.676$\pm$0.009&8.558$\pm$0.013&8.488$\pm$0.016&AAA1&10.06&
9.61&\nodata&4&
PELS173
\\
60.267197&20.372704&11.813$\pm$0.019&11.139$\pm$0.022&10.906$\pm$0.016&AAA1&
\nodata&\nodata&13.12&22&
DH896
\\
60.285774&22.956268&13.075$\pm$0.026&12.364$\pm$0.027&12.121$\pm$0.022&AAA1&
\nodata&\nodata&14.40&22&
DH897
\\
60.300270&23.903667&12.710$\pm$0.021&12.126$\pm$0.025&11.861$\pm$0.018&AAA1&
\nodata&\nodata&14.49&22&
DH898
\\
60.308235&23.175064&12.964$\pm$0.021&12.244$\pm$0.020&12.033$\pm$0.019&AAA1&
\nodata&\nodata&14.73&22&
DH899
\\
60.358501&21.585827&13.146$\pm$0.021&12.542$\pm$0.022&12.255$\pm$0.019&AAA1&
\nodata&\nodata&14.85&22&
DH900
\\
60.454834&22.168186&13.112$\pm$0.019&12.524$\pm$0.027&12.237$\pm$0.018&AAA1&
\nodata&\nodata&14.81&22&
DH901
\\
60.498222&25.320168&15.208$\pm$0.036&14.539$\pm$0.060&14.217$\pm$0.062&AAA1&
\nodata&\nodata&17.43&22&
DH902
\\
60.594200&24.806797&13.992$\pm$0.024&13.257$\pm$0.026&13.084$\pm$0.029&AAA1&
\nodata&\nodata&15.48&22&
DH903
\\
60.708202&23.510780&12.947$\pm$0.018&12.316$\pm$0.023&12.056$\pm$0.021&AAA1&
\nodata&\nodata&14.56&22&
DH904
\\
60.755016&25.406534&15.928$\pm$0.071&15.154$\pm$0.083&14.682$\pm$0.092&AAA1&
\nodata&\nodata&18.62&22&
DH905
\\
60.818947&24.588871&14.155$\pm$0.023&13.588$\pm$0.026&13.273$\pm$0.029&AAA1&
\nodata&\nodata&16.13&22&
DH906
\\
60.919399&25.359707&12.277$\pm$0.016&11.555$\pm$0.022&11.309$\pm$0.018&AAA1&
\nodata&\nodata&14.12&22&
DH908
\\
60.932632&23.896503&13.109$\pm$0.018&12.516$\pm$0.027&12.198$\pm$0.021&AAA1&
\nodata&\nodata&15.23&22&
DH909
\\
60.934029&22.944309&8.519$\pm$0.031&8.262$\pm$0.013&8.183$\pm$0.019&AAA1&10.25&
9.67&\nodata&4&
PELS174 AKV595
\\
60.956493&23.720613&13.886$\pm$0.026&13.255$\pm$0.029&12.996$\pm$0.025&AAA1&
\nodata&\nodata&15.79&22&
DH910
\\
61.147995&25.120106&10.470$\pm$0.020&10.003$\pm$0.029&9.947$\pm$0.026&AAE1&
\nodata&\nodata&11.42&22&
DH911
\\
61.190189&24.688738&12.736$\pm$0.021&12.062$\pm$0.029&11.768$\pm$0.026&AAA1&
\nodata&\nodata&14.95&22&
DH912
\\
61.307121&22.305193&13.367$\pm$0.020&12.719$\pm$0.023&12.412$\pm$0.021&AAA1&
\nodata&\nodata&15.69&22&
DH914
\\
61.307224&24.145317&13.963$\pm$0.027&13.341$\pm$0.039&12.978$\pm$0.035&AAA1&
\nodata&\nodata&16.23&22&
DH915
\\
\enddata
\tablenotetext{a}{Standard 2MASS photometric data quality flag for
$JH$\ks, in that order.  If the number following the 2MASS quality
flags is a 1, the 2MASS data come from the standard 2MASS catalog; if
it is a 2, the data come from the deep catalog.}
\tablerefs{
1 -- various Stauffer papers from 1980 through 1990 (\citet{stauffer80}, \citet{stauffer82},
       \citet{stauffer84}, \citet{stauffer87}, \citet{stauffer89}
2 -- \citet{landolt79}
3 -- \citet{jomi58} and/or \citet{iriarte67}
4 -- \citet{vanlee86}
5 -- \citet{prosser91}
6 -- \citet{festin98}
7 -- \citet{stauffer98}
8 -- \citet{rosvick92}
9 -- \citet{mermilliod97}
10 -- \citet{steele95}
11 -- average of photometry from (1) and from \citet{messina01}
12 -- average of data from (1), (5) and (10)
13 -- average of (1) and (3) for the \ic\ magnitude
14 -- average of \citet{messina01}, \citet{landolt79}, and \citet{vanlee86}
15 -- average of \citet{jomi58}, \citet{stauffer84}, \citet{vanlee86}, and \citet{messina01}
16 -- average of (1) and \citet{robinson74}
17 -- average of (1), \citet{messina01}, and \citet{robinson74}
18 -- average of (1) and (2)
19 -- from \citet{pinfield00}, but converted to \ic\ estimate as detailed above
20 -- photographic photometry from \citet{stauffer91}
21 -- photographic photometry from \citet{hambly93}
22 -- estimate of \ic\ derived from \citet{deacon04} as described above
23 -- estimate of \ic\ derived from \citet{slesnick06} as described above
}
\end{deluxetable}


==> table4_electronic.tex <==
\begin{deluxetable}{llllllll}
\tablecaption{Single-Star Pleiades Loci}
\tablewidth{0pt}
\tabletypesize{\scriptsize}
\tablehead{
\colhead{$B$} &  \colhead{$V$} &
\colhead{\ic} & \colhead{\ks} &
\colhead{[3.6]} &
\colhead{[4.5]} & \colhead{[5.8]} & 
\colhead{[8]} 
}
\startdata
6.598&6.600&6.574&6.592&6.602&6.615&6.602&6.602\\
6.706&6.700&6.665&6.671&6.682&6.695&6.682&6.682\\
6.814&6.800&6.755&6.750&6.761&6.775&6.762&6.762\\
6.922&6.900&6.848&6.834&6.841&6.855&6.841&6.841\\
7.030&7.000&6.940&6.910&6.920&6.935&6.921&6.921\\
7.142&7.100&7.030&6.982&6.990&7.005&6.991&6.991\\
7.254&7.200&7.115&7.039&7.050&7.064&7.050&7.049\\
7.370&7.300&7.200&7.104&7.109&7.124&7.108&7.107\\
7.490&7.400&7.283&7.162&7.168&7.183&7.165&7.164\\
7.610&7.500&7.367&7.228&7.238&7.252&7.233&7.231\\
7.730&7.600&7.450&7.287&7.297&7.311&7.291&7.288\\
7.850&7.700&7.533&7.345&7.347&7.360&7.339&7.336\\
7.968&7.800&7.615&7.387&7.396&7.409&7.387&7.384\\
8.084&7.900&7.698&7.428&7.436&7.449&7.426&7.422\\
8.200&8.000&7.780&7.469&7.475&7.488&7.465&7.460\\
8.320&8.100&7.840&7.508&7.515&7.527&7.503&7.498\\
8.440&8.200&7.900&7.546&7.555&7.567&7.542&7.536\\
8.564&8.300&7.975&7.591&7.594&7.606&7.580&7.575\\
8.692&8.400&8.050&7.648&7.654&7.665&7.638&7.632\\
8.820&8.500&8.125&7.701&7.703&7.715&7.687&7.680\\
8.936&8.600&8.200&7.762&7.762&7.774&7.744&7.737\\
9.052&8.700&8.275&7.815&7.812&7.823&7.793&7.785\\
9.168&8.800&8.350&7.876&7.881&7.892&7.860&7.851\\
9.284&8.900&8.425&7.929&7.931&7.941&7.909&7.899\\
9.400&9.000&8.500&7.990&7.990&8.000&7.966&7.957\\
9.516&9.100&8.583&8.048&8.049&8.059&8.026&8.016\\
9.632&9.200&8.667&8.112&8.108&8.118&8.085&8.075\\
9.750&9.300&8.750&8.170&8.168&8.178&8.145&8.135\\
9.870&9.400&8.840&8.242&8.236&8.246&8.214&8.204\\
9.990&9.500&8.930&8.314&8.305&8.315&8.284&8.274\\
10.102&9.600&9.020&8.384&8.374&8.384&8.353&8.343\\
10.214&9.700&9.103&8.442&8.433&8.443&8.413&8.403\\
10.328&9.800&9.185&8.500&8.493&8.503&8.472&8.462\\
10.444&9.900&9.268&8.564&8.552&8.562&8.532&8.522\\
10.560&10.000&9.350&8.622&8.611&8.621&8.591&8.581\\
10.680&10.100&9.437&8.687&8.680&8.690&8.661&8.651\\
10.800&10.200&9.523&8.746&8.739&8.749&8.720&8.710\\
10.920&10.300&9.610&8.818&8.808&8.818&8.790&8.780\\
11.040&10.400&9.696&8.890&8.877&8.887&8.859&8.849\\
11.160&10.500&9.782&8.950&8.936&8.946&8.918&8.908\\
11.272&10.600&9.867&9.012&8.995&9.005&8.978&8.968\\
11.384&10.700&9.952&9.066&9.054&9.063&9.036&9.026\\
11.500&10.800&10.035&9.119&9.104&9.111&9.085&9.074\\
11.620&10.900&10.118&9.174&9.153&9.160&9.133&9.122\\
11.740&11.000&10.198&9.224&9.203&9.208&9.182&9.170\\
11.860&11.100&10.273&9.267&9.252&9.257&9.231&9.218\\
11.980&11.200&10.353&9.317&9.302&9.305&9.279&9.267\\
12.100&11.300&10.439&9.373&9.351&9.354&9.328&9.315\\
12.220&11.400&10.524&9.423&9.401&9.402&9.376&9.363\\
12.340&11.500&10.610&9.480&9.460&9.461&9.435&9.421\\
12.456&11.600&10.680&9.525&9.499&9.500&9.474&9.460\\
12.572&11.700&10.750&9.570&9.547&9.549&9.523&9.509\\
12.688&11.800&10.820&9.612&9.586&9.588&9.562&9.549\\
12.804&11.900&10.905&9.660&9.634&9.637&9.611&9.598\\
12.920&12.000&10.990&9.714&9.682&9.686&9.659&9.647\\
13.040&12.100&11.065&9.756&9.730&9.735&9.708&9.696\\
13.160&12.200&11.140&9.804&9.768&9.774&9.748&9.736\\
13.278&12.300&11.225&9.852&9.816&9.823&9.796&9.785\\
13.394&12.400&11.310&9.906&9.874&9.882&9.855&9.844\\
13.510&12.500&11.370&9.942&9.903&9.911&9.884&9.874\\
13.626&12.600&11.430&9.978&9.941&9.951&9.924&9.913\\
13.742&12.700&11.490&10.014&9.969&9.980&9.952&9.942\\
13.860&12.800&11.550&10.050&10.005&10.019&9.985&9.977\\
13.980&12.900&11.620&10.089&10.041&10.058&10.019&10.013\\
14.100&13.000&11.690&10.128&10.077&10.097&10.053&10.048\\
14.220&13.100&11.760&10.168&10.113&10.136&10.087&10.083\\
14.340&13.200&11.830&10.206&10.149&10.173&10.120&10.119\\
14.460&13.300&11.885&10.232&10.167&10.190&10.137&10.136\\
14.580&13.400&11.940&10.263&10.194&10.214&10.163&10.163\\
14.700&13.500&12.015&10.299&10.230&10.247&10.196&10.198\\
14.820&13.600&12.090&10.346&10.275&10.288&10.239&10.243\\
14.940&13.700&12.165&10.390&10.311&10.320&10.272&10.278\\
15.060&13.800&12.240&10.442&10.356&10.361&10.314&10.322\\
15.180&13.900&12.307&10.487&10.401&10.402&10.357&10.366\\
15.300&14.000&12.367&10.529&10.437&10.436&10.390&10.401\\
15.420&14.100&12.422&10.564&10.463&10.461&10.414&10.426\\
15.540&14.200&12.476&10.606&10.507&10.504&10.455&10.469\\
15.660&14.300&12.530&10.639&10.533&10.529&10.480&10.494\\
15.780&14.400&12.595&10.678&10.569&10.563&10.513&10.528\\
15.900&14.500&12.659&10.722&10.604&10.597&10.546&10.562\\
16.020&14.600&12.723&10.761&10.639&10.631&10.578&10.596\\
16.140&14.700&12.788&10.811&10.683&10.674&10.619&10.639\\
16.256&14.800&12.852&10.856&10.727&10.716&10.660&10.681\\
16.368&14.900&12.917&10.909&10.771&10.759&10.701&10.724\\
16.480&15.000&12.981&10.955&10.806&10.793&10.734&10.758\\
16.588&15.100&13.046&11.004&10.850&10.835&10.775&10.800\\
16.696&15.200&13.110&11.045&10.885&10.868&10.808&10.833\\
16.804&15.300&13.170&11.086&10.928&10.908&10.849&10.875\\
16.912&15.400&13.230&11.127&10.962&10.940&10.882&10.908\\
17.020&15.500&13.290&11.174&10.996&10.973&10.915&10.941\\
17.124&15.600&13.350&11.224&11.039&11.013&10.956&10.983\\
17.228&15.700&13.397&11.266&11.082&11.054&10.997&11.024\\
17.332&15.800&13.443&11.300&11.108&11.078&11.021&11.049\\
17.436&15.900&13.490&11.342&11.143&11.111&11.054&11.082\\
17.540&16.000&13.567&11.406&11.203&11.167&11.111&11.140\\
17.644&16.100&13.644&11.462&11.246&11.208&11.152&11.182\\
17.748&16.200&13.722&11.526&11.308&11.267&11.211&11.241\\
17.852&16.300&13.793&11.584&11.354&11.311&11.254&11.285\\
17.956&16.400&13.859&11.643&11.409&11.363&11.306&11.337\\
\nodata&16.500&13.924&11.693&11.455&11.407&11.349&11.380\\
\nodata&16.600&13.990&11.752&11.510&11.460&11.400&11.433\\
\nodata&16.700&14.058&11.805&11.556&11.504&11.443&11.476\\
\nodata&16.800&14.126&11.858&11.611&11.557&11.495&11.528\\
\nodata&16.900&14.193&11.903&11.648&11.592&11.529&11.563\\
\nodata&17.000&14.258&11.955&11.694&11.636&11.572&11.607\\
\nodata&17.100&14.325&12.000&11.740&11.680&11.615&11.650\\
\nodata&17.200&14.395&12.053&11.787&11.728&11.664&11.697\\
\nodata&17.300&14.468&12.118&11.853&11.795&11.732&11.763\\
\nodata&17.400&14.544&12.176&11.909&11.853&11.790&11.819\\
\nodata&17.500&14.620&12.242&11.966&11.911&11.848&11.876\\
\nodata&17.600&14.700&12.308&12.032&11.978&11.916&11.942\\
\nodata&17.700&14.780&12.374&12.088&12.035&11.974&11.998\\
\nodata&17.800&14.850&12.434&12.144&12.093&12.032&12.054\\
\nodata&17.900&14.910&12.486&12.201&12.151&12.090&12.111\\
\nodata&18.000&14.988&12.556&12.269&12.217&12.157&12.177\\
\nodata&18.100&15.066&12.626&12.338&12.282&12.222&12.242\\
\nodata&18.200&15.144&12.688&12.396&12.339&12.279&12.299\\
\nodata&18.300&15.222&12.758&12.465&12.405&12.345&12.365\\
\nodata&18.400&15.300&12.828&12.534&12.470&12.410&12.430\\
\nodata&18.500&15.377&12.898&12.602&12.536&12.476&12.496\\
\nodata&18.600&15.453&12.959&12.661&12.593&12.533&12.553\\
\nodata&18.700&15.529&13.029&12.728&12.658&12.598&12.617\\
\nodata&18.800&15.606&13.099&12.792&12.724&12.664&12.680\\
\nodata&18.900&15.682&13.162&12.847&12.781&12.721&12.734\\
\nodata&19.000&15.758&13.234&12.912&12.846&12.786&12.797\\
\nodata&19.100&15.834&13.297&12.976&12.912&12.852&12.860\\
\nodata&19.200&15.910&13.369&13.041&12.978&12.918&12.923\\
\nodata&19.300&15.986&13.441&13.105&13.044&12.984&12.986\\
\nodata&19.400&16.062&13.501&13.160&13.100&13.040&13.040\\
\nodata&19.500&16.138&13.569&13.222&13.165&13.105&13.103\\
\nodata&19.600&16.214&13.629&13.275&13.220&13.160&13.157\\
\nodata&19.700&16.289&13.697&13.336&13.284&13.224&13.220\\
\nodata&19.800&16.365&13.756&13.389&13.339&13.279&13.274\\
\nodata&\nodata&16.465&13.837&13.459&13.413&13.353&13.346\\
\nodata&\nodata&16.565&13.905&13.512&13.468&13.408&13.400\\
\nodata&\nodata&16.665&13.972&13.574&13.533&13.473&13.463\\
\nodata&\nodata&16.765&14.040&13.635&13.596&\nodata&\nodata\\
\nodata&\nodata&16.865&14.111&13.695&13.658&\nodata&\nodata\\
\nodata&\nodata&16.965&14.183&13.755&13.720&\nodata&\nodata\\
\nodata&\nodata&17.065&14.256&13.824&13.792&\nodata&\nodata\\
\nodata&\nodata&17.165&14.328&13.884&13.854&\nodata&\nodata\\
\nodata&\nodata&17.265&14.380&13.927&13.898&\nodata&\nodata\\
\nodata&\nodata&17.365&14.422&13.961&13.934&\nodata&\nodata\\
\nodata&\nodata&17.465&14.465&13.996&13.970&\nodata&\nodata\\
\nodata&\nodata&17.565&14.507&14.039&14.014&\nodata&\nodata\\
\nodata&\nodata&17.665&14.564&14.082&14.059&\nodata&\nodata\\
\nodata&\nodata&17.765&14.626&14.142&14.121&\nodata&\nodata\\
\nodata&\nodata&17.865&14.689&14.194&14.174&\nodata&\nodata\\
\nodata&\nodata&17.965&14.751&14.245&14.228&\nodata&\nodata\\
\nodata&\nodata&18.065&14.793&14.280&14.263&\nodata&\nodata\\
\nodata&\nodata&18.165&14.825&14.305&14.290&\nodata&\nodata\\
\nodata&\nodata&18.265&14.858&14.340&14.326&\nodata&\nodata\\
\nodata&\nodata&18.365&14.890&14.366&14.352&\nodata&\nodata\\
\nodata&\nodata&18.465&14.918&14.391&14.379&\nodata&\nodata\\
\nodata&\nodata&18.565&14.943&14.409&14.397&\nodata&\nodata\\
\nodata&\nodata&18.665&14.968&14.434&14.424&\nodata&\nodata\\
\nodata&\nodata&18.765&14.993&14.452&14.441&\nodata&\nodata\\
\nodata&\nodata&\nodata&15.093&14.539&14.529&\nodata&\nodata\\
\nodata&\nodata&\nodata&15.193&14.627&14.617&\nodata&\nodata\\
\nodata&\nodata&\nodata&15.293&14.715&14.705&\nodata&\nodata\\
\nodata&\nodata&\nodata&15.393&14.803&14.793&\nodata&\nodata\\
\nodata&\nodata&\nodata&15.493&14.891&14.881&\nodata&\nodata\\
\enddata
\end{deluxetable}

